String Diagrams for Quantum Foundations, Computing and Natural Language Processing

Applied category theory provides powerful mathematical tools for modelling processes and their composition. Symmetric monoidal categories, which involve series and parallel composition, are particularly well-suited for describing the composition of processes in space and time. Also called process theories, they admit string diagrams, which constitute a visually intuitive, mathematically rigorous, expressive and flexible syntax that is applicable to wide-ranging scientific domains. In this thesis, we employ string diagrams to investigate a selection of topics in the areas of quantum foundations, computing, and natural language processing: (1) We formalise constructor theory as a process theory. In the context of quantum physics, we also demonstrate the conflict between constructor-theoretic principles of locality and composition. Moreover, we argue that if the principle of locality is rejected, categorical quantum mechanics (CQM) can be conceived as a constructor theory of quantum physics. (2) We develop a formalism for wave-based logic circuits with phase encoding. We motivate the formalism using the example of spin-wave circuits, and then demonstrate its utility in design, analysis and optimisation of Boolean logic circuits. (3) We investigate the elimination of inter-language grammatical bureaucracy in the distributional compositional circuits (DisCoCirc) framework. In particular, we develop a hybrid grammar for a restricted fragment of the Urdu language, and show that Urdu text endowed with this hybrid grammar maps surjectively to DisCoCirc text circuits. Furthermore, we show that for the same language fragment, Urdu and English text circuits become the same up to gate-level translation. The aforementioned work supports the view that a process-relational outlook in science is well-supported by applied category-theoretic tools, particularly string diagrams.

==> macros/constructors/tikzstyles3.tex <==
%%% Bob %%%
%\usepackage[svgnames]{xcolor}
%\usepackage{tikz}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric}

\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}

\tikzstyle{none}=[inner sep=0pt]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{every picture}=[baseline=-0.25em,scale=1]
\tikzstyle{dotpic}=[] % for backwards-compatibility
%\tikzstyle{diredges}=[every to/.style={diredge}]





% ================
% = VARIOUS DOTS =
% ================

%\tikzstyle{dot}=[inner sep=0mm,minimum width=0mm,minimum height=0mm,draw,shape=circle]


==> macros/discocirc/defs.tex <==
\newcommand\nuclear{\omding\char195\xspace}
\newcommand\goodskull{\omding\char194\xspace}
\newcommand\frowny{\raisebox{-0.5mm}{\scalebox{1.4}{\omding\char197}}\xspace}
\newcommand\smily{\raisebox{-0.5mm}{\scalebox{1.4}{\omding\char196}}\xspace}

\newcommand*{\threesim}{% 
  \mathrel{\vcenter{\offinterlineskip
  \hbox{$\sim$}\vskip-.35ex\hbox{$\sim$}\vskip-.35ex\hbox{$\sim$}}}}

\newcommand{\C}{\ensuremath{\mathbb{C}}}

\newcommand{\smallsum}{\textstyle{\sum\limits_i}\xspace}
\newcommand{\smallsumi}[1]{\textstyle{\sum\limits_{#1}}\xspace}

\newcommand{\emptydiag}{\,\tikz{\node[style=empty diagram] (x) {};}\,}
\newcommand{\scalar}[1]{\,\tikz{\node[style=scalar] (x) {$#1$};}\,}
\newcommand{\dscalar}[1]{\,\tikz{\node[style=scalar, doubled] (x) {$#1$};}\,}
\newkeycommand{\boxmap}[style=small box][1]{\,\tikz{\node[style=\commandkey{style}] (x) {$#1$};\draw(0,-1.25)--(x)--(0,1.25);}\,}
\newkeycommand{\dboxmap}[style=dbox][1]{\,\tikz{\node[style=\commandkey{style}] (x) {$#1$};\draw[boldedge] (0,-1.25)--(x)--(0,1.25);}\,}
\newcommand{\dhadamard}{\,\tikz{\node[style=dhadamard] (x) {$H$};\draw[boldedge] (0,-1.25)--(x)--(0,1.25);}\,}
\newcommand{\tboxmap}[3]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=small box] (0) at (0, 0) {$#1$};
    \node [style=none] (1) at (0, -0.5) {};
    \node [style=none] (2) at (0, -1.25) {};
    \node [style=none] (3) at (0, 1.25) {};
    \node [style=none] (4) at (0, 0.5) {};
    \node [style=right label] (5) at (0.25, -1) {$#2$};
    \node [style=right label] (6) at (0.25, 1) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (2.center) to (1.center);
    \draw (4.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}}
\newcommand{\boxstate}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(x)--(0,1.25);}\,}
\newcommand{\boxeffect}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(0,-1.25)--(x);}\,}
\newcommand{\boxmapTWOtoONE}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(-0.8,-1)--(x)--(0,1);\draw (0.8,-1)--(x);}\,}
\newcommand{\boxmapONEtoTWO}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(0,-1)--(x)--(-1,1);\draw (x)--(1,1);}\,}

\newcommand{\doubleop}{\ensuremath{\textsf{double}}\xspace}

\newcommand{\kscalar}[1]{\,\tikz{\node[style=kscalar] (x) {$#1$};}\,}
\newcommand{\kscalarconj}[1]{\,\tikz{\node[style=kscalarconj] (x) {$#1$};}\,}

\newcommand{\dmap}[1]{\,\tikz{\node[style=dmap] (x) {$#1$};\draw[boldedge] (0,-1.3)--(x)--(0,1.3);}\,}
\newcommand{\dmapdag}[1]{\,\tikz{\node[style=dmapdag] (x) {$#1$};\draw[boldedge] (0,-1.3)--(x)--(0,1.3);}\,}
\newcommand{\dmaptrans}[1]{\,\tikz{\node[style=dmaptrans] (x) {$#1$};\draw[boldedge] (0,-1.3)--(x)--(0,1.3);}\,}
\newcommand{\dmapconj}[1]{\,\tikz{\node[style=dmapconj] (x) {$#1$};\draw[boldedge] (0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\map}[1]{\,\tikz{\node[style=map] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\maptypes}[3]{\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=map] (0) at (0, 0) {$#1$};
    \node [style=none] (1) at (0, -1.5) {};
    \node [style=none] (2) at (0, 1.5) {};
    \node [style=right label] (3) at (0.25, -1.25) {$#2$};
    \node [style=right label] (4) at (0.25, 1) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (0);
    \draw (0) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}}

\newcommand{\mapdag}[1]{\,\tikz{\node[style=mapdag] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\maptrans}[1]{\,\tikz{\node[style=maptrans] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\mapconj}[1]{\,\tikz{\node[style=mapconj] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\mapONEtoTWO}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=map] (0) at (0, 0) {$#1$};
    \node [style=none] (1) at (0, -0.5) {};
    \node [style=none] (2) at (-0.75, 0.5) {};
    \node [style=none] (3) at (-0.75, 1.25) {};
    \node [style=none] (4) at (0, -1.25) {};
    \node [style=none] (5) at (0.75, 0.5) {};
    \node [style=none] (6) at (0.75, 1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (4.center) to (1.center);
    \draw (2.center) to (3.center);
    \draw (5.center) to (6.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\classicalstate}[1]{%
\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=dkpoint] (0) at (0, -0.75) {$#1$};
    \node [style=white dot] (1) at (0, 0.25) {};
    \node [style=none] (2) at (0, 1) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\wirelabel}[style=white label]{\,\tikz{\node[style=\commandkey{style}]{};}\,\xspace}

\newkeycommand{\pointmap}[style=point][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.3) {$#1$};\node [style=none] (3) at (0, 0.9) {};\node [style=none] (3) at (0, -0.9) {};\draw (x)--(0,0.7);}\,}

%% these are the new ones, prefer to point/copoint
\newkeycommand{\point}[style=point,estyle=][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.05) {$#1$};\draw [\commandkey{estyle}] (x)--(0,1.05);}\,}

\newcommand{\pointdag}[1]{\,\tikz{\node[style=copoint] (x) at (0,0.05) {$#1$};\draw (x)--(0,-1.05);}\,}

\newcommand{\graypointmap}[1]{\pointmap[style=gray point]{#1}}

\newkeycommand{\copointmap}[style=copoint][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,0.3) {$#1$};\draw (x)--(0,-0.7);}\,}

\newcommand{\graycopointmap}[1]{\copointmap[style=gray copoint]{#1}}

\newcommand{\dpointmap}[1]{\,\tikz{\node[style=point,doubled] (x) at (0,-0.3) {$#1$};\draw[boldedge] (x)--(0,0.7);}\,}

\newcommand{\dcopointmap}[1]{\,\tikz{\node[style=copoint, doubled] (x) at (0,0.3) {$#1$};\draw[boldedge] (x)--(0,-0.7);}\,}

\newcommand{\graydcopointmap}[1]{\,\tikz{\node[style=gray copoint, doubled] (x) at (0,0.3) {$#1$};\draw[boldedge] (x)--(0,-0.7);}\,}

\newkeycommand{\dpoint}[style=point][1]{\,\tikz{\node[style=\commandkey{style},doubled] (x) at (0,-0.3) {$#1$};\draw[boldedge] (x)--(0,0.7);}\,}
\newcommand{\dcopoint}[1]{\,\tikz{\node[style=copoint, doubled] (x) at (0,0.3) {$#1$};\draw[boldedge] (x)--(0,-0.7);}\,}

\newkeycommand{\kpoint}[style=kpoint,estyle=][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.05) {$#1$};\draw [\commandkey{estyle}] (x)--(0,1.05);}\,}

\newkeycommand{\kpointgray}[style=gray kpoint,estyle=][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.05) {$#1$};\draw [\commandkey{estyle}] (x)--(0,1.05);}\,}

\newcommand{\kpointgrayconj}[1]{\,\tikz{\node[style=gray kpointconj] (x) at (0,-0.05) {$#1$};\draw (x)--(0,1.05);}\,}

\newcommand{\kpointgrayadj}[1]{\,\tikz{\node[style=gray kpointadj] (x) at (0,0.05) {$#1$};\draw (x)--(0,-1.05);}\,}

\newcommand{\kpointconj}[1]{\,\tikz{\node[style=kpoint conjugate] (x) at (0,-0.05) {$#1$};\draw (x)--(0,1.05);}\,}

\newcommand{\kpointdag}[1]{\,\tikz{\node[style=kpoint adjoint] (x) at (0,0.05) {$#1$};\draw (x)--(0,-1.05);}\,}
\newcommand{\kpointadj}[1]{\kpointdag{#1}}
\newcommand{\kpointtrans}[1]{\,\tikz{\node[style=kpoint transpose] (x) at (0,0.05) {$#1$};\draw (x)--(0,-1.05);}\,}

\newkeycommand{\typedkpoint}[style=kpoint,edgestyle=][2]{%
\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=\commandkey{style}] (1) at (0, -0.75) {$#2$};
    \node [style=right label] (2) at (0.25, 0.5) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{edgestyle}] (1) to (0.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\typedkpointdag}[style=kpoint adjoint,edgestyle=][2]{%
\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1) {};
    \node [style=\commandkey{style}] (1) at (0, 0.75) {$#2$};
    \node [style=right label] (2) at (0.25, -0.5) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{edgestyle}] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\typedpoint}[2]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=point] (1) at (0, -0.5) {$#2$};
    \node [style=right label] (2) at (0.25, 0.5) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1) to (0.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\bistate}[style=kpoint][1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style}, minimum width=1 cm, inner sep=2pt] (0) at (0, -0.25) {$#1$};
    \node [style=none] (1) at (-0.75, 0) {};
    \node [style=none] (2) at (0.75, 0) {};
    \node [style=none] (3) at (-0.75, 0.88) {};
    \node [style=none] (4) at (0.75, 0.88) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (3.center);
    \draw (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\bistatebig}[style=kpoint][1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style}, minimum width=, minimum width=1.26 cm, inner sep=2pt] (0) at (0, -0.25) {$#1$};
    \node [style=none] (1) at (-1, 0) {};
    \node [style=none] (2) at (1, 0) {};
    \node [style=none] (3) at (-1, 0.88) {};
    \node [style=none] (4) at (1, 0.88) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (3.center);
    \draw (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}


\newkeycommand{\dbistate}[style=dkpoint][1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style}, minimum width=1 cm, inner sep=2pt] (0) at (0, -0.25) {$#1$};
    \node [style=none] (1) at (-0.75, 0) {};
    \node [style=none] (2) at (0.75, 0) {};
    \node [style=none] (3) at (-0.75, 1.0) {};
    \node [style=none] (4) at (0.75, 1.0) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [boldedge] (1.center) to (3.center);
    \draw [boldedge] (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\bistateadj}[1]{\,\begin{tikzpicture}[yshift=-3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpointadj, minimum width=1 cm, inner sep=2pt] (0) at (0, 0.5) {$#1$};
    \node [style=none] (1) at (-0.75, 0.25) {};
    \node [style=none] (2) at (0.75, 0.25) {};
    \node [style=none] (3) at (-0.75, -0.63) {};
    \node [style=none] (4) at (0.75, -0.63) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (3.center);
    \draw (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\dbistateadj}[1]{\,\begin{tikzpicture}[yshift=-3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpointadj, doubled, minimum width=1 cm, inner sep=2pt] (0) at (0, 0.5) {$#1$};
    \node [style=none] (1) at (-0.75, 0.25) {};
    \node [style=none] (2) at (0.75, 0.25) {};
    \node [style=none] (3) at (-0.75, -0.5) {};
    \node [style=none] (4) at (0.75, -0.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [boldedge] (1.center) to (3.center);
    \draw [boldedge] (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\bistatebraket}[style1=kpoint,style2=kpointadj][2]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}, minimum width=1 cm, inner sep=2pt] (0) at (0, -0.75) {$#1$};
    \node [style=none] (1) at (-0.75, -0.5) {};
    \node [style=none] (2) at (0.75, -0.5) {};
    \node [style=none] (3) at (-0.75, 0.5) {};
    \node [style=none] (4) at (0.75, 0.5) {};
    \node [style=\commandkey{style2}, minimum width=1 cm, inner sep=2pt] (5) at (0, 0.75) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (3.center);
    \draw (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\binop}[2]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0.75, -1.25) {};
    \node [style=right label, xshift=1 mm] (1) at (0.75, -1) {$#1$};
    \node [style=none] (2) at (0, 1.25) {};
    \node [style=white dot] (3) at (0, 0) {$#2$};
    \node [style=none] (4) at (-0.75, -1.25) {};
    \node [style=right label] (5) at (-0.5, -1) {$#1$};
    \node [style=right label] (6) at (0.25, 1) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [bend right=15, looseness=1.00] (0.center) to (3);
    \draw [bend left=15, looseness=1.00] (4.center) to (3);
    \draw (3) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\weight}[style=dkpoint][1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style}] (0) at (0, -0.5) {$#1$};
    \node [style=upground] (1) at (0, 0.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\weightmap}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.25) {};
    \node [style=dmap] (1) at (0, 0) {$#1$};
    \node [style=upground] (2) at (0, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0.center) to (1);
    \draw [style=boldedge] (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\weightdag}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=downground] (0) at (0, -0.75) {};
    \node [style=dkpointdag] (1) at (0, 0.75) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\mapbent}[1]{\,\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=map] (0) at (1, 0) {$#1$};
		\node [style=none] (1) at (1, 1.25) {};
		\node [style=none] (2) at (-0.5, -0.5) {};
		\node [style=none] (3) at (-0.5, 1.25) {};
		\node [style=none] (4) at (1, -0.5) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (0) to (1.center);
		\draw [in=-90, out=-90, looseness=1.75] (4.center) to (2.center);
		\draw (2.center) to (3.center);
		\draw (4.center) to (0);
	\end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\qproc}[1]{\left(\vphantom{\widehat X}#1\right)}

\newcommand{\dmapdiscard}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=dmap] (0) at (0, 0) {$#1$};
    \node [style=none] (1) at (0, -1.25) {};
    \node [style=upground] (2) at (0, 1.50) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0) to (1.center);
    \draw [style=boldedge] (0) to (2);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\dkpoint}[style=dkpoint][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.1) {$#1$};\draw[boldedge] (x)--(0,1);}\,}
\newkeycommand{\dkpointadj}[style=dkpointadj][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,0.1) {$#1$};\draw[boldedge] (x)--(0,-1);}\,}
\newkeycommand{\dkpointtrans}[style=dkpointtrans][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,0.1) {$#1$};\draw[boldedge] (x)--(0,-1);}\,}
\newkeycommand{\dkpointconj}[style=dkpointconj][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.1) {$#1$};\draw[boldedge] (x)--(0,1);}\,}

\newkeycommand{\blackkpoint}[style=black kpoint][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.1) {$#1$};\draw (x)--(0,1);}\,}
\newkeycommand{\blackkpointadj}[style=black kpointadj][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,0.1) {$#1$};\draw (x)--(0,-1);}\,}
\newkeycommand{\blackdkpoint}[style=black dkpoint][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.1) {$#1$};\draw[boldedge] (x)--(0,1);}\,}
\newkeycommand{\blackdkpointadj}[style=black dkpointadj][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,0.1) {$#1$};\draw[boldedge] (x)--(0,-1);}\,}

\newcommand{\trace}{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -0.60) {};
    \node [style=upground] (1) at (0, 0.40) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=none] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\spider}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=#1] (0) at (0, 0) {};
    \node [style=none] (1) at (1.5, 1.25) {};
    \node [style=none] (2) at (-1, 1.25) {};
    \node [style=none] (3) at (1.25, -1.25) {};
    \node [style=none] (4) at (-0.75, -1.25) {};
    \node [style=none] (5) at (0.25, 1) {$\cdot\cdot\cdot\cdot\cdot$};
    \node [style=none] (6) at (0.25, -1) {$\cdot\cdot\cdot$};
    \node [style=none] (7) at (-1.5, 1.25) {};
    \node [style=none] (8) at (-1.25, -1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=swap, in=135, out=-90, looseness=0.75] (2.center) to (0);
    \draw [style=swap, in=-90, out=45, looseness=0.75] (0) to (1.center);
    \draw [style=swap, in=90, out=-45, looseness=0.75] (0) to (3.center);
    \draw [style=swap, in=90, out=-135, looseness=0.75] (0) to (4.center);
    \draw [style=swap, in=-153, out=90, looseness=0.50] (8.center) to (0);
    \draw [style=swap, in=149, out=-90, looseness=0.50] (7.center) to (0);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand\discard\trace

%%% BOB %%%
%\newcommand\D{\textrm{\footnotesize $D$}\xspace}
%\newcommand\sqrtD{\textrm{\footnotesize $\sqrt{D}$}\xspace}
%\newcommand\oneoverD{\ensuremath{{\textstyle{1\over{D}}}}\xspace}
%\newcommand\oneoversqrtD{\ensuremath{{\textstyle{1\over{\sqrt{D}}}}}\xspace}
%\newcommand\oneoversqrttwo{\ensuremath{{\textstyle{1\over{\sqrt{2}}}}}\xspace}

\newcommand{\maxmix}{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (-0.25, 0.60) {};
    \node [style=downground] (1) at (-0.25, -0.40) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=none] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\namedeq}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 0.75) {\footnotesize $#1$};
    \node [style=none] (1) at (0, 0) {$=$};
  \end{pgfonlayer}
\end{tikzpicture}\,}
\newcommand{\namedmapsto}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 0.75) {\footnotesize $#1$};
    \node [style=none] (1) at (0, 0) {$\mapsto$};
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\scalareq}{\ensuremath{\approx}\xspace}
\newcommand{\scalareqalt}{\ensuremath{\threesim}\xspace}
%
%\ensuremath{\overset{\diamond}{=}}\xspace}

% \newkeycommand{\pointketbra}[style1=copoint,style2=point][2]{\,%
% \begin{tikzpicture}
%   \begin{pgfonlayer}{nodelayer}
%     \node [style=none] (0) at (0, -1.9) {};
%     \node [style=\commandkey{style1}] (1) at (0, -0.95) {$#1$};
%     \node [style=\commandkey{style2}] (2) at (0, 0.95) {$#2$};
%     \node [style=none] (3) at (0, 1.9) {};
%   \end{pgfonlayer}
%   \begin{pgfonlayer}{edgelayer}
%     \draw (0.center) to (1);
%     \draw (2) to (3.center);
%   \end{pgfonlayer}
% \end{tikzpicture}\,}

\newkeycommand{\pointketbra}[style1=copoint,style2=point,estyle=][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.75) {};
    \node [style=\commandkey{style1}] (1) at (0, -0.75) {$#1$};
    \node [style=\commandkey{style2}] (2) at (0, 0.75) {$#2$};
    \node [style=none] (3) at (0, 1.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{estyle}] (0.center) to (1);
    \draw [\commandkey{estyle}] (2) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\twocopointketbra}[style1=copoint,style2=copoint,style3=point][3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (-0.75, -1.75) {};
    \node [style=none] (1) at (0.75, -1.75) {};
    \node [style=\commandkey{style1}] (2) at (-0.75, -0.75) {$#1$};
    \node [style=\commandkey{style2}] (3) at (0.75, -0.75) {$#2$};
    \node [style=\commandkey{style3}] (4) at (0, 0.75) {$#3$};
    \node [style=none] (5) at (0, 1.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (2);
    \draw (1.center) to (3);
    \draw (4) to (5.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\graytwocopointketbra}{\twocopointketbra[style1=gray copoint,style2=gray copoint,style3=gray point]}

\newkeycommand{\twopointketbra}[style1=copoint,style2=point,style3=point][3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.75) {};
    \node [style=none] (1) at (-0.75, 1.75) {};
    \node [style=\commandkey{style1}] (2) at (0, -0.75) {$#1$};
    \node [style=\commandkey{style2}] (3) at (-0.75, 0.75) {$#2$};
    \node [style=\commandkey{style3}] (4) at (0.75, 0.75) {$#3$};
    \node [style=none] (5) at (0.75, 1.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (2);
    \draw (1.center) to (3);
    \draw (4) to (5.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\graytwopointketbra}{\twopointketbra[style1=gray copoint,style2=gray point,style3=gray point]}

\newcommand{\idwire}{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.5) {};
    \node [style=none] (3) at (0, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\didwire}{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.5) {};
    \node [style=none] (3) at (0, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [boldedge] (0.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\didwirelong}{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -2) {};
    \node [style=none] (3) at (0, 2) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [boldedge] (0.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\shortidwire}{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1) {};
    \node [style=none] (3) at (0, 1) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\pointbraket}[style1=point,style2=copoint,estyle=][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -0.625) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.625) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{estyle}] (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\graypointbraket}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=gray point] (0) at (0, -0.625) {$#1$};
    \node [style=gray copoint] (1) at (0, 0.625) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\dpointbraket}[2]{\kpointbraket[style1=dpoint,style2=dcopoint,estyle=boldedge]{#1}{#2}}

\newcommand{\dkpointbraket}[2]{\kpointbraket[style1=dkpoint,style2=dkpointdag,estyle=boldedge]{#1}{#2}}

\newcommand{\dpointbraketx}[2]{\kpointbraketx[style1=dpoint,style2=dcopoint,estyle=boldedge]{#1}{#2}}

\newcommand{\dkpointbraketx}[2]{\kpointbraketx[style1=dkpoint,style2=dkpointdag,estyle=boldedge]{#1}{#2}}

\newkeycommand{\kpointketbra}[style1=kpointdag,style2=kpoint,estyle=][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.9) {};
    \node [style=\commandkey{style1}] (1) at (0, -0.95) {$#1$};
    \node [style=\commandkey{style2}] (2) at (0, 0.95) {$#2$};
    \node [style=none] (3) at (0, 1.9) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{estyle}] (0.center) to (1);
    \draw [\commandkey{estyle}] (2) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\dkpointketbra}[2]{\kpointketbra[style1=dkpointdag,style2=dkpoint,estyle=boldedge]{#1}{#2}}

\newcommand{\kpointketbratwocols}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.9) {};
    \node [style=kpointdag] (1) at (0, -0.85) {$#1$};
    \node [style=kpoint,fill=gray!40!white] (2) at (0, 0.85) {$#2$};
    \node [style=none] (3) at (0, 1.9) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer} 
    \draw (0.center) to (1);
    \draw (2) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\boxpointmap}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1) {$#1$};
    \node [style=map] (1) at (0, 0.5) {$#2$};
    \node [style=none] (2) at (0, 1.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\boxtranspointmap}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.50) {$#1$};
    \node [style=maptrans] (1) at (0, 0) {$#2$};
    \node [style=none] (2) at (0, 1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\kpointmap}[style1=kpoint,style2=map][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.1) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.5) {$#2$};
    \node [style=none] (2) at (0, 1.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\kpointmaptrans}[style1=kpointconj,style2=mapadj][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.1) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.5) {$#2$};
    \node [style=none] (2) at (0, 1.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\kpointmapadj}[style1=kpointadj,style2=map][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, 1.1) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, -0.5) {$#2$};
    \node [style=none] (2) at (0, -1.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\dkpointmap}[style1=dkpoint,style2=dmap][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.2) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.4) {$#2$};
    \node [style=none] (2) at (0, 1.7) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw[style=boldedge] (0) to (1);
    \draw[style=boldedge] (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\dkpointmapx}[style1=dkpoint,style2=dmap][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.4) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.6) {$#2$};
    \node [style=none] (2) at (0, 1.9) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw[style=boldedge] (0) to (1);
    \draw[style=boldedge] (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\boxpointmapdag}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.50) {$#1$};
    \node [style=mapdag] (1) at (0, 0) {$#2$};
    \node [style=none] (2) at (0, 1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\boxcopointmap}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.75) {};
    \node [style=map] (1) at (0, -0.5) {$#1$};
    \node [style=copoint] (2) at (0, 1) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\boxcopointmapdag}[style1=map,style2=copoint][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.75) {};
    \node [style=\commandkey{style1}] (1) at (0, -0.5) {$#1$};
    \node [style=\commandkey{style2}] (2) at (0, 1) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\kpointdagmap}[style1=map,style2=kpointdag][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.75) {};
    \node [style=\commandkey{style1}] (1) at (0, -0.5) {$#1$};
    \node [style=\commandkey{style2}] (2) at (0, 1.1) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\kpointdagmapdag}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.75) {};
    \node [style=mapdag] (1) at (0, -0.5) {$#1$};
    \node [style=kpointdag] (2) at (0, 1.1) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\sandwichmap}[style1=point,style2=map,style3=copoint][3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.50) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0) {$#2$};
    \node [style=\commandkey{style3}] (2) at (0, 1.50) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newkeycommand{\kpointsandwichmap}[style1=kpoint,style2=map,style3=kpointdag][3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.5) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0) {$#2$};
    \node [style=\commandkey{style3}] (2) at (0, 1.5) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\dkpointsandwichmap}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=dkpoint] (0) at (0, -1.5) {$#1$};
    \node [style=dmap] (1) at (0, 0) {$#2$};
    \node [style=dkpointdag] (2) at (0, 1.5) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [boldedge] (0) to (1);
    \draw [boldedge] (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\dkpointsandwichmapx}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=dkpoint] (0) at (0, -1.85) {$#1$};
    \node [style=dmap] (1) at (0, 0) {$#2$};
    \node [style=dkpointdag] (2) at (0, 1.85) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [boldedge] (0) to (1);
    \draw [boldedge] (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\kpointsandwichmapdag}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpoint] (0) at (0, -1.5) {$#1$};
    \node [style=mapdag] (1) at (0, 0) {$#2$};
    \node [style=kpointdag] (2) at (0, 1.5) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\sandwichmapdag}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.50) {$#1$};
    \node [style=mapdag] (1) at (0, 0) {$#2$};
    \node [style=copoint] (2) at (0, 1.50) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\sandwichmaptrans}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.50) {$#1$};
    \node [style=maptrans] (1) at (0, 0) {$#2$};
    \node [style=copoint] (2) at (0, 1.50) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newkeycommand{\sandwichmapconj}[style1=point,style2=mapconj,style3=copoint][3]{\,% 
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.50) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0) {$#2$};
    \node [style=\commandkey{style3}] (2) at (0, 1.50) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newkeycommand{\sandwichtwo}[style1=point,style2=map,style3=map,style4=copoint][4]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style2}] (0) at (0, -1) {$#2$};
    \node [style=\commandkey{style3}] (1) at (0, 1) {$#3$};
    \node [style=\commandkey{style1}] (2) at (0, -2.6) {$#1$};
    \node [style=\commandkey{style4}] (3) at (0, 2.6) {$#4$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (2) to (0);
    \draw (0) to (1);
    \draw (1) to (3);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\longbraket}[style1=point,style2=copoint][2]{\,% 
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -2.6) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 2.6) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\onb}[style=point]{\ensuremath{\{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.3) {$j$};\draw (x)--(0,0.7);}\,\}}\xspace}

\newcommand{\whiteonb}{\onb[style=point]}

\newcommand{\grayonb}{\onb[style=gray point]}

\newcommand{\redonb}{\onb[style=red point]}

\newcommand{\greenonb}{\onb[style=green point]}

\newcommand{\whiteonbi}{\ensuremath{\left\{\raisebox{1mm}{\pointmap{i}}\right\}_i}\xspace}
\newcommand{\grayonbi}{\ensuremath{\left\{\raisebox{1mm}{\graypointmap{i}}\right\}_i}\xspace}
\newcommand{\greyonbi}{\ensuremath{\left\{\raisebox{1mm}{\graypointmap{i}}\right\}_i}\xspace}

\newcommand{\redpointmap}[1]{\,\tikz{\node[style=red point] (x) at (0,-0.3) {$#1$};\draw (x)--(0,0.7);}\,}

\newcommand{\redcopointmap}[1]{\,\tikz{\node[style=red copoint] (x) at (0,0.3) {$#1$};\draw (x)--(0,-0.7);}\,}

\newcommand{\greenpointmap}[1]{\,\tikz{\node[style=green point] (x) at (0,-0.3) {$#1$};\draw (x)--(0,0.7);}\,}

\newcommand{\greencopointmap}[1]{\,\tikz{\node[style=green copoint] (x) at (0,0.3) {$#1$};\draw (x)--(0,-0.7);}\,}

\newcommand{\meas}{\ensuremath{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=white dot] (0) at (0, 0) {};
    \node [style=none] (1) at (0, 0.75) {};
    \node [style=none] (2) at (0, -0.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=swap] (1.center) to (0);
    \draw [style=boldedge] (0) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}\xspace}

\newcommand{\encode}{\ensuremath{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -0.75) {};
    \node [style=none] (1) at (0, 0.75) {};
    \node [style=white dot] (2) at (0, 0) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=swap] (2.center) to (0);
    \draw [style=boldedge] (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}\xspace}

% \newkeycommand{\comult}[style=white dot]{\,\begin{tikzpicture}
%   \begin{pgfonlayer}{nodelayer}
%     \node [style=none] (0) at (0, -1) {};
%     \node [style=none] (1) at (-0.75, 1) {};
%     \node [style=\commandkey{style}] (2) at (0, 0) {};
%     \node [style=none] (3) at (0.75, 1) {};
%   \end{pgfonlayer}
%   \begin{pgfonlayer}{edgelayer}
%     \draw [bend left=15, looseness=1.00] (2) to (1.center);
%     \draw (0.center) to (2);
%     \draw [bend right=15, looseness=1.00] (2) to (3.center);
%   \end{pgfonlayer}
% \end{tikzpicture}\,\xspace}

% \newkeycommand{\mult}[style=white dot]{\,\begin{tikzpicture}
%   \begin{pgfonlayer}{nodelayer}
%     \node [style=none] (0) at (0, 1) {};
%     \node [style=none] (1) at (-0.75, -1) {};
%     \node [style=\commandkey{style}] (2) at (0, 0) {};
%     \node [style=none] (3) at (0.75, -1) {};
%   \end{pgfonlayer}
%   \begin{pgfonlayer}{edgelayer}
%     \draw [bend right=15, looseness=1.00] (2) to (1.center);
%     \draw (0.center) to (2);
%     \draw [bend left=15, looseness=1.00] (2) to (3.center);
%   \end{pgfonlayer}
% \end{tikzpicture}\,\xspace}

\newcommand{\grayphasemult}[2]{\,\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=gray dot] (0) at (0, 0.5) {};
		\node [style=gray phase dot] (1) at (0.75, -0.75) {$#1$};
		\node [style=gray phase dot] (2) at (-0.75, -0.75) {$#2$};
		\node [style=none] (3) at (0, 1.5) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-165, out=90, looseness=1.00] (2) to (0);
		\draw [in=-15, out=90, looseness=1.00] (1) to (0);
		\draw (0) to (3.center);
	\end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\grayphasemultbis}[2]{\,\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=gray dot] (0) at (0, 0.5) {};
		\node [style=point] (1) at (0.75, -0.75) {$#1$};
		\node [style=point] (2) at (-0.75, -0.75) {$#2$};
		\node [style=none] (3) at (0, 1.5) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-165, out=90, looseness=1.00] (2) to (0);
		\draw [in=-15, out=90, looseness=1.00] (1) to (0);
		\draw (0) to (3.center);
	\end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\phasepointmult}[2]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=white dot] (0) at (0, 0.5) {};
    \node [style=white dot] (1) at (-0.75, -0.75) {$#1$};
    \node [style=none] (2) at (0, 1.5) {};
    \node [style=white dot] (3) at (0.75, -0.75) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [in=-165, out=90, looseness=1.00] (1) to (0);
    \draw [in=-15, out=90, looseness=1.00] (3) to (0);
    \draw (0) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}


\newcommand{\grayphasepoint}[1]{\phasepoint[style=gray phase dot]{#1}}
\newcommand{\grayphasecopoint}[1]{\phasecopoint[style=gray phase dot]{#1}}

\newcommand{\graysquarepoint}[1]{\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=gray square point] (0) at (0, -0.5) {};
        \node [style=none] (1) at (0, 0.75) {};
        \node [style=none] (2) at (0.75, -0.5) {$#1$};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (0) to (1.center);
    \end{pgfonlayer}
\end{tikzpicture}}

\newkeycommand{\phase}[style=white phase dot][1]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 1) {};
        \node [style=\commandkey{style}] (2) at (0, -0) {$#1$}; 
        \node [style=none] (3) at (0, -1) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (2) to (0.center);
        \draw (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

% \newcommand{\whitephase}[1]{\phase{#1}}
% \newcommand{\greyphase}[1]{\phase[style=gray dot]{#1}}
% \newcommand{\grayphase}[1]{\phase[style=gray dot]{#1}}

\newkeycommand{\dphase}[style=white phase ddot][1]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 1.25) {};
        \node [style=\commandkey{style}] (2) at (0, -0) {$#1$};
        \node [style=none] (3) at (0, -1.25) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw [boldedge] (2) to (0.center);
        \draw [boldedge] (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\dphasegray}[1]{\dphase[style=gray phase ddot]{#1}}

\newkeycommand{\dphasepoint}[style=white phase ddot][1]{\,\begin{tikzpicture}[yshift=-3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=\commandkey{style}] (1) at (0, 0) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\dphasepointgray}[style=gray phase ddot][1]{\,\begin{tikzpicture}[yshift=-3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=\commandkey{style}] (1) at (0, 0) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\dphasecopoint}[style=white phase ddot][1]{\,\begin{tikzpicture}[yshift=3mm,yscale=-1]
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=\commandkey{style}] (1) at (0, 0) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\dphasepointsm}[style=white phase ddot][1]{\,\begin{tikzpicture}[yshift=-3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=\commandkey{style}] (1) at (0, 0) {\footnotesize\!$#1$\!};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\measure}[1]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 0.75) {};
        \node [style=#1] (2) at (0, -0) {};
        \node [style=none] (3) at (0, -0.75) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (2) to (0.center);
        \draw[doubled] (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\nondemmeasure}[1]{\,\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=none] (0) at (1, 1) {};
		\node [style=none] (1) at (1, 1.25) {};
		\node [style=none] (2) at (0.75, 0.5) {};
		\node [style=#1] (3) at (0, -0.25) {};
		\node [style=none] (4) at (0, 1.25) {};
		\node [style=none] (5) at (0, -1.25) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (0.center) to (1.center);
		\draw (3) to (2.center);
		\draw [in=-90, out=45, looseness=1.00] (2.center) to (0.center);
		\draw [style=boldedge] (5.center) to (3);
		\draw [style=boldedge] (3) to (4.center);
	\end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\prepare}[1]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 0.75) {};
        \node [style=#1] (2) at (0, -0) {};
        \node [style=none] (3) at (0, -0.75) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw[doubled] (2) to (0.center);
        \draw (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\whitephase}[1]{\phase[style=white phase dot]{#1}}
\newcommand{\whitedphase}[1]{\dphase[style=white phase ddot]{#1}}
\newcommand{\greyphase}[1]{\phase[style=grey phase dot]{#1}}
\newcommand{\greydphase}[1]{\dphase[style=grey phase ddot]{#1}}


\newkeycommand{\phasepoint}[style=white phase dot][1]{\,\begin{tikzpicture}[yshift=-3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=\commandkey{style}] (1) at (0, 0) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\phasecopoint}[style=white phase dot][1]{\,\begin{tikzpicture}[yshift=3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1) {};
    \node [style=\commandkey{style}] (1) at (0, 0) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}


\newcommand{\pointcopointmap}[2]{\,\tikz{
  \node[style=copoint] (x) at (0,-0.7) {$#2$};\draw (x)--(0,-1.5);
  \node[style=point] (y) at (0,0.7) {$#1$};\draw (0,1.5)--(y);
}\,}

\newcommand{\innerprodmap}[2]{\,\tikz{
\node[style=copoint] (y) at (0,0.625) {$#1$};
\node[style=point] (x) at (0,-0.625) {$#2$};
\draw (x)--(y);}\,}

\newkeycommand{\kpointbraket}[style1=kpoint,style2=kpoint adjoint,estyle=][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -0.735) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.735) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{estyle}] (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\kkpointbraket}[style1=kpoint,style2=kpoint adjoint,estyle=][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -0.685) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.685) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{estyle}] (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\kpointbraketx}[style1=kpoint,style2=kpoint adjoint,estyle=][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -0.885) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.885) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{estyle}] (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\kpointbraketconj}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpoint conjugate] (0) at (0, -0.735) {$#1$};
    \node [style=kpoint transpose] (1) at (0, 0.735) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\wginnerprodmap}[2]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=point] (0) at (0, -0.75) {$#2$};
        \node [style=gray copoint] (1) at (0, 0.75) {$#1$};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (0) to (1);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\def\alpvec{[\vec{\alpha}]}
\def\alpprevec{\vec{\alpha}}
\def\betvec{[\vec{\beta}_j]}
\def\betprevec{\vec{\beta}_j}

\def\blackmu{\mu_{\smallblackdot}} 
\def\graymu {\mu_{\smallgraydot}}
\def\whitemu{\mu_{\smallwhitedot}}

\def\blacketa{\eta_{\smallblackdot}} 
\def\grayeta {\eta_{\smallgraydot}}
\def\whiteeta{\eta_{\smallwhitedot}}

\def\blackdelta{\delta_{\smallblackdot}} 
\def\graydelta {\delta_{\smallgraydot}}
\def\whitedelta{\delta_{\smallwhitedot}}

\def\blackepsilon{\epsilon_{\smallblackdot}} 
\def\grayepsilon {\epsilon_{\smallgraydot}}
\def\whiteepsilon{\epsilon_{\smallwhitedot}}

% \def\whiteeta{\eta_{\!\smallwhitedot}}
% \def\whitevarepsilon{\varepsilon_{\!\smallwhitedot}}

\def\whitePhi{\Phi_{\!\smallwhitedot}}
\def\graymeas{m_{\!\smallgraydot}}

\newcommand{\Owg}{\ensuremath{{\cal O}_{\!\smallwhitedot\!,\!\smallgraydot}}}
\newcommand{\whiteK}{\ensuremath{{\cal  K}_{\!\smallwhitedot}}}
\newcommand{\grayK}{\ensuremath{{\cal  K}_{\!\smallgraydot}}}


% BRAS AND KETS
\newcommand{\bra}[1]{\ensuremath{\left\langle #1 \right|}}
\newcommand{\ket}[1]{\ensuremath{\left|  #1 \right\rangle}}
\newcommand{\roundket}[1]{\ensuremath{\left|  #1 \right)}}
\newcommand{\braket}[2]{\ensuremath{\langle#1|#2\rangle}}
\newcommand{\ketbra}[2]{\ensuremath{\ket{#1}\!\bra{#2}}}

\newcommand{\ketGHZ} {\ket{\textit{GHZ}\,}}
\newcommand{\ketW}   {\ket{\textit{W\,}}}
\newcommand{\ketBell}{\ket{\textit{Bell\,}}}
\newcommand{\ketEPR} {\ket{\textit{EPR\,}}}
\newcommand{\ketGHZD}{\ket{\textrm{GHZ}^{(D)}}}
\newcommand{\ketWD}  {\ket{\textrm{W}^{(D)}}}

\newcommand{\braGHZ} {\bra{\textit{GHZ}\,}}
\newcommand{\braW}   {\bra{\textit{W\,}}}
\newcommand{\braBell}{\bra{\textit{Bell\,}}}
\newcommand{\braEPR} {\bra{\textit{EPR\,}}}


% CATEGORY VARIABLES
\newcommand{\catC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\catCop}{\ensuremath{\mathcal{C}^{\mathrm{op}}}\xspace}
\newcommand{\catD}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\catDop}{\ensuremath{\mathcal{D}^{\mathrm{op}}}\xspace}


% STANDARD CATEGORIES
\newcommand{\catSet}{\ensuremath{\textrm{\bf Set}}\xspace}
\newcommand{\catRel}{\ensuremath{\textrm{\bf Rel}}\xspace}
\newcommand{\catFRel}{\ensuremath{\textrm{\bf FRel}}\xspace}
\newcommand{\catVect}{\ensuremath{\textrm{\bf Vect}}\xspace}
\newcommand{\catFVect}{\ensuremath{\textrm{\bf FVect}}\xspace}
\newcommand{\catFHilb}{\ensuremath{\textrm{\bf FHilb}}\xspace}
\newcommand{\catHilb}{\ensuremath{\textrm{\bf Hilb}}\xspace}
\newcommand{\catSuperHilb}{\ensuremath{\textrm{\bf SuperHilb}}\xspace}
\newcommand{\catAb}{\ensuremath{\textrm{\bf Ab}}\xspace}
\newcommand{\catTop}{\ensuremath{\textrm{\bf Top}}\xspace}
\newcommand{\catCHaus}{\ensuremath{\textrm{\bf CHaus}}\xspace}
\newcommand{\catHaus}{\ensuremath{\textrm{\bf Haus}}\xspace}
\newcommand{\catGraph}{\ensuremath{\textrm{\bf Graph}}\xspace}
\newcommand{\catMat}{\ensuremath{\textrm{\bf Mat}}\xspace}
\newcommand{\catGr}{\ensuremath{\textrm{\bf Gr}}\xspace}
\newcommand{\catSpek}{\ensuremath{\textrm{\bf Spek}}\xspace}




% ========================
% = COMMUTATIVE DIAGRAMS =
% ========================

\tikzstyle{cdiag}=[matrix of math nodes, row sep=3em, column sep=3em, text height=1.5ex, text depth=0.25ex,inner sep=0.5em]
\tikzstyle{arrow above}=[transform canvas={yshift=0.5ex}]
\tikzstyle{arrow below}=[transform canvas={yshift=-0.5ex}]

\newcommand{\csquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
\end{tikzpicture}
}

% commands for putting pushout/pullback brackets on commutative diags
\newcommand{\NWbracket}[1]{%
\draw #1 +(-0.25,0.5) -- +(-0.5,0.5) -- +(-0.5,0.25);}
\newcommand{\NEbracket}[1]{%
\draw #1 +(0.25,0.5) -- +(0.5,0.5) -- +(0.5,0.25);}
\newcommand{\SWbracket}[1]{%
\draw #1 +(-0.25,-0.5) -- +(-0.5,-0.5) -- +(-0.5,-0.25);}
\newcommand{\SEbracket}[1]{%
\draw #1 +(0.25,-0.5) -- +(0.5,-0.5) -- +(0.5,-0.25);}
\newcommand{\THETAbracket}[2]{%
\draw [rotate=#1] #2 +(0.25,0.5) -- +(0.5,0.5) -- +(0.5,0.25);}

\newcommand{\posquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node [swap] {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
    \NWbracket{(m-2-2)}
\end{tikzpicture}
}

\newcommand{\pbsquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node [swap] {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
  \SEbracket{(m-1-1)}
\end{tikzpicture}
}

\newcommand{\ctri}[6]{
    \begin{tikzpicture}[-latex]
        \matrix (m) [cdiag,ampersand replacement=\&] { #1 \& #2 \\ #3 \& \\ };
        \path [arrs] (m-1-1) edge node {$#4$} (m-1-2)
              (m-1-1) edge node [swap] {$#5$} (m-2-1)
              (m-2-1) edge node [swap] {$#6$} (m-1-2);
    \end{tikzpicture}
}

% \newcommand{\crun}[5]{
% \ensuremath{#1 \overset{#2}{\longrightarrow} #3 \overset{#4}{\longrightarrow} #5}
% }

\newcommand{\carr}[3]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #3 \\};
    \path [arrs] (m-1-1) edge node {$#2$} (m-1-2);
\end{tikzpicture}
}

\newcommand{\crun}[5]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #3 \& #5 \\};
    \path [arrs] (m-1-1) edge node {$#2$} (m-1-2)
                 (m-1-2) edge node {$#4$} (m-1-3);
\end{tikzpicture}
}

\newcommand{\cspan}[5]{
\ensuremath{#1 \overset{#2}{\longleftarrow} #3
               \overset{#4}{\longrightarrow} #5}
}

\newcommand{\ccospan}[5]{
\ensuremath{#1 \overset{#2}{\longrightarrow} #3
               \overset{#4}{\longleftarrow} #5}
}

\newcommand{\cpair}[4]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\};
    \path [arrs] (m-1-1.20) edge node {$#3$} (m-1-2.160)
                 (m-1-1.-20) edge node [swap] {$#4$} (m-1-2.-160);
\end{tikzpicture}
}

\newcommand{\csquareslant}[9]{
\begin{tikzpicture}[-latex]
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2)
                 (m-1-2) edge node [swap] {$#9$} (m-2-1);
\end{tikzpicture}
}




==> macros/discocirc/tikzfigures.tex <==
% define in-prose representations for lots of generators

%%%%REVERSED BY BOB %%%%%%%%

%\newcommand{\bigcounit}[1]{%
%\,\begin{tikzpicture}[dotpic,scale=2,yshift=-1mm]
%\node [#1] (a) at (0,0.25) {}; 
%\draw (0,-0.2)--(a);
%\end{tikzpicture}\,}
%\newcommand{\bigunit}[1]{%
%\,\begin{tikzpicture}[dotpic,scale=2,yshift=1.5mm]
%\node [#1] (a) at (0,-0.25) {}; 
%\draw (a)--(0,0.2);
%\end{tikzpicture}\,}
%\newcommand{\bigcomult}[1]{%
%\,\begin{tikzpicture}[dotpic,scale=2,yshift=0.5mm]
%	\node [#1] (a) {};
%	\draw (-90:0.55)--(a);
%	\draw (a) -- (45:0.6);
%	\draw (a) -- (135:0.6);
%\end{tikzpicture}\,}
%\newcommand{\bigmult}[1]{%
%\,\begin{tikzpicture}[dotpic,scale=2]
%	\node [#1] (a) {};
%	\draw (a) -- (90:0.55);
%	\draw (a) (-45:0.6) -- (a);
%	\draw (a) (-135:0.6) -- (a);
%\end{tikzpicture}\,}


%\newcommand{\dotcounit}[1]{%
%\,\begin{tikzpicture}[dotpic,yshift=-1mm]
%\node [#1] (a) at (0,0.35) {}; 
%\draw (0,-0.3)--(a);
%\end{tikzpicture}\,}
%\newcommand{\dotunit}[1]{%
%\,\begin{tikzpicture}[dotpic,yshift=1.5mm]
%\node [#1] (a) at (0,-0.35) {}; 
%\draw (a)--(0,0.3);
%\end{tikzpicture}\,}
%\newcommand{\dotcomult}[1]{%
%\,\begin{tikzpicture}[dotpic,yshift=0.5mm]
%	\node [#1] (a) {};
%	\draw (-90:0.55)--(a);
%	\draw (a) -- (45:0.6);
%	\draw (a) -- (135:0.6);
%\end{tikzpicture}\,}
%\newcommand{\dotmult}[1]{%
%\,\begin{tikzpicture}[dotpic]
%	\node [#1] (a) {};
%	\draw (a) -- (90:0.55);
%	\draw (a) (-45:0.6) -- (a);
%	\draw (a) (-135:0.6) -- (a);
%\end{tikzpicture}\,}

%\newcommand{\ddotmult}[1]{%
%\,\begin{tikzpicture}[dotpic]
%	\node [#1] (a) {};
%	\draw [boldedge] (a) -- (90:0.55);
%	\draw [boldedge] (a) (-45:0.6) -- (a);
%	\draw [boldedge] (a) (-135:0.6) -- (a);
%\end{tikzpicture}\,}

% \newcommand{\spider}[2]{%
% \begin{tikzpicture}[dotpic]
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=#1] (0) at (0, 0) {};
% 		\node [style=none] (1) at (1.25, 1) {};
% 		\node [style=none] (2) at (-0.75, 1) {};
% 		\node [style=none] (3) at (1, -1) {};
% 		\node [style=none] (4) at (-0.75, -1) {};
% 		\node [style=none] (5) at (0.25, 0.75) {$\cdot\cdot\cdot$};
% 		\node [style=none] (6) at (0, -0.75) {$\cdot\cdot\cdot$};
% 		\node [style=none] (7) at (-1.25, 1) {};
% 		\node [style=none] (8) at (-1.25, -1) {};
% 		\node [style=none, anchor=west] (9) at (0.75, 0) {$#2$};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw [style=swap, in=135, out=-90, looseness=0.75] (2.center) to (0);
% 		\draw [style=swap, in=-90, out=45, looseness=0.75] (0) to (1.center);
% 		\draw [style=swap, in=90, out=-45, looseness=0.75] (0) to (3.center);
% 		\draw [style=swap, in=90, out=-135, looseness=0.75] (0) to (4.center);
% 		\draw [style=swap, in=-153, out=90, looseness=0.50] (8.center) to (0);
% 		\draw [style=swap, in=149, out=-90, looseness=0.50] (7.center) to (0);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% }

%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\dotidualiser}[1]{%
%\begin{tikzpicture}[dotpic,yshift=1.5mm]
%	\node [#1] (a) {};
%	\draw [medium diredge] (a) to (-90:0.35);
%	\draw [medium diredge] (a) to (90:0.35);
%\end{tikzpicture}}
%\newcommand{\dotdualiser}[1]{%
%\begin{tikzpicture}[dotpic,yshift=1.5mm]
%	\node [#1] (a) {};
%	\draw [medium diredge] (-90:0.35) to (a);
%	\draw [medium diredge] (90:0.35) to (a);
%\end{tikzpicture}}
%\newcommand{\dottickunit}[1]{%
%\begin{tikzpicture}[dotpic,yshift=-1mm]
%\node [#1] (a) at (0,0.35) {}; 
%\draw [postaction=decorate,
%       decoration={markings, mark=at position 0.3 with \edgetick},
%       decoration={markings, mark=at position 0.85 with \edgearrow}] (a)--(0,-0.25);
%\end{tikzpicture}}
%\newcommand{\dottickcounit}[1]{%
%\begin{tikzpicture}[dotpic,yshift=1mm]
%\node [#1] (a) at (0,-0.35) {}; 
%\draw [postaction=decorate,
%       decoration={markings, mark=at position 0.8 with \edgetick},
%       decoration={markings, mark=at position 0.45 with \edgearrow}] (0,0.25) -- (a);
%\end{tikzpicture}}
%\newcommand{\dotonly}[1]{%
%\,\begin{tikzpicture}[dotpic]
%\node [#1] (a) at (0,0) {};
%\end{tikzpicture}\,}
%NEW:
%\newcommand{\smalldotonly}[1]{%
%\,\begin{tikzpicture}[dotpic,yshift=-0.15mm]
%\node [#1] (a) at (0,0) {};
%\end{tikzpicture}\,}
%
%\newcommand{\dotthreestate}[1]{%
%\,\begin{tikzpicture}[dotpic,yshift=2.5mm]
%	\node [#1] (a) at (0,0) {};
%	\draw (a) -- (0,-0.6);
%	\draw [bend right] (a) to (-0.4,-0.6) (0.4,-0.6) to (a);
%\end{tikzpicture}\,}
%\newcommand{\dotcap}[1]{%
%\,\begin{tikzpicture}[dotpic,yshift=2.5mm]
%	\node [#1] (a) at (0,0) {};
%	\draw [bend right,medium diredge] (a) to (-0.4,-0.6);
%	\draw [bend left,medium diredge] (a) to (0.4,-0.6);
%\end{tikzpicture}\,}
%\newcommand{\dotcup}[1]{%
%\,\begin{tikzpicture}[dotpic,yshift=4mm]
%	\node [#1] (a) at (0,-0.6) {};
%	\draw [bend right,medium diredge] (-0.4,0) to (a);
%	\draw [bend left,medium diredge] (0.4,0) to (a);
%\end{tikzpicture}\,}

% this doesn't have a colour
%\newcommand{\tick}{%
%\,\,\begin{tikzpicture}[dotpic]
%	\node [style=none] (a) at (0,0.35) {};
%	\node [style=none] (b) at (0,-0.35) {};
%	\draw [dirtickedge] (a) -- (b);
%\end{tikzpicture}\,\,}

% these only make sense in black
%\newcommand{\lolli}{%
%\,\begin{tikzpicture}[dotpic,yshift=-1mm]
%	\path [use as bounding box] (-0.25,-0.25) rectangle (0.25,0.5);
%	\node [style=dot] (a) at (0, 0.15) {};
%	\node [style=none] (b) at (0, -0.25) {};
%	\draw [medium diredge] (a) to (b.center);
%	\draw [diredge, out=45, looseness=1.00, in=135, loop] (a) to ();
%\end{tikzpicture}\,}

%\newcommand{\cololli}{%
%\,\begin{tikzpicture}[dotpic]
%	\path [use as bounding box] (-0.25,-0.5) rectangle (0.25,0.5);
%	\node [style=none] (a) at (0, 0.5) {};
%	\node [style=dot] (b) at (0, 0) {};
%	\draw [diredge, in=-45, looseness=2.00, out=-135, loop] (b) to ();
%	\draw [medium diredge] (a.center) to (b);
%\end{tikzpicture}\,}

%\newcommand{\unit}{\dotunit{dot}}
%\newcommand{\counit}{\dotcounit{dot}}
%\newcommand{\mult}{\dotmult{dot}}
%\newcommand{\comult}{\dotcomult{dot}}

% BLACK DOTS
%\newcommand{\blackdot}{\dotonly{black dot}\xspace}
%\newcommand{\smallblackdot}{\smalldotonly{smalldot}\xspace}%NEW
%\newcommand{\blackunit}{\dotunit{black dot}\xspace}
%\newcommand{\blackcap}{\dotcap{black dot}\xspace}
%\newcommand{\blackcup}{\dotcup{black dot}\xspace}



%\newcommand{\tickunit}{\dottickunit{dot}}
%\newcommand{\tickcounit}{\dottickcounit{dot}}
%\newcommand{\dualiser}{\dotdualiser{dot}}
%\newcommand{\idualiser}{\dotidualiser{dot}}
%\newcommand{\threestate}{\dotthreestate{dot}}

%\newcommand{\blackobs}{\ensuremath{\mathcal O_{\!\smallblackdot}}\xspace}

% WHITE DOTS
%\newcommand{\whitedot}{\dotonly{white dot}\xspace}
%\newcommand{\smallwhitedot}{\smalldotonly{small white dot}\xspace}
%\newcommand{\whiteunit}{\dotunit{white dot}\xspace}
%\newcommand{\whitecounit}{\dotcounit{white dot}\xspace}
%\newcommand{\whitemult}{\dotmult{white dot}\xspace}
%\newcommand{\whitecomult}{\dotcomult{white dot}\xspace}
%\newcommand{\whitetickunit}{\dottickunit{white dot}\xspace}
%\newcommand{\whitetickcounit}{\dottickcounit{white dot}\xspace}
%\newcommand{\whitecap}{\dotcap{white dot}\xspace}
%\newcommand{\whitecup}{\dotcup{white dot}\xspace}

% GREEN DOTS
%\newcommand{\greendot}{\dotonly{green dot}}
%\newcommand{\greenunit}{\dotunit{green dot}}
%\newcommand{\greencounit}{\dotcounit{green dot}}
%\newcommand{\greenmult}{\dotmult{green dot}}
%\newcommand{\greencomult}{\dotcomult{green dot}}
%\newcommand{\greentickunit}{\dottickunit{green dot}}
%\newcommand{\greentickcounit}{\dottickcounit{green dot}}
%\newcommand{\greencap}{\dotcap{green dot}}
%\newcommand{\greencup}{\dotcup{green dot}}

%\newcommand{\whiteobs}{\ensuremath{\mathcal O_{\!\smallwhitedot}}\xspace}


% ALTERNATE WHITE DOTS
%\newcommand{\altwhitedot}{\dotonly{alt white dot}}
%\newcommand{\altwhiteunit}{\dotunit{alt white dot}}
%\newcommand{\altwhitecounit}{\dotcounit{alt white dot}}
%\newcommand{\altwhitemult}{\dotmult{alt white dot}}
%\newcommand{\altwhitecomult}{\dotcomult{alt white dot}}
%\newcommand{\altwhitetickunit}{\dottickunit{alt white dot}}
%\newcommand{\altwhitetickcounit}{\dottickcounit{alt white dot}}
%\newcommand{\altwhitecap}{\dotcap{alt white dot}}
%\newcommand{\altwhitecup}{\dotcup{alt white dot}}

% GRAY DOTS
%\newcommand{\graydot}{\dotonly{gray dot}\xspace}
%\newcommand{\smallgraydot}{\smalldotonly{small gray dot}\xspace}
%\newcommand{\grayunit}{\dotunit{gray dot}\xspace}
%\newcommand{\graycounit}{\dotcounit{gray dot}\xspace}
%\newcommand{\graymult}{\dotmult{gray dot}\xspace}
%\newcommand{\dgraymult}{\ddotmult{gray ddot}\xspace}
%\newcommand{\graycomult}{\dotcomult{gray dot}\xspace}
%\newcommand{\graytickunit}{\dottickunit{gray dot}\xspace}
%\newcommand{\graytickcounit}{\dottickcounit{gray dot}\xspace}
%\newcommand{\graycap}{\dotcap{gray dot}\xspace}
%\newcommand{\graycup}{\dotcup{gray dot}\xspace}

%\newcommand{\grayobs}{\ensuremath{\mathcal O_{\!\smallgraydot}}\xspace}


%\newcommand{\blacktranspose}{\ensuremath{{\,\blackdot\!\textrm{\rm\,T}}}}
%\newcommand{\whitetranspose}{\ensuremath{{\!\!\altwhitedot\!\!}}}
%\newcommand{\graytranspose}{\ensuremath{{\,\graydot\!\textrm{\rm\,T}}}}

%\newcommand{\whiteconjugate}{\ensuremath{{\!\!\altwhitedot\!\!}}}

% \newcommand{\spider}[4][dot]{\node [#1] (#2) at (0,0) {};
% \node [bn] (#2_d1) at (-1,1) {};
% \node [bn] (#2_d2) at (-0.5,1) {};
% \node [bn] (#2_dm) at (1,1) {};
% \node [bn] (#2_c1) at (-1,-1) {};
% \node [bn] (#2_c2) at (-0.5,-1) {};
% \node [bn] (#2_cn) at (1,-1) {};

% \node [anchor=west] at (#2_dm.east) {$#3$};
% \node [anchor=west] at (#2_cn.east) {$#4$};
% \node at (0.2,0.7) {\small{...}};
% \node at (0.2,-0.7) {\small{...}};

% \draw (#2)--(#2_d1) (#2)--(#2_d2) (#2)--(#2_dm);
% \draw (#2)--(#2_c1) (#2)--(#2_c2) (#2)--(#2_cn);}

%\newcommand{\circl}{\begin{tikzpicture}[dotpic]
%		\node [style=none] (a) at (-0.25, 0.25) {};
%		\node [style=none] (b) at (0.25, 0.25) {};
%		\node [style=none] (c) at (-0.25, -0.25) {};
%		\node [style=none] (d) at (0.25, -0.25) {};
%		\draw [in=45, out=135] (b.center) to (a.center);
%		\draw [in=135, out=225] (a.center) to (c.center);
%		\draw [in=225, out=-45] (c.center) to (d.center);
%		\draw [style=diredge, in=-45, out=45] (d.center) to (b.center);
%\end{tikzpicture}}

% \newcommand{\icircl}{\begin{tikzpicture}[dotpic]
% 	\node [circle,draw=black,inner sep=1pt] {\footnotesize\sf{}{$-$}};
% \end{tikzpicture}}

% \newcommand{\rtcircl}{\ensuremath{\sqrt{\begin{tikzpicture}[dotpic]
% 	\node [circle,draw=black,inner sep=1pt] {\tiny\sf\phantom{$-$}};
% \end{tikzpicture}}}}
% \newcommand{\rticircl}{\ensuremath{\sqrt{\begin{tikzpicture}[dotpic]
% 	\node [circle,draw=black,inner sep=1pt] {\tiny\bf\sf{}{$-$}};
% \end{tikzpicture}}}}

% \newcommand{\dcircl}{\begin{tikzpicture}[dotpic]
% 	\draw [use as bounding box,draw=none] (-0.15,-0.3) rectangle (0.15,0.3);
% 	\node [small dot] (0) {};
% 	\draw [uploop] (0) to ();
% 	\draw [downloop] (0) to ();
% \end{tikzpicture}}


==> macros/interpretations/preamble.tex <==
\oddsidemargin 10pt
\evensidemargin 10 pt
\topmargin -.5in
\headsep 20pt
\footskip 38pt
\textheight 8.9in
\textwidth 6.25in

\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}
\usepackage{hyperref}
\usepackage{amsmath,amssymb}
\usepackage{xspace}
\usepackage{color}
\usepackage{epsfig}
\graphicspath{{.}{./figures/}}
\pagestyle{headings}
\usepackage{keycommand}
\usepackage{macros/tikzfig}
\input{macros/defs.tex}
\input{macros/tikzstyles.tex}
\input{macros/tikzfigures.tex}
\def\bR{\begin{color}{red}}
\def\bB{\begin{color}{blue}}
\def\bM{\begin{color}{magenta}}
\def\bC{\begin{color}{cyan}}
\def\bW{\begin{color}{white}}
\def\bBl{\begin{color}{black}}
\def\bG{\begin{color}{green}}
\def\bY{\begin{color}{yellow}}
\def\e{\end{color}\xspace}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}\par\noindent}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}\par\noindent}
\newcommand{\bec}{\begin{center}}
\newcommand{\eec}{\end{center}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}\par\noindent}
\newcommand{\beqa}{\begin{eqnarray*}}
\newcommand{\eeqa}{\end{eqnarray*}\par\noindent}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}\par\noindent}
\newcommand{\TODOb}[1]{\marginpar{\scriptsize\bB \textbf{TODO:} #1\e}}
\newcommand{\TODOm}[1]{\marginpar{\scriptsize\bM \textbf{TODO:} #1\e}}
\newcommand{\TODOd}[1]{\marginpar{\scriptsize\bG \textbf{TODO:} #1\e}}
\newcommand{\COMMb}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMm}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMd}[1]{\marginpar{\scriptsize\bG \textbf{COMM:} #1\e}}
\newcommand{\Kon}[1]{\marginpar{\scriptsize\bM \textbf{Konment:} #1\e}}

\def\QiNLP{Q${}^i$NLP}

==> macros/interpretations/preamble2.tex <==
\oddsidemargin -15pt
\evensidemargin -15pt
\topmargin -.8in
\headsep 20pt
\footskip 38pt
\textheight 9.5in
\textwidth 6.95in

\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}
\usepackage{hyperref}
\usepackage{amsmath,amssymb}
\usepackage{xspace}
\usepackage{color}
\usepackage{epsfig}
\graphicspath{{.}{./figures/}}
\pagestyle{headings}
\usepackage{keycommand}
\usepackage{macros/tikzfig}
\input{macros/defs.tex}
\input{macros/tikzstyles.tex}
\input{macros/tikzfigures.tex}
\def\bR{\begin{color}{red}}
\def\bB{\begin{color}{blue}}
\def\bM{\begin{color}{magenta}}
\def\bC{\begin{color}{cyan}}
\def\bW{\begin{color}{white}}
\def\bBl{\begin{color}{black}}
\def\bG{\begin{color}{green}}
\def\bY{\begin{color}{yellow}}
\def\e{\end{color}\xspace}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}\par\noindent}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}\par\noindent}
\newcommand{\bec}{\begin{center}}
\newcommand{\eec}{\end{center}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}\par\noindent}
\newcommand{\beqa}{\begin{eqnarray*}}
\newcommand{\eeqa}{\end{eqnarray*}\par\noindent}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}\par\noindent}
\newcommand{\TODOb}[1]{\marginpar{\scriptsize\bB \textbf{TODO:} #1\e}}
\newcommand{\TODOm}[1]{\marginpar{\scriptsize\bM \textbf{TODO:} #1\e}}
\newcommand{\TODOd}[1]{\marginpar{\scriptsize\bG \textbf{TODO:} #1\e}}
\newcommand{\COMMb}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMm}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMd}[1]{\marginpar{\scriptsize\bG \textbf{COMM:} #1\e}}
\newcommand{\Kon}[1]{\marginpar{\scriptsize\bM \textbf{Konment:} #1\e}}

\def\QiNLP{Q${}^i$NLP}

==> macros/wavelogic/tikzstyles2.tex <==
% TiKZ style file generated by TikZiT. You may edit this file manually,
% but some things (e.g. comments) may be overwritten. To be readable in
% TikZiT, the only non-comment lines must be of the form:
% \tikzstyle{NAME}=[PROPERTY LIST]

% Node styles
\tikzstyle{red dot}=[fill=red, draw=black, shape=circle]
\tikzstyle{green dot}=[fill={rgb,255: red,0; green,131; blue,0}, draw=black, shape=circle]
\tikzstyle{new style 0}=[fill=white, draw=black, shape=circle]
\tikzstyle{dot}=[fill=white, draw=black, shape=circle, inner sep=1pt]

% Edge styles


==> text/cats.tex <==
%\input{macros/interpretations/defs0} 

\chapter{\label{cats}Symmetric Monoidal Categories}

This section is adapted from the book~\cite{CKbook}. %All the definitions quoted in this appendix, along with additional exposition, can be found in the book~\cite{CKbook}.

From a category-theoretic perspective, a process theory is a \textit{strict symmetric monoidal category}. Essentially, this is a symbolic way to axiomatise series composition $\circ$ and parallel composition $\otimes$. First we define a strict monoidal category.

\begin{definition}\cite{CKbook}
	``A \textit{strict monoidal category} $\mathcal{C}$ consists of:	
	\begin{itemize}
	\item a collection ob($\mathcal{C}$) of \textit{objects}
	\item for every pair of objects $A$, $B$, a set $\mathcal{C}$($A$, $B$) of \textit{morphisms}
	\item for every object $A$, a special identity morphism: $1_A \in \mathcal{C}(A, A)$
     \item a sequential composition operation for morphisms:  $\circ : \mathcal{C}(B, C) \times \mathcal{C}(A, B) \rightarrow \mathcal{C}(B, C)$
	\item a parallel composition operation for objects: $\otimes : \text{ob}(\mathcal{C}) \times \text{ob}(\mathcal{C}) \rightarrow \text{ob}(\mathcal{C})$ 
	\item a unit object: $I \in \text{ob}(\mathcal{C})$
	\item and a parallel composition operation for morphisms: \[\otimes : \mathcal{C}(A, B)  \times \mathcal{C}(C, D)  \rightarrow \mathcal{C} (A \otimes C , B \otimes D)\]
      \end{itemize}
satisfying the following conditions:
\begin{itemize}
\item $\otimes$ is associative and unital on objects: $(A \otimes B) \otimes C = A \otimes (B \otimes C); A\otimes I = A = I \otimes A$
\item $\otimes$ is associative and unital on morphisms: $(f \otimes g) \otimes h = f \otimes (g \otimes h); f\otimes 1_I = f = 1_I \otimes f$
\item $\circ$ is associative and unital on morphisms: $(h \circ g) \circ f = h \circ (g \circ f); 1_B \circ f = f = f \circ 1_A$
\item $\otimes$ and $\circ$ satisfy the \textit{interchange law}: $
(g_1 \otimes g_2) \circ (f_1 \otimes f_2) = (g_1 \circ f_1) \otimes (g_2 \circ f_2)$''
\end{itemize}
\end{definition}

Compare the above definition with the definition of process theory in Chapter \ref{chapinterpretations1} (Def. \ref{def:ProcTheor}). \textit{Types} or \textit{system-types} in process theory correspond to \text{objects} in category theory; \textit{processes} correspond to \textit{morphisms}. The set $\mathcal{C}$($A$, $B$) therefore should be considered the set of all processes with input type $A$ and output type $B$. A member of this set can be denoted by either $f \in \mathcal{C}(A, B)$ or $f: A \rightarrow B$. A collection of such sets with sequential composition gives a \textit{category}. A \textit{monoidal category} is a category with both sequential and parallel composition. The `strict' part of the above definition will be explained shortly. Adding a swap morphism to a monoidal category makes it symmetric. 

%\textcolor{red}{revise above.}

%\textcolor{red}{more definitions and explanation}

\begin{definition}\cite{CKbook}
	``A \textit{strict symmetric monoidal category} is a strict monoidal category with a \textit{swap morphism}: $\sigma_{A, B} : A \otimes B \rightarrow B \otimes A$
	defined for all objects $A$, $B$, satisfying:
	\[
	\sigma_{B, A} \circ \sigma_{A, B} = 1_{A \otimes B} \quad \quad \quad \sigma_{A, I} = 1_A 
	\]
	\[
	(f \otimes g) \circ \sigma_{A, B} = \sigma_{B', A'} \circ (g \otimes f) 
	\]
	\[
	(1_B \otimes \sigma_{A, C}) \circ (\sigma_{A, B} \otimes 1_C) = \sigma_{A, B \otimes C}"
	\]
\end{definition}
A monoidal category is called strict when $\otimes$ is associative and unital exactly. On the other hand, in the non-strict monoidal category, associativity and unitality of $\otimes$ are isomorphisms rather than identities.

\begin{definition}\cite{CKbook}
	``An object $A$ is \textit{isomorphic} to an object $B$, denoted $A \cong B$
	if and only if there exists a pair of morphisms:
	\[
	f : A \rightarrow B \quad \quad \quad  f^{-1} : B \rightarrow A
	\]
	such that:
\[
	f^{-1} \circ f = 1_A \quad \quad \quad f \circ f^{-1} = 1_B
\]
	The morphism $f$ is then called an \textit{isomorphism}.''
\end{definition}

Non-strict monoidal categories are the more common species of monoidal categories. Their unitality and associativity of parallel composition are isomorphisms rather than identities:
\[
(A \otimes B) \otimes C \cong A \otimes (B \otimes C) \quad \quad \quad A \otimes I \cong A \cong I \otimes A
\]
These are called \textit{structural isomorphisms} and must be included in the definition of a category in order to define non-strict monoidal category. Additionally, a number of equations, called \textit{coherence equations} must be added to the definition to ensure that the behaviour of structural isomorphisms is sensible when they are composed. The following theorem gives the relation between strict and non-strict (symmetric) monoidal categories.

\begin{theorem}[Coherence theorem]\cite{CKbook}
	``Every (symmetric) monoidal category $\mathcal{C}$  is equivalent to a strict (symmetric) monoidal category $\mathcal{C'}$.''
\end{theorem}

Equivalence between two categories mean that they are the same for all practical purposes. The above theorem justifies considering $(A \otimes B) \otimes C$, $A \otimes (B \otimes C)$ and $A \otimes B \otimes C$ the same. In other words, we don't need to worry about parentheses in associativity of $\otimes$. Likewise, the theorem justifies considering $A \otimes I$, $A$ and $I \otimes A$ the same.

Finally, the following theorem justifies using string diagrams for symmetric monoidal categories. 

\begin{theorem}\cite{CKbook}
	``[String] diagrams are sound and complete for symmetric monoidal categories. That is, two morphisms $f$ and $g$ are provably equal using the equations of a symmetric monoidal category if and only if they can be expressed as the same [string] diagram.''
\end{theorem}

This appendix can be summarised as the following correspondence. 
\[
\text{string diagrams} \leftrightarrow \text{process theory} \leftrightarrow \text{symmetric monoidal category}
\]
 


%\textcolor{red}{revise above and add details.}

%\textcolor{red}{double check all definitions}

%\textcolor{red}{examples?}

%\textcolor{red}{quote or italicise?}

%\textcolor{red}{relate with definition of process theory in interpretation chapters}

==> text/interpretations2.tex <==
%\input{macros/interpretations/defs0} 

\chapter{\label{chapinterpretations2}Interpreting Quantum Physics Diagrammatically}

\epigraph{`David Mermin once summarized a popular attitude towards quantum theory as ``Shut up and
	calculate!''. We suggest a different slogan: ``Shut up and contemplate!'''}  
{Lucien Hardy and Robert Spekkens, 2010~\cite{hardy2010physics}}

In this chapter, we shall use categorical quantum mechanics (CQM) as a lens through which to study a number of mainstream interpretations of non-relativistic quantum theory. Our focus will be on \textit{ontological} interpretations of \textit{quantum theory}. Therefore, we shall discuss neither \textit{epistemic} interpretations like QBism~\cite{caves2002quantum, healey2016quantum} nor \textit{foil theories} like Spekken's toy model~\cite{spekkens2007evidence, coecke2011phase, spekkens2016quasi}.\footnote{For Spekken's toy bit theory, there exists a complete graphical calculus~\cite{backens2016complete}.}
		%Spekken's toy theory. Miriam Backens' article on complete calculus for Spekken's toy theory. Read the intro.
		%just talk briefly about its existence and graphical formalism and how it compares with regular quantum. }} 

Historically, the interpretations\footnote{Strictly speaking, not all of them are interpretations because they do not merely interpret the same fixed formalism but also change the mathematical structure of the theory. Therefore, these `interpretations' are in fact different theories~\cite{freire2022oxford}. However, in keeping with convention, we shall refer to these as `interpretations'} of quantum theory were developed to solve some fundamental problems in quantum theory, most importantly the measurement problem. It was von Neumann's formulation of quantum theory~\cite{vonNeumann1932quantenmechanik} that provided the backdrop for the development of these interpretations. The conceptual paradigm underlying the standard formulation is one in which theories are fundamentally about specifying states of physical systems and tracking their dynamics or evolution. 
%Today, there exist many different reconstructions of quantum theory~\cite{hardy2001quantum, dakic2009quantum, hardy2012operator, masanes2011derivation, chiribella2011informational, hohn2017quantum, selby2021reconstructing, tull2020categorical, westerbaan2022computer}, which derive the standard quantum formalism from a set of physical postulates that one finds reasonable. Therefore, one is offered different directions in the quantum interpretation programme. One may interpret the standard formalism (which is what has been the focus of quantum interpretations till date). Alternatively, one may pick a reconstruction and interpret its postulates, as advocated by Goyal~\cite{goyal2022role}. Still another option is taking the essential ideas of the traditional interpretations of quantum theory and expressing them in a different formulation of quantum theory.
As an alternative formulation of quantum theory, CQM is rooted in a different conceptual paradigm in which theories specify processes and how they compose~\cite{coecke2011universe}. %This line of inquiry is partly motivated by the question: what would interpretations of quantum theory look like if their starting point was CQM rather than textbook quantum theory? 
According to this approach, physical reality is fundamentally about processes, their interaction and composition. Now that there exists an alternative to the standard formulation, there is an opportunity to revisit the traditional interpretations of quantum theory within this new formulation. 

An interpretation is not merely a prescription about how to understand and use the formalism of quantum theory. Rather, it foregrounds certain aspects of the theory at the expense of others, and hence offers up its own conceptual scaffolding to the way we think about quantum physics---particularly its structure and ontology. In principle, one should be able to express the key aspects of any interpretation within CQM. This is what we attempt in this chapter. %we present a few interpretations of quantum theory within the diagrammatic language of CQM. 

%CQM offers precisely such an opportunity. In this chapter and next, my aim is to demonstrate that CQM can be used as a canvas for interpretations of quantum theory. 
CQM is essentially neutral regarding the specific interpretation we apply it to, as it is, in principle, compatible with all of them. Using CQM for interpretations provides multiple advantages. Firstly, it provides an alternative, compositional lens to study, compare and evaluate quantum interpretations on a common ground or equal footing. %The different notions of quantum measurement and interpretations of quantum theory can be compared with respect to the varied levels of structural complexity involved in them. 
Secondly, one can carry out standard quantum mechanical calculations with the tools of CQM---computational and conceptual---within the framework of a specific interpretation of quantum theory. %The computational and conceptual benefits of CQM are naturally included. 
Thirdly, it provides a new conceptual way to think of the quantum world and interpretations -- \emph{i.e.} in terms of processes and their composition rather than in terms of entities and their evolution. %Perhaps, most importantly, this approach can help bridge the various strands of work in quantum foundations, in particular emphasising that picturalism/compositionality is itself a framework for reasoning about interpretations of quantum theory, even though it does not aim to `solve the measurement problem'.

At the outset, we offer two clarifications. First, we are not developing new graphical calculi for interpretations of quantum theory. Second, we are not claiming to offer definitive graphical versions of the various interpretations. These interpretations are evolving research areas~\cite{knox2022routledge, freire2022oxford} in their own right. %and their proponents disagree on key ideas, leading to different variants of a particular interpretation. We encourage the practitioners and proponents of these interpretations to explore both these lines of inquiry.
Rather, our work takes the first steps in expressing the postulates and essential ideas of these interpretations in the diagrammatic language offered by CQM. Through examples, we also show how diagrammatic reasoning and calculations can be performed within CQM versions of these interpretations. We start with a description of textbook or orthodox quantum theory, sometimes called `the Copenhagen interpretation'\footnote{The Copenhagen interpretation is a set of ideas -- such as complementarity, wave-particle duality, the completeness of quantum theory, collapse of the wavefunction due to measurement, and the essential role of observers in measurement -- usually attributed to Niels Bohr (and people associated with his institute in Copenhagen)~\cite{howard2022copenhagen}, but were actually popularised by Werner Heisenberg in the 1950s~\cite{howard2004invented}. In fact, there is no single `Copenhagen interpretation' since the views of the key figures usually associated with the interpretation differed strongly concerning the validity of the aforementioned ideas~\cite{howard2004invented, howard2022copenhagen}.} and offer a representation of it in CQM. This is used as a segue into the measurement problem and a characterisation of its `solutions' in terms of interpreting or modifying textbook quantum theory. Next, we look at the EPR-Bell-type scenario in textbook quantum theory, setting the stage to compare and contrast other interpretations.

Our general strategy is to look at the interpretations in terms of how they describe measurements for single and bipartite systems such as those in the EPR-Bell scenario, and provide a corresponding representation in CQM. We shall make frequent use of the definitions and tools developed in the previous chapter. The interpretations we discuss include textbook quantum theory, consistent histories~\cite{schlosshauer2005decoherence}, relational quantum mechanics~\cite{rovelli1996relational, rovelli2021relational}, Everettian quantum mechanics~\cite{everett1957relative}, and hidden variable models.

% (including de-Broglie-Bohm-like theories~\cite{bohm1952suggested, bohm1952suggestedii}, a hidden measurement theories [], superdeterminisitic theories~\cite{hossenfelder2020rethinking, hossenfelder2020superdeterminism, hance2022does}), and stochastic theories.

\section{Textbook Quantum Mechanics}\label{secTQM}

Here, we describe the postulates (numbered \textbf{P1-P5}) of textbook or orthodox quantum theory\footnote{This may also be called von Neumann's formulation of quantum theory as it was presented in his monograph~\cite{vonNeumann1932quantenmechanik}.} and provide their representation within CQM. In most textbooks, \textit{pure-state quantum theory} is considered primary while \textit{mixed-state quantum theory} is considered secondary or derivative. We start with pure-state quantum theory.

\textbf{P1.} \textit{A quantum system is completely specified by its state} $\ket{\psi}$ \textit{up to a global phase} $\alpha$ \textit{in a Hilbert space} $\mathcal{H}$.

\noindent Diagrammatically, this quantum state is represented as
\begin{equation}\label{copen2}
	e^{i \alpha}\ \tikzfig{interpretations/copenhagen0b}
\end{equation}
 
\textbf{P2.} \textit{The observables of the system are given by Hermitian operators (\textit{i.e.} self-adjoint linear operators) acting on the states and the results of measurement are given by their eigenvalues.}

\noindent Diagrammatically, a self-adjoint linear map is obtained by defining the map
\begin{equation}\label{copen6}
\map{f} \ := \  \sum_i r_i \map{P^i}
\end{equation}
where $\{P^i\}_i$ are mutually orthogonal projectors and the numbers $\{r_i\}_i$ associated with the projectors are distinct and real numbers, called \textit{eigenvalues}.\footnote{For clarity, we discuss only ONB measurements here. In more general von Neumann measurements, some of the eigenvalues may be repeated.}  

\begin{remark}
von Neumann measurements should be at the heart of von Neumann's formulation of quantum theory. At first glance, the map $f$ in Eq. (\ref{copen6}) looks different from a von Neumann measurement as defined in CQM. However, on closer inspection, it is not that different. By the spectral theorem~\cite{CKbook}, for some orthonormal basis (ONB) $\ket{i}$, we have
\[
\map{f} \ = \  \sum_i r_i  \tikzfig{interpretations/copenhagen0c}
\]
using which the projectors $\{P^i\}_i$ can be recovered. These projectors make a non-demolition von Neumann ONB measurement~\cite{CKbook}
\begin{equation}\label{copen4}
	\left(\dmap{\widehat P^i}\right)^i  \ := \  \left(\tikzfig{interpretations/copenhagen2b}\right)^i
\end{equation}
%as described in the previous chapter. %A special case of von Neumann measurement is a non-demolition ONB measurement, the projectors of which are given by
%\begin{equation}\label{copen3}
%\left(\dmap{\widehat P^i}\right)^i \ = \  \left(\tikzfig{interpretations/copenhagen2b}\right)^i
%\end{equation}
where $\left\{\tikzfig{interpretations/copenhagen0d}\right\}_i$ are the corresponding eigenstates.  

Therefore, from the perspective of CQM, the map $f$ should be understood as one specific representation of the actual processes—namely, the mutually orthogonal projectors.  
\end{remark}

\textbf{P3.} \textit{In the absence of measurement, the state evolves in a deterministic, reversible manner; that is, via unitary evolution}. %(which can be tracked by the Schrodinger equation \textcolor{red}{should we mention it?}).}

\noindent Diagrammatically, a unitary evolution $U$ is represented as
\begin{equation}\label{copen5b}
	\map{U}
\end{equation}

\textbf{P4a.} \textit{When a measurement is performed, the state of the system irreversibly collapses to one of the eigenstates of the observable. }

\noindent Diagrammatically, if a state $\ket{\psi}$ is subjected to a measurement given by the observable (\ref{copen6}), its collapse to the $i$ eigenstate is given by
\begin{equation}\label{copen7}
	\sqrt{\frac{1}{\scalebox{0.6}{\tikzfig{interpretations/copenhagen4d}}}} \ \  \tikzfig{interpretations/copenhagen30bz}
\end{equation}

%In CQM, one of the projectors from the list (\ref{copen4}) is applied to the state (\ref{copen1}) as a result of measurement:
%\begin{equation}\label{copen7}
%\frac{1}{\scalebox{0.6}{\tikzfig{interpretations/copenhagen3}}} \  \tikzfig{interpretations/copenhagen30b}
%\end{equation}
%This projector is the doubled version of the one from postulate (\textbf{P2}); see Eq. (\ref{copen5}).
%\[
%\tikzfig{interpretations/copenhagen20}
%\]    

\textbf{P4b.} \textit{The probability of the measurement outcome is given by the Born rule.}

\noindent Diagrammatically, the Born rule is represented as
\begin{equation}\label{p4born}
		P(i | \ket{\psi}) \ = \ \tikzfig{interpretations/copenhagen4d} 
\end{equation}
which is $\braket{\psi|P^i|\psi}$ in the Dirac notation.

Using sliding, we can express the Born rule as a traced diagram: 
\begin{equation}
	P(i | \ket{\psi}) \ = \ \tikzfig{interpretations/copenhagen4e} 
\end{equation}
which is $\text{Tr}(P^i \ket{\psi} \bra{\psi})$ in the Dirac notation.

\textbf{P5.} \textit{The composite state of two quantum systems corresponding to Hilbert spaces $\mathcal{H}_1$ and $\mathcal{H}_2$ is given by the tensor product $\ket{\psi}_1 \otimes \ket{\psi}_2$ up to a global phase $\phi$, where $\ket{\psi}_1 \in \mathcal{H}_1$ and $\ket{\psi}_2 \in \mathcal{H}_2$.}

\noindent Diagrammatically, the tensor product according to this postulate is given by 
\begin{equation}\label{singten}
	e^{i \phi}\ \tikzfig{interpretations/copenhagen0f}
\end{equation}
%whereas the corresponding tensor product in CQM is
%\[
%\tikzfig{interpretations/copenhagen0e}
%\]  

In mixed-state quantum theory, instead of pure states and von Neumann measurements, we use the more general concepts of density matrices and positive operator-valued measure (POVM) measurements.

A general density matrix is represented by 
\begin{equation}\label{densmat}
\dkpoint{\boldsymbol\rho} \ := \  \tikzfig{interpretations/densitymat1} 
\end{equation}
where $g$ is a linear map. A density matrix is a process in a doubled Hilbert space $ \mathcal{H} \otimes \mathcal{H}$. The doubled version of the quantum state (\ref{copen2}) is a special case of the density matrix:
\begin{equation}\label{copen1}
	\tikzfig{interpretations/doubledstate} 
	%\tikzfig{interpretations/copenhagen0} \ := \ 
\end{equation}
which we symbolically represent as $\widehat{\psi}$. Notice that the global phase is eliminated by doubling.
Likewise, the doubled version of the tensor product (\ref{singten}) is
\[
\tikzfig{interpretations/copenhagen0e}
\]  
%In CQM, the corresponding description is that the state of a quantum system is the following process in the doubled Hilbert space $ H \otimes H$.
%\begin{equation}\label{copen1}
%	\tikzfig{interpretations/copenhagen0}
%\end{equation}
%which we symbolically represent as $\widehat{\psi}$. Notice that this diagram is not a literal reading of postulate (\textbf{P1}), according to which the state is: %$\widehat{\psi}_1 \otimes \widehat{\psi}_2$:
%\begin{equation}\label{copen2}
%	\tikzfig{interpretations/copenhagen0b}
%\end{equation}

\noindent The doubled version of the unitary map (\ref{copen5b}), $\widehat{U}$ acts on states in doubled Hilbert spaces.
\begin{equation}\label{copen5}
	\tikzfig{interpretations/doubledU1}  %\dmap{\widehat U} 
\end{equation}
%in contrast with the single unitary map $U$ in postulate (\textbf{P3}).

\noindent In the doubled version of the collapse postulate (\textbf{P4}), one of the projectors from the list (\ref{copen4}) is applied to the state (\ref{copen1}) as a result of measurement:
\begin{equation}\label{copen7}
	\frac{1}{\scalebox{0.6}{\tikzfig{interpretations/copenhagen3}}} \  \tikzfig{interpretations/copenhagen30b}
\end{equation}
%This projector is the doubled version of the one from postulate (\textbf{P2}); see Eq. (\ref{copen5}).

A demolition POVM measurement is given by
\begin{equation}\label{povmcop}
\left( \tikzfig{interpretations/povm} \right)^i = \left( \tikzfig{interpretations/povm2} \right)^i 
\end{equation}
where $\{\widehat f_i\}_i$ is a family of pure quantum maps. For the state (\ref{densmat}), the Born rule (Eq. (\ref{bornrule})) for POVM gives the probability of occurrence of the measurement outcome $i$ as follows:
\begin{equation}\label{copen8b}
		P(i | \boldsymbol \rho) \ = \ \tikzfig{interpretations/bornpovm1} \ = \ \tikzfig{interpretations/bornpovm0} \ = \ \tikzfig{interpretations/bornpovm2} \ = \  \tikzfig{interpretations/bornpovm3}  \  = \  \tikzfig{interpretations/bornpovm4} %\ = \ \tikzfig{interpretations/copenhagen4d} 
\end{equation}
where after un-doubling the diagram, we have used sliding and the definitions $\ \map{E^{i}} \ := \ \tikzfig{interpretations/bornpovm5}\ $ and $\ \map{\tilde{\rho}} \ := \ \tikzfig{interpretations/bornpovm6}$.\footnote{We use the symbol $\tilde{\rho}$ for the density operator in the standard formulation, which corresponds to $\boldsymbol \rho$ in our doubled version of CQM. The two can be translated into each other using the process-state duality. \[\dkpoint{\boldsymbol\rho} \ = \  \tikzfig{interpretations/densitymat1} \ \longleftrightarrow \ \ \map{\tilde{\rho}} \ = \ \tikzfig{interpretations/bornpovm6} \]} In the usual algebraic notation, Eq. (\ref{copen8b}) is $P(i | \boldsymbol \rho) = \text{Tr}(E_i \tilde{\rho})$.

A demolition von Neumann ONB measurement is a special case of the POVM measurement (\ref{povmcop}). 
\begin{equation}
	\left( \tikzfig{interpretations/onbcop1} \right)^i = \left( \tikzfig{interpretations/onbcop2} \right)^i 
\end{equation}
The Born rule (Eq. (\ref{copen8b})) becomes
\begin{equation}\label{copen8c}
		P(i | \boldsymbol \rho) \ = \ \tikzfig{interpretations/bornpovm1b} \ = \ \tikzfig{interpretations/copenhagen3d} \ = \  \tikzfig{interpretations/bornpovm2b} \ = \  \tikzfig{interpretations/bornpovm3b}  = \  \tikzfig{interpretations/bornpovm4b}
\end{equation}
where after un-doubling the diagram, we have used sliding, and the fact that $P^i$ is a projection.

\noindent For the special case of a pure state $\ket{\psi}$, the Born rule (Eq. \ref{copen8c}) becomes 
\begin{equation}\label{copen8}
		P(i | \ket{\psi}) \ = \ \tikzfig{interpretations/bornpovm1c} \ = \ \tikzfig{interpretations/copenhagen3} \ = \  \tikzfig{interpretations/copenhagen4} \ = \  \tikzfig{interpretations/copenhagen4d2}  \ = \ \tikzfig{interpretations/copenhagen4d} 
\end{equation}
which recovers Eq. (\ref{p4born}).
%\textcolor{red}{is sliding mentioned earlier?}
%The last diagram of Eq. (\ref{copen8}) in Dirac notation is $\braket{\psi|P^i|\psi}$, which is the Born rule in postulate (\textbf{P4b}).

%Using sliding again, we can express the Born rule as a traced diagram: 
%\begin{equation}\label{copen9}
%	P(i | \ket{\psi}) \ = \ \tikzfig{interpretations/copenhagen4e} 
%\end{equation}
%which in Dirac notation is $\text{Tr}(P^i \ket{\psi} \bra{\psi})$, again in %agreement with postulate (\textbf{P4b}).

\begin{example}[Unitary evolution followed by ONB measurement]
	
A state (\ref{copen1}) that undergoes unitary evolution (\ref{copen5}) and is then subjected to an ONB measurement giving the outcome $i$ (\ref{copen4}) is %diagrammatically represented as		
	\[
  \tikzfig{interpretations/copenhagen2}
	\]    
meaning the state $\ \tikzfig{interpretations/copenhagen0}\ $ is measured as, or collapses to, $\ \tikzfig{interpretations/copenhagen0d}\ $, \textit{i.e.,} one of the eigenstates of the ONB. The probability of this measurement outcome is given by	
	\[
	P \left(i | \ U \ket{\psi} \right) %\ \ = \ \  \tikzfig{interpretations/copenhagen5} 
	\ \ = \ \ \tikzfig{interpretations/copenhagen5b} 
	\]	
	\noindent which in Dirac notation is $\overline{\braket{\psi|U|i}} \braket{\psi|U|i} = |\braket{\psi|U|i}|^2$.
\end{example}

\begin{remark}
A benefit of defining a Hermitian operator (as in Eq. (\ref{copen6})) for an observable is that the \textit{expectation value} or \textit{mean} of the observable can be calculated~\cite{CKbook}. If the eigenvalues in Eq. (\ref{copen6}) are physical quantities, such as spin or polarisation, associated with the projectors, the mean is given by replacing $P^i$ in Eq. (\ref{copen8}) with $f$ from Eq. (\ref{copen6}): 
\begin{equation}\label{copen10}
	E_{f} (\ket{\psi}) \ \ := \ \ \tikzfig{interpretations/copenhagen4f}  \ \  = \ \  \sum_i r_i  \ \tikzfig{interpretations/copenhagen4d}  
\end{equation}
In Dirac notation, it corresponds to $\braket{\psi | f |\psi}$. $E_{f} (\ket{\psi})$ is not a probability but a weighted average of the eigenvalues $r_i$. The quantity $E_{f} (\ket{\psi})$ gives the average value of the measurement outcomes corresponding to the observable $f$ if the same measurement is performed on identically prepared systems $\ket{{\psi}}$.
\end{remark}

Textbook quantum theory gives a privileged status to unitary evolution (\ref{copen5}) and von Neumann measurements (\ref{copen4}). However, unitary maps and von Neumann measurements alone do not form a \textit{process theory}~\cite{CKbook}; \emph{i.e.}, they are not compositionally closed, as explained in the remark below.

\begin{remark}\label{privilegeunitary}
Composing a unitary process and a state in parallel	
\[
\dmap{\widehat U} \ \tikzfig{interpretations/copenhagen0}
\]
does not yield a unitary or a state. It is an isometry. 	

Series or parallel composition of a (non-demolition) von Neumann measurement and a unitary yield neither a von Neumann measurement nor a unitary:
\[
\left(\dmap{\widehat P^i} \  \dmap{\widehat U}  \right)^i   \quad \quad \quad \left( \tikzfig{interpretations/copenhagen6}  \right)^i 
\]
Indeed, even composing two von Neumann measurements in series does not generally give a von Neumann measurement:
\[
 \left( \tikzfig{interpretations/copenhagen7}\right)^{ij} 
\]
unless the two measurements commute~\cite{CKbook}.

The emphasis on unitarity is justified by some physicists using the Stinespring dilation (see Remark \ref{stinespringrem}): any causal process arises from a unitary process, a pure state, and discarding. 
\end{remark}

%\textcolor{red}{Stinespring for CP channels rather than causal. See Sean comments}

%\begin{remark}
%	using doubled stuff etc...
%\end{remark}

%\textcolor{red}{Important: pure state quantum mechanics in this chapter? clarify at the beginning. Maybe just in Textbook QM}

%\textcolor{red}{notes here}        

%\[\includegraphics[width=0.8\linewidth]{figures/b3.jpg}\]

%\[\includegraphics[width=0.8\linewidth]{figures/b4.jpg}\]

%\[\includegraphics[width=0.8\linewidth]{figures/b5.jpg}\]

\begin{convention}
	From this point onwards, we shall ignore non-zero scalar factors in diagrammatic expressions, equations and calculations. Therefore, the equality sign `$=$' should be interpreted as `equal up to a global non-zero scalar'.
\end{convention}

\section{The Measurement Problem}

Generally speaking, two kinds of dynamics are involved in textbook quantum mechanics. The evolution of the quantum state is unitary in the absence of measurement; but as soon as a measurement takes place, there is an instantaneous, irreversible `collapse' of the state. The postulates of quantum theory do not clearly describe what constitutes a measurement, what a measuring device or object is, and, most importantly, why there are two kinds of dynamics. This is called the measurement problem~\cite{norsen2017foundations}.

To motivate a systematic discussion of interpretations, we provide another description of the measurement problem, following Ref.~\cite{maudlin1995three}. The measurement problem is defined as the incompatibility between the following three claims of quantum theory:

\textbf{MP1.} The state specifies all the physical properties of the system. 

\textbf{MP2.} The state always evolves according to a linear, deterministic dynamical equation, \emph{i.e.,} the Schr\"{o}dinger equation.

\textbf{MP3.} Measuring the state of a system always yields definite outcomes.

One can see that \textbf{MP2} and \textbf{MP3} correspond to postulates \textbf{P3} and \textbf{P4} of textbook quantum theory. The mainstream interpretations of quantum theory reject one of the claims \textbf{MP1-3}. 

\subsection{Solving the Measurement Problem}

Interpretations of quantum theory that reject \textbf{MP1} are usually called hidden variable theories or additional variable theories, because they supplement the quantum states with additional physical variables to completely characterise quantum systems. The most popular example of a hidden variable theory was proposed by David Bohm~\cite{bohm1952suggested, bohm1952suggestedii}. Later, we shall discuss two variants of hidden variable theories %(Bohm-like and superdeterministic~\cite{hossenfelder2020superdeterminism, hossenfelder2020rethinking}), 
as well as two kinds of hidden measurement theories. In the latter, the hidden variables are added to the measurement process rather than the state.  

Interpretations that reject \textbf{MP2} are called collapse or non-linear theories~\cite{ghirardi2002collapse}. An important example of such interpretations is the spontaneous collapse theory by Ghirardi, Rimini and Weber (GRW)~\cite{ghirardi1986unified, ghirardi2002collapse}, which modifies the Schr\"{o}dinger equation by adding stochastic and non-linear terms to it. We shall not analyse GRW theory since it is non-linear and our scope is limited to linear maps between Hilbert spaces. We shall, however, discuss stochastic interpretations of quantum theory such as the consistent histories interpretation~\cite{griffiths2009consistent, griffiths2014consistent}. 

Interpretations that reject \textbf{MP3} may be called unitary quantum mechanics. A typical example is the many worlds interpretation~\cite{vaidman2002many, wallace2012emergent}, which was spawned by Hugh Everrett's relative-state interpretation of quantum mechanics~\cite{everett1957relative}. In the many worlds interpretation, when a measurement is performed, each outcome of the measurement is realised but in a different world. Another reading of Everett's interpretation gave rise to the relational interpretation~\cite{rovelli1996relational, rovelli2021relational}, in which a quantum system may have different states with respect to different systems. Note that the relational interpretation does not reject \textbf{MP3} but \textbf{MP1}, in the sense that the state of a system is relational and requires the reference of another system. We shall discuss the many worlds interpretation (restricted to Everett's formulation) and relational quantum mechanics in this chapter. 

%\textcolor{red}{How is measurement problem dissolved in cqm}

%\textcolor{red}{is the measurement problem dissolved because preparations, tests and other process are put on similar footing?}

\subsection{Dissolving the Measurement Problem}\label{secdissolv}

%The measurement problem is a pathological feature of standard quantum theory. Even after so much research effort into developing the interpretations of quantum theory to date, there is barely any consensus on whether the measurement problem is solved or if it is, which interpretation solves it in a convincing manner~\cite{schlosshauer2011elegance, freire2022oxford}. The number of interpretations keeps increasing.\footnote{According to Mermin, "Quantum mechanics is the most useful and powerful theory physicists have ever devised. Yet today, nearly 90 years after its formulation, disagreement about the meaning of the theory is stronger than ever. New interpretations appear every year. None ever disappear."~\cite{mermin2012commentary}} The interested reader is referred to surveys aimed at providing an exposition, classification and comparison of these interpretations~\cite{belinfante1973survey, jammer1974philosophy, dickson1998quantum, bub1999interpreting, cabello2017interpretations, adlam2023taxonomy}. Perhaps, this situation calls for another approach to addressing the measurement problem. Instead of sticking to the conceptual framework in which physical theories describe particles and their trajectories, one ought to entertain the possibility of a framework in which physical theories describe processes and how they compose and interact.

%We contend that this framework \textit{dissolves} the measurement problem. In other words, quantum theory is not a theory of quantum objects and their trajectories, but it is about quantum processes and how they compose. If we let go of our commitment to objects-and-dynamics-first view of physical theories, we do not have to worry about two kinds of dynamics in quantum theory; in other words, there is no measurement problem left. Perhaps that is the lesson of quantum theory and the measurement problem. CQM offers a formulation of quantum theory in such a process-relational and compositional framework. In CQM, the mode of explanation is not in terms of systems and their dynamics but in terms of processes and their composition.


The measurement problem is a pathological feature of standard quantum theory. Despite extensive research efforts into developing interpretations of quantum theory, there is no consensus on whether the measurement problem has been solved, or if it has, how~\cite{schlosshauer2011elegance, freire2022oxford}. Indeed, the number of interpretations continues to increase~\cite{belinfante1973survey, jammer1974philosophy, dickson1998quantum, bub1999interpreting, cabello2017interpretations, adlam2023taxonomy}.\footnote{According to Mermin, "Quantum mechanics is the most useful and powerful theory physicists have ever devised. Yet today, nearly 90 years after its formulation, disagreement about the meaning of the theory is stronger than ever. New interpretations appear every year. None ever disappear."~\cite{mermin2012commentary}}
In light of this, perhaps this situation calls for a different approach to addressing the measurement problem. Instead of adhering to a conceptual framework in which physical theories describe particles and their trajectories, we might entertain the possibility of a framework in which physical theories describe processes and how they compose and interact.

CQM offers a formulation of quantum theory in such a process-relational and compositional framework that, we contend, \textit{dissolves} the measurement problem. In other words, if we cast quantum theory as a theory of quantum processes and how they compose, rather than a theory of quantum objects and their trajectories, we no longer need to grapple with the dual dynamics in quantum theory, and the measurement problem ceases to exist. %Perhaps this is the true lesson of quantum theory and the measurement problem.  %In CQM, the mode of explanation is not in terms of systems and their dynamics but rather in terms of processes and their composition.
\section{The EPR-Bell scenario}

In this section, we discuss the Einstein-Podolsky-Rosen(EPR)-Bell scenario~\cite{einstein1935can, bell1964einstein}, in which a bipartite entangled system is shared between Alice and Bob who perform local measurements. Correlations between Alice's and Bob's measurement outcomes violate the Bell inequalities~\cite{bell2004speakable, scarani2019bell}, ruling out local hidden variable theories. In other words, the experiments demonstrate that quantum physics is non-local. 

The original motivation of the thought experiment by Einstein et al.~\cite{einstein1935can} was to show the incompleteness of quantum mechanics. Later, with Bell's theorem~\cite{bell1964einstein} and the experimental violations of Bell's inequalities~\cite{brunner2014bell, anwar2024quantum}, the EPR-Bell scenario highlighted entanglement and non-locality as essential features of quantum physics.  

For illustration, suppose Alice and Bob share the Bell state, $\ket{\Phi^+}= \left(\ket{00} + \ket{11}\right)/\sqrt{2}$, represented by the doubled cup
\[
\tikzfig{interpretations/bell0}
\]
Usually, Alice is placed at the left-hand side and Bob at the right-hand side.
\[
\tikzfig{interpretations/bellb0}
\]
\noindent The two parties can apply unitary operators $\widehat U_{\Phi}$ and $\widehat U_{\Psi}$ to their quantum systems respectively. These unitaries may correspond to the change of measurement bases.
\[
\tikzfig{interpretations/bell0b}
\]

%\textcolor{red}{clarify what it means to have measurement bases ($\Phi$ and $\Psi$) with examples.}

\begin{proposition}
 If Alice and Bob share an entangled state and Alice discards her system, Bob gets a maximally mixed state.
\end{proposition}

\begin{proof}
If Alice discards her state, we have
%Using the causality of unitary processes and OCM, we have:
\begin{equation}\label{bellcalc1}
	\begin{split}
		%\tikzfig{interpretations/bell0b2b} 
		\scalebox{0.8}{\tikzfig{interpretations/bell0b2}}\ \ &= \ \  \scalebox{0.8}{\tikzfig{interpretations/bell0b3}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/bell0b3b}}\\
		 &= \ \ \ \  \scalebox{0.8}{\tikzfig{interpretations/bell0b3c}}  \ \ \ \ \ \   = \ \ \ \ \quad \quad \quad \quad\quad\quad  \scalebox{0.8}{\tikzfig{interpretations/bell0b5}}
	\end{split}
\end{equation}
%we see that 
%\[
%\tikzfig{interpretations/bell0b2} \ \ = \ \ \tikzfig{interpretations/bell0b5b}
%\]
\end{proof}

%\textcolor{red}{discarding one part of the state... partial trace... (marginal probability?)}

The calculation above (\ref{bellcalc1}) shows that if Alice discards her state, Bob ends up with a maximally mixed state. Likewise if Bob discards his state, Alice gets a maximally mixed state. What happens if Alice measures her state to be $\tikzfig{interpretations/copenhagen0d}$ in the ONB $\left\{\tikzfig{interpretations/copenhagen0d}\right\}_i$? 
\[
\tikzfig{interpretations/bell0f}  \ \ = \ \ \tikzfig{interpretations/bell0f2}
\]
%\textcolor{red}{should revise all the ONBs as triangles?}
\noindent This equation means that on Alice measuring the state $\ \tikzfig{interpretations/copenhagen0d}\ $, Bob's state becomes $\ \tikzfig{interpretations/copenhagen0d}\ $ as well. Subsequently, if Bob measures $\ \tikzfig{interpretations/copenhagen0d2}\ $, we get the diagram
\[
\tikzfig{interpretations/bell0c2} \ \ = \ \ \delta_i^j
\]
This number represents Bob's probability of measuring $\ \tikzfig{interpretations/copenhagen0d2}\ $ when Alice measures $\ \tikzfig{interpretations/copenhagen0d}\ $.
Another way to think of this number is that it is the probability of Alice measuring $\tikzfig{interpretations/copenhagen0d}$ and Bob measuring $\tikzfig{interpretations/copenhagen0d2}\ $: 
\[
\tikzfig{interpretations/bell0d2} \ \ = \ \ \tikzfig{interpretations/bell0c2} 
\]
More generally, taking unitaries into account, the joint probability of Alice measuring her system to be $\ \tikzfig{interpretations/copenhagen0d}\ $  and Bob measuring his system to be $\ \tikzfig{interpretations/copenhagen0d2}\ $ is given by 
\[
\tikzfig{interpretations/bell0d}
\]
where the unitaries $\widehat U_{\Phi}$ and $\widehat U_{\Phi}$ represent the change of measurement bases. 

%\textcolor{red}{(conditional?) probability}
%\[
%\tikzfig{interpretations/bell0c}  \ \ = \ \ \tikzfig{interpretations/bell0c2}
%\]
%where the right-hand side is obtained applying OCM.
%\[
%\tikzfig{interpretations/bell0c3}
%\]


\subsection{Demolition Measurement}

%For a Bell state shared by two parties, we have seen how to calculate the updated state after either party measures or discards their state. We have also seen how to calculate the joint probabilities of measurement outcomes.

If we want to incorporate the flow of classical information in our EPR diagrams, it can be done using the measure operation as follows: 
\[
\tikzfig{interpretations/bell0e}
\]
Here, Alice and Bob perform measurements with measurement bases set by applying unitaries $\widehat U_{\Phi}$ and $\widehat U_{\Psi}$ to their systems respectively. The thick wires represent the flow of quantum information, while the thin lines represent the flow of classical information. These measurements are demolition measurements because the quantum state is destroyed. %and the measurement outcomes in the form of classical information flow in the upward direction.

\subsection{Non-demolition Measurement}

If both parties perform non-demolition measurements, we get the diagram
\[
\tikzfig{interpretations/bell2b}
\]
where each measurement produces an output via both a quantum and a classical wire.

\begin{comment}
If Alice discards the classical information, 
\[
\tikzfig{interpretations/bell2b2} 
\]
what happens to the overall system?
\end{comment}

\begin{proposition}\label{belldec}
	If Alice and Bob share a Bell state, and either party performs a non-demolition measurement and then discards the classical outcome of the measurement, the quantum entanglement is destroyed but the two systems retain perfect classical correlations.
\end{proposition}

\begin{proof}
Without loss of generality, assume Alice performs a non-demolition measurement (with measurement basis set by unitary $\widehat U_{\Phi}$),  and then discards the classical outcome of the measurement.
%\[
%\tikzfig{interpretations/bell2bb1}
%\]
%Using diagram rewrite rules and OCM, we have
\[
\scalebox{0.8}{\tikzfig{interpretations/bell2bb1}}  \ \  \overset{(f)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/bell2bb2}} \ \  \overset{(f)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/bell2bb3}}  
  \overset{(OCM)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/bell2bb4}} 
\]
\end{proof}
\noindent The final diagram above comprises a a cup followed by encoding and then a unitary process applied to Bob's system. The thin cup corresponds to a bipartite classical system with perfect correlations; in Dirac notation given by $\frac{\ket{00}\bra{00}}{2} + \frac{\ket{11}\bra{11}}{2}$.

The above calculation shows that Alice discarding the classical information obtained from non-demolition measurement results in decoherence. The decoherence, in turn, leads to the loss of quantum correlations between the two systems. Since decoherence plays an important role in discussions of interpreting quantum theory, we discuss it in the next section. 


\section{Decoherence}\label{secdec}

Superpositions and interference effects play a key role in quantum physics.\footnote{According to Richard Feynman, interference is \textit{``a phenomenon which is impossible, absolutely impossible, to explain in any classical way, and which has in it the heart of quantum mechanics. In reality, it contains the only mystery. We cannot make the mystery go away by “explaining” how it works. We will just tell you how it works. In telling you how it works we will have told you about the basic peculiarities of all quantum mechanics."}~\cite{feynman1965feynman}} Observing interference effects requires maintenance of coherence of superposed wavefunctions in, say, a double-slit experiment. However, this coherence can be lost to spontaneous, uncontrolled factors, or can be intentionally suppressed by the experimenter. Decoherence theory studies the loss of coherence in such scenarios. It is deemed important for the solution of foundational issues in quantum theory, such as the measurement problem, the directionality of time, and how the classical world `emerges' from quantum entities and/or interactions~\cite{bacciagaluppi2003role}. 

It must be made clear from the outset that the term `decoherence' is used in two different senses in quantum physics and quantum foundations~\cite{bacciagaluppi2003role}. The more common use of the term is in the sense of environmental or dynamical decoherence, which involves modelling and investigation of concrete situations in which interference effects are spontaneously erased by interaction of the quantum system with its environment~\cite{schlosshauer2019quantum}. The second, less common sense is in the context of the decoherent histories or consistent histories formulation or interpretation of quantum theory~\cite{griffiths2014consistent}. The former sense of decoherence pertains to the modelling of concrete situations whereas the latter is a general, abstract theory encapsulating key aspects of the phenomenon of decoherence. To avoid confusion between the two meanings, we shall use the term `consistent histories' for the latter case. The theory of consistent histories makes mathematically precise the description of emergence and how to make sense of probabilities in quantum experiments in a consistent manner. 

Decoherence is sometimes invoked as a solution to the `measurement problem'~\cite{bacciagaluppi2003role}. There are reasonable criticisms to the claim that it is~\cite{bub1999interpreting, pearle1998true, adler2003decoherence, joos2003basic}, including one in which decoherence makes the measurement problem more pathological by involving interactions with the environment ~\cite{bacciagaluppi2003role}. In the foundations of physics, decoherence is studied not just as a standalone phenomenon but also as part of the different interpretations that attempt to solve the measurement problem and other problems in quantum theory~\cite{bacciagaluppi2003role, schlosshauer2019quantum}.


\subsection{Decoherence -- Take I}

As shown in Remark \ref{discarddec}, measuring a state and then discarding the classical outcome of the measurement results in decoherence of the state: 
\begin{equation}\label{dectake1}
\tikzfig{interpretations/decoherencee1} \ \ \overset{(f)}{=} \ \ \tikzfig{interpretations/decoherencee2}
\end{equation}
In Proposition \ref{belldec}, it was shown that if one system of a bipartite state is measured and then its classical outcome discarded, the overall system loses its quantum correlations, and only the classical correlations are left. It is instructive to compare this notion of decoherence with that of decoherence due to interaction with the environment.

\subsection{Decoherence -- Take II}

%\textcolor{red}{check context again from the reference to improve explanation}

%\textcolor{blue}{Decoherence and `interference damping' (see~\cite{schlosshauer2019quantum})...}

Consider an environmental variable represented by the quantum state $R$ (R standing for the `ready' state) that gets entangled with the quantum state $\widehat{\psi}$ via a unitary interaction $\widehat U$:
\begin{equation}\label{dectake2c}
\tikzfig{interpretations/decoherenceb}
\end{equation}
%Now, after the two states are entangled, if the environment state undergoes decoherence, the whole two-state system loses quantum correlations, as shown below using OCM:
%\[
%\tikzfig{interpretations/decoherencec} \ \ = \ \ 
%\tikzfig{interpretations/decoherencec2}
%\]
Decoherence due to interaction with the environment arises from the fact that we do not have access to the environmental variable. This is represented by discarding the wire corresponding to the environment state:
\begin{equation}\label{dectake2}
\tikzfig{interpretations/decoherenceb2} %\ \ = \ \ 
%\tikzfig{interpretations/decoherenceb3} \ \  = \ \ \tikzfig{interpretations/bell0b5}
\end{equation}
We can further characterise the process by defining the unitary process $\widehat U$ and the ready state $R$ as follows:
\begin{equation}\label{dectake2b}
\tikzfig{interpretations/decoherenceb2b} \quad \quad \quad \quad \tikzfig{interpretations/decoherenceb2c} 
\end{equation}
\emph{i.e.}, the state $0$ and a CNOT gate where the left qubit is the target and the right one control. A CNOT gate can entangle two qubits if the control qubit is a superposition state. It can be verified that plugging these into diagram (\ref{dectake2c}) gives the Bell state $\tikzfig{interpretations/doubled_cup}\ $ if $\ \tikzfig{interpretations/Copenhagen0} \ = \ \tikzfig{interpretations/decoherenceb2d}\ $. %Similar definitions will show up throughout the chapter.

\noindent Using definitions (\ref{dectake2b}), diagram (\ref{dectake2}) becomes
\[
\tikzfig{interpretations/decoherenceb2e} 
\]
which can be simplified by un-doubling and then using diagram rewrite rules:
\[
\scalebox{0.8}{\tikzfig{interpretations/decoherenceb2e}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f}} \ \ \overset{(f)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f2}} 
\]
\[
\ \ \overset{(id)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f3}} \ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f4}} \ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f5}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherencee2}}
\]
which is the same expression as that of Eq. (\ref{dectake1}). This implies that decoherence, operationally defined as measurement followed by encoding, can arise by intentionally discarding the classical outcome of a non-demolition measurement, or by spontaneous, uncontrolled environmental factors. Moreover, Proposition \ref{belldec} shows that when one part of a bipartite system decoheres, the overall system loses its quantum correlations.  

\begin{convention}
	Throughout this chapter, we use definitions similar to those in Eq. (\ref{dectake2b}) for illustrative purposes, as they are consistent with those used in the quantum interpretations literature. For instance, we generally pick the initial ready/pointer states to be $\ket{0}$, and the entangling unitary to be the CNOT gate. These definitional choices are not the only ones possible. The various aspects of quantum theory and its interpretations discussed in this chapter can also be illustrated using other definitions, provided they are used consistently.
\end{convention}

%\textcolor{blue}{Decoherence should be $100\%$ doable.}

%\textcolor{red}{notes}

%\[\includegraphics[width=0.8\linewidth]{figures/b16.jpg}\]

%\[\includegraphics[width=0.8\linewidth]{figures/b17.jpg}\]

%\[\includegraphics[width=0.8\linewidth]{figures/b18.jpg}\]

%\[\includegraphics[width=0.8\linewidth]{figures/b19.jpg}\]

%\[\includegraphics[width=0.8\linewidth]{figures/b20.jpg}\]

%\[\includegraphics[width=0.8\linewidth]{figures/b21.jpg}\]  

%\textcolor{red}{The role of decoherence in different interpretations... }

%Decoherence vs decoherent/consistent histories...
%Decoherence references... Decoherent histories references...
%Quantum darwinism?

\section{Consistent Histories}\label{seccons}

The consistent or decoherent histories interpretation or framework was developed by Griffiths~\cite{griffiths1984consistent} and later built upon by others~\cite{omnes1988logical, gell1996quantum}. A detailed exposition can be found in the books~\cite{omnes1999understanding, griffiths2003consistent}.

This interpretation gives no special status to measurements. In textbook quantum mechanics, probabilities are introduced via measurement processes and when no measurement takes place, the time evolution of quantum systems is linear and deterministic. In the consistent histories approach, the evolution of quantum systems is always stochastic or probabilistic. The probabilities are assigned by the Born rule or its extended variants. The main emphasis of this approach is that quantum systems should be described using a well-defined sample space of probabilities, called a \textit{framework}~\cite{griffiths2014consistent}. Moreover, the wavefunction is not considered real; rather, it is deemed merely a calculating device for determining the probabilities of histories that are real.

In this approach, measurements are not considered fundamental; the focus is instead on histories of quantum \textit{events}, which are `sets of time-ordered projection operators', and how to assign probabilities to these histories in a consistent manner~\cite{schlosshauer2005decoherence}. The original motivation for this approach came from cosmology. Since the universe is a closed system by assumption, there can be no external observer. On the other hand, an external observer is essential in the Copenhagen (class of) interpretation(s). There are some slight differences between the different approaches to consistent histories. We shall closely follow the description provided in the review~\cite{schlosshauer2005decoherence}.

%\textcolor{red}{BIG TODO: subscript should be $o_k$ or $o$, superscript should be $k$ }

\textbf{CH1. Histories.}  Here is how to describe a \textit{history} in this interpretation. Consider a quantum system, initially in the the state $\tilde{\rho}$ at time $t_0$, that undergoes $n$ projective measurements %$\{P_k\}_k$ 
\[
\left\{\map{P_k}\right\}_k
\]
in a time sequence $t_1 < t_2 < ... < t_n$ (where $t_1 > t_0$), with unitary evolution in between the measurements. For each time instant $t_k$, the projective measurements are defined as an exhaustive set of mutually orthogonal operators:
\[
\mathcal{P}^{(k)} := \left\{\map{P_k^{o_k}}\right\}_{o_k}
\]
obeying the equations $\sum_{o_k} \map{P_k^{o_k}} \ \ = \  \tikzfig{interpretations/singlewire} \quad , \quad \tikzfig{interpretations/consistent4b} \ = \ \delta_{i}^{j}\  \map{P_k^{i}}$.
%\[
%\sum_{\alpha_i} \widehat P_{\alpha_i}^{(i)} (t_i) = \mathbb{1} \ \ \ \ \  \text{and} \ \ \ \  \ \widehat P_{\alpha_i}^{(i)} (t_i) \widehat P_{\beta_i}^{(i)} (t_i) = \delta_{\alpha_i, \beta_i} \widehat P_{\alpha_i}^{(i)} (t_i)
%\]
%Consider a quantum system $S$ described by a density matrix $\rho$ at an initial time $t_0$. Take a sequence of instances of time $t_1 < t_2 < ... < t_n$, with $t_0 < t_1$. For each $t_i$ in the sequence, define an exhaustive set $\mathcal{P}^{(i)} = \{\widehat P_{\alpha_i}^{(i)} (t_i) | \alpha_i = 1, ..., m_i  \}, 1 \leq i \leq n$, of mutually orthogonal projection operators $\widehat P_{\alpha_i}^{(i)} (t_i)$, 
%\[
%\mathcal{H}_{\{\alpha\}} = \left \{ \dmap{\widehat P_{\alpha_1}^{(1)} (t_1)}, \dmap{\widehat P_{\alpha_2}^{(2)} (t_2)}, ..., \dmap{\widehat P_{\alpha_n}^{(n)} (t_n)}  \right \}
%\]
%which obey the following equations:
%Diagrammatically, the equations are
%\[
%\sum_{\alpha_i} \dmap{\widehat P_{\alpha_i}^{(i)} (t_i)} = \ \ 
%\tikzfig{interpretations/doubledwire2} \ \ \ \ \  \text{and} \ \ \ \  \ \tikzfig{interpretations/consistent4}\ = \  \dscalar{\delta_{\alpha_i, \beta_i}} \dmap{\widehat P_{\alpha_i}^{(i)} (t_i)}
%\]
%\textcolor{red}{maybe remove t_i from boxes because time is apparent in the diagrams anyway}
%\textcolor{red}{numbers as diamonds everywhere.}
In the Heisenberg picture, the projector evolves and the state is fixed. We shall represent the time-evolved projector with a tilde on the projector symbol:
%\[
%\widehat P_{\alpha_i}^{(i)} (t) = U^{\dagger} (t, t_0) \widehat P_{\alpha_i}^{(i)} (t_0) U(t, t_0)
%\]
%\[
%\dmap{\widehat P_{\alpha_i}^{(i)} (t)} \ = \ \  \tikzfig{interpretations/consistent5} 
%\]
\begin{equation}\label{heisevol}
\map{\tilde{P}^{o_k}_k} \ := \ \  \tikzfig{interpretations/consistent10} 
\end{equation}
%\[
%\tikzfig{interpretations/non-dem-map}
%\]
where $U$ represents unitary evolution. %The time-evolved projector is represented with a tilde on the projector symbol.  
% is a unitary operator corresponding to the dynamical evolution of the operator \textcolor{red}{(or state vector?)} from time $t_0$ to $t$.


\begin{comment}

As described earlier, von Neumann measurements are defined as quantum processes
\[
\tikzfig{interpretations/measdiag1}
\]
for which the following equation holds:
\[
\tikzfig{interpretations/diagramsUUorth3}
\]
Moreover, it can be checked that a \emph{non-demolition} measurement
\[
\tikzfig{interpretations/CQMII-7}
\]
is indeed a von Neumann measurement. Composing the measurement result wire with a classical outcome $i$, we get
\[
\tikzfig{interpretations/CQMII-9-2}
\] 
Hence, the measurement changes the state to be measured to the state $i$. This is a projector measurement/operator.

\[
\dmap{\widehat P_{\alpha}} \ \  \equiv \ \ \  \tikzfig{interpretations/CQMII-9-3}
\]

\end{comment}

What is a possible history from the exhaustive set of projection operators for the time sequence? A special case of a possible history is a `maximally fine-grained' one, which is defined for the time sequence $t_1 < t_2 < ... < t_n$ by picking one projection operator from $\mathcal{P}^{(k)}$ for each time instant $t_k$:
%\[
%\mathcal{H}_{\{\alpha\}} = \{\widehat P_{\alpha_1}^{(1)} (t_1), \  \widehat P_{\alpha_2}^{(2)} (t_2), \ ..., \ \widehat P_{\alpha_n}^{(n)} (t_n) \}
%\]
$\mathcal{H}_{\{o\}} = \left \{ \map{P_1^{o_1}}, \map{P_2^{o_2}}, ..., \map{P_n^{o_n}}  \right \}$. Diagrammatically, this history is represented as 
\begin{equation}\label{history1}
\tikzfig{interpretations/consistentc10}
\end{equation}
with unitary evolution occurring between each pair of projectors, as mentioned earlier.

At this point, a set $\mathfrak{h} = \{\mathcal{H}_{\{o\}} \}$
of all the possible histories can also be defined. Each history can be thought of as a sequence of propositions to the effect `the system $\tilde{\rho}$ was, at time $t_k$, in a state of the subspace spanned by $\left\{\map{P_k^{o_k}}\right\}_{o_k}$.'~\cite{schlosshauer2005decoherence}.

`Coarse-grained' histories can be obtained by combining maximally fine-grained histories. This is achieved by assigning a combination of the projection operators $P^{o_k}_k$ with $0$ and $1$ as coefficients to each time instant $t_k$.
%\[
%\widehat Q_{\beta_i}^{(i)} (t_i) = \sum_{\alpha_i} \pi_{\alpha_i}^{(i)} \widehat P_{\alpha_i}^{(i)} (t_i), \ \ \ \  \pi_{\alpha_i}^{(i)} \in \{0, 1\}
%\]
%\[
%\map{\widehat Q_{\beta_i}^{(i)} (t_i)} \ = \ \sum_{\alpha_i} \pi_{\alpha_i}^{(i)} \map{\widehat P_{\alpha_i}^{(i)} (t_i)}, \ \ \ \  \pi_{\alpha_i}^{(i)} \in \{0, 1\} 
%\]
%\[
%\widehat Q_{\beta_i}^{(i)} (t_i) = \sum_{\alpha_i} \pi_{\alpha_i}^{(i)} \widehat P_{\alpha_i}^{(i)} (t_i), \ \ \ \  \pi_{\alpha_i}^{(i)} \in \{0, 1\}
%\]
\[
\map{Q_{k}^{s_k}} \ = \ \sum_{o_k} \pi_{k}^{o_k} \map{P^{o_k}_k}, \ \ \ \  \pi_{k}^{o_k}  \in \{0, 1\} 
\]
This history would be diagrammatically represented as 
\begin{equation}\label{history2}
	\tikzfig{interpretations/consistentc14}
\end{equation}

\textbf{CH2. Probabilities.} In textbook quantum mechanics, events are given by the eigenstates of a projection operator $\tilde{P}^{o}$, and probabilities are assigned to individual events using the Born rule: $p(o) = \text{Tr}\big[\tilde{P}^{o} \tilde{\rho} \tilde{P}^{o}\big]$. Diagrammatically, this formula is
\[
p(o) \ \ = \ \ \tikzfig{interpretations/consistentb3c} \ = \  \tikzfig{interpretations/consistentb3b} \ = \  \tikzfig{interpretations/consistentb1b}  \ = \ \tikzfig{interpretations/born5}
\]
This is the Heisenberg picture (using the convention of Eq. (\ref{heisevol})). %in which the projector operator evolves and the state is fixed. %We can equivalently express it in the Schr\"{o}dinger picture, in which the state evolves and the projector is fixed.
%\[
%p(o)   \ = \ \tikzfig{interpretations/born5} \ = \ \tikzfig{interpretations/consistentb2} \ = \ \tikzfig{interpretations/consistentb2b} 
%\]
%where we have used the fact that the unitary $\widehat U$ is causal. The Schr\"{o}dinger picture version of Eq. (\ref{consistentborn1}) is $p(o) = \text{Tr}\big[P^{o} U \rho U^{\dagger} P^{o}\big]$. %and $\tikzfig{interpretations/consistentb2d} \ := \ \tikzfig{interpretations/consistentb2e}$.

%Note: the time variable can be removed from the diagram because by convention, it is known that time moves from bottom to top in the diagram. \textcolor{red}{is it correct?}

%Suppose two projector valued measurements are made in a sequence with unitary time evolution in between, we have 
%\[
%\tikzfig{interpretations/consistentc1} \ \ = \ \  \tikzfig{interpretations/consistentc2} 
%\]
%where on the right hand side, we have used unitarity as well as the fact that unitaries are causal. Now, we can define the Heisenberg evolution of projectors in accordance with Eq. (\ref{heisevol}):
%\[
%\tikzfig{interpretations/consistentc2} \ \ = \ \ \tikzfig{interpretations/consistentc3} 
%\]
%where $\tikzfig{interpretations/consistentc4}$ and $\tikzfig{interpretations/consistentc5}$.

Likewise, for calculating the probability $p(\mathcal{H}_{\{o\}})$ of a history $\mathcal{H}_{\{o\}}$, an extension of the Born rule is defined in the consistent histories interpretation~\cite{schlosshauer2005decoherence}:
%\[
%p(\mathcal{H}_{\{o\}})  \ := \ p(o_1, o_2, ..., o_n) \ = \ \text{Tr}[P_n^{o_n} U_n \cdots  U_2 P_1^{o_1} U_1 \rho U_1^{\dagger} P_1^{o_1} U_2^{\dagger}   \cdots U_n^{\dagger}  P_n^{o_n}] 
%\]
%in the Schr\"{o}dinger picture, or
$p(\mathcal{H}_{\{o\}}) \ = \ \text{Tr}[\tilde{P}_n^{o_n} \cdots  \tilde{P}_1^{o_1} \tilde{\rho} \tilde{P}_1^{o_1}  \cdots \tilde{P}_n^{o_n}]$ where $\tilde{P}_k^{o_k} := U^{\dagger}_1 ... U^{\dagger}_k P_k^{o_k} U_k ... U_1$. This is diagrammatically given by 
\begin{equation}\label{bornconsistency2}
p(\mathcal{H}_{\{o\}}) \ = \  \tikzfig{interpretations/consistentc11}
\end{equation}
This formula works fine for calculating the probabilities of maximally fine-grained histories such as the one in diagram (\ref{history1}). However, for coarse-grained histories, a \textit{consistency condition} has to be satisfied for a similar formula to be applicable. 

%where $\mathcal{D}(\alpha, \alpha)$ is a special case of the \textit{decoherence functional} $\mathcal{D}(\alpha, \beta)$ given by []
%\[
%\mathcal{D}(\alpha, \beta) = \text{Tr}[\widehat P_{\alpha_n}^{(n)} (t_n) \cdots \widehat P_{\alpha_1}^{(1)} (t_1) \rho_0 \widehat P_{\beta_1}^{(1)} (t_1) \cdots \widehat P_{\beta_n}^{(n)} (t_n)] 
%\]


%Since the density matrix $\rho_0$ is defined as
%\[
%\dkpoint{\boldsymbol\rho_0}\ = \sum_{ij} \rho^{ij} \pointmap{i} \pointmap{j}
%\]
%the decoherence functional $\mathcal{D}(\alpha, \beta)$ is diagrammatically given by 
%\[
%\mathcal{D}(\alpha, \beta) \  = \tikzfig{interpretations/consistent1}
%\]
%\textcolor{red}{should we write t's}

%Therefore, the probability $p(\mathcal{H}_{\{\alpha\}})$ of the history $\mathcal{H}_{\{\alpha\}}$ is given by 
%\[
%p(\mathcal{H}_{\{\alpha\}}) \ = \tikzfig{interpretations/consistent3}  \ = \ \tikzfig{interpretations/consistent2}  
%\]

%\textcolor{red}{should we write t's}
\textbf{CH3. Consistency.} Suppose we take a coarse-grained history that is obtained by combining two maximally fine-grained histories of $n$ projective measurements, say \\ $
\mathcal{H}_{\{o\}} := \left \{ \map{P_{1}^{o_{1}}}, ..., \map{P_{{l-1}}^{o_{{l-1}}}}, \map{P_{l_\alpha}^{o_{l_\alpha}}}, \map{P_{{l+1}}^{o_{{l+1}}}}, ..., \map{P_{n}^{o_{n}}}  \right \}
$ and 
\\ $
\mathcal{H}_{\{o'\}} := \left \{ \map{P_{1}^{o_{1}}}, ..., \map{P_{{l-1}}^{o_{{l-1}}}}, \map{P_{l_\beta}^{o_{l_\beta}}}, \map{P_{{l+1}}^{o_{{l+1}}}}, ..., \map{P_{n}^{o_{n}}}  \right \}
%\mathcal{H}_{\{o'\}} := \left \{ \map{P_1^{o_1}}, ..., \map{P_{l-1}^{o_{l-1}}}, \map{P_l^{m_l}}, \map{P_{l+1}^{o_{l+1}}}, ..., \map{P_n^{o_n}}  \right \}
$ : 
\[
\mathcal{H}_{\{o \lor o'\}} := \left \{ \map{P_1^{o_1}}, ..., \map{P_{l-1}^{o_{l-1}}}, \map{P_{l_{\alpha}}^{o_{l_\alpha}}} + \map{P_{l_{\beta}}^{o_{l_\beta}}}, \map{P_{l+1}^{o_{l+1}}}, ..., \map{P_n^{o_n}}  \right \}
\]
where $ \map{P_{l_\alpha}^{o_{l_\alpha}}} + \map{P_{l_\beta}^{o_{l_{\beta}}}}\  =: \ \map{f_l^{s_l}}%\ := \ %\map{P_k^{o_k}} + \map{P_k^{m_k} }
$
is defined to mean that at time $t_l$, the system is within the range determined by the union of $ \map{P_{l_\alpha}^{o_{l_\alpha}}}$ and $\map{P_{l_\beta}^{o_{l_{\beta}}}}$.\footnote{Here $\left\{\map{P_{l_\alpha}}\right\}_{l_\alpha}$ and $\left\{\map{P_{l_\beta}}\right\}_{l_\beta}$ are different projective measurements in general.} Now one can use a formula similar to Eq. (\ref{bornconsistency2}) to calculate the probability of this coarse-grained history:
\begin{equation}%\label{bornconsist}
	p(\mathcal{H}_{\{o \lor o' \}} ) \ = \  \tikzfig{interpretations/consistentc13b}
	%\tikzfig{interpretations/consistentc13}
\end{equation}
% if and only if the following equation holds for all $\mathcal{H}_{\{\alpha\}} \neq \mathcal{H}_{\{\beta\}}$, for the coarse grained history~\cite{gell1996quantum}:
if and only if the following equation holds for the coarse-grained history:
\begin{equation}\label{consistencycond1}
\text{Re}\left[\tikzfig{interpretations/consistent1b2}\right]\ = 0  \ \ \text{if} \ \  \map{P_{l_\alpha}^{o_{l_\alpha}}} \neq \map{P_{l_\beta}^{o_{l_{\beta}}}} 
\end{equation}
%\textcolor{red}{change pure state to density matrix rho}
%This equation gives the \textit{consistency condition} for the two histories $\mathcal{H}_{\{\alpha\}}$ and $\mathcal{H}_{\{\beta\}}$. 
\noindent Eq. (\ref{consistencycond1}) gives the \textit{consistency condition} for the two histories $\mathcal{H}_{\{o\}}$ and $\mathcal{H}_{\{o'\}}$. %, $\mathcal{H}_{\{\alpha \lor \beta \}}$. 
The expression inside the square brackets on the left-hand side is called the \textit{decoherence functional}~\cite{schlosshauer2005decoherence}. It calculates the overlap between the two histories that are combined as part of coarse-graining. The consistency condition defines consistent histories as those that are `orthogonal', or have no interference between them. 

This condition ensures that probabilities in the consistent histories are linear, \emph{i.e.,} the probability of a history involving combined projection operators is equal to the sum of the probabilities of the individual, fine-grained histories. Diagrammatically, this requirement is
\[
 \scalebox{0.8}{\tikzfig{interpretations/consistentc13b}} \ \overset{!}{=} \   \scalebox{0.8}{\tikzfig{interpretations/consistentc13c}} \ + \ \scalebox{0.8}{\tikzfig{interpretations/consistentc13d}}
\]
\[ \iff
  \scalebox{0.8}{\tikzfig{interpretations/consistent1c}} \ + \ \scalebox{0.8}{\tikzfig{interpretations/consistent1b}} \ + \ \scalebox{0.8}{\tikzfig{interpretations/consistentc13c}} \ + \ \scalebox{0.8}{\tikzfig{interpretations/consistentc13d}} \ \overset{!}{=} \   \scalebox{0.8}{\tikzfig{interpretations/consistentc13c}} \ + \ \scalebox{0.8}{\tikzfig{interpretations/consistentc13d}}
\]
which holds iff Eq. (\ref{consistencycond1}) is true.

More generally, consider coarse-graining over the two maximally fine-grained histories of $n$ projections, $
\mathcal{H}_{\{\alpha\}} := \left \{ \map{P_{1_\alpha}^{o_{1_\alpha}}}, ..., \map{P_{n_\alpha}^{o_{n_\alpha}}}  \right \}
$ and $
\mathcal{H}_{\{\beta\}} := \left \{ \map{P_{1_\beta}^{o_{1_\beta}}}, ..., \map{P_{n_\beta}^{o_{n_\beta}}}  \right \}
$: $\mathcal{H}_{\{\alpha \lor \beta\}} := \left \{ \map{f_1^{s_1}}, ..., \map{f_n^{s_n}} \right \}$ where $\ \map{f_k^{s_k}} :=  \map{P_{k_\alpha}^{o_{k_\alpha}}} + \map{P_{k_\beta}^{o_{k_\beta}} }$ for all $k$.\footnote{For all $k$, $\left\{\map{P_{k_\alpha}}\right\}_{k_\alpha}$ and $\left\{\map{P_{k_\beta}}\right\}_{k_\beta}$ are different projective measurements in general.} The probability of this coarse-grained history is given by:
\begin{equation}\label{bornconsistency3}
	p(\mathcal{H}_{\{\alpha \lor \beta \}} ) \ = \ \tikzfig{interpretations/consistentc13}
\end{equation}
if and only if the following equation holds~\cite{griffiths1984consistent, omnes1990hilbert, omnes1992consistent}:
\begin{equation}\label{decfunct}
	\tikzfig{interpretations/consistent1}\ = 0  \ \ \text{if} \ \ \mathcal{H}_{\{\alpha\}} \neq \mathcal{H}_{\{\beta\}} %\delta_{\alpha}^{\beta}
	%\tikzfig{interpretations/consistentc12} 
\end{equation}
\noindent This is a necessary and sufficient condition for consistency. If this condition is violated, the sum rule for calculation of probabilities does not apply. This is a case when interference effects are present in the combination of histories $\mathcal{H}_{\{\alpha\}}$ and $\mathcal{H}_{\{\beta\}}$~\cite{schlosshauer2005decoherence}. Hence, for the validity of the standard laws of probability for coarse-grained histories, the consistency condition must be met by a set $\mathfrak{h}$ of possible histories~\cite{schlosshauer2005decoherence}. 

If the consistency condition (Eq. (\ref{decfunct})) holds, Eq. (\ref{bornconsistency3}) can be thought of as the distribution function of a stochastic process in which the histories play the role of trajectories of quantum systems~\cite{bacciagaluppi2003role}. The projectors do not correspond to measurements but to \textit{events}. In other words, this conception of decoherence suggests that the probabilities of quantum events must be calculated under the assumption that quantum states have already collapsed at earlier time instants, chosen or defined within the abstract model~\cite{bacciagaluppi2003role}. In a qualitative sense, classical behaviour emerges because the probabilities of quantum events follow the usual rules of probability, owing to the consistency condition~\cite{bacciagaluppi2003role}.

A set of histories $\mathfrak{h}$ is consistent or decoherent when all the members of the set (\textit{i.e.} the histories) meet the consistency condition. In other words, these histories are independent and free from interference. Such histories are said to belong to the same \textit{framework}. Histories within the same framework can be combined via coarse-graining. 

When discussing the histories of quantum systems, it is essential to remain within a single framework, as determined by the experimental setup. This is known as the \textit{single framework rule}~\cite{griffiths2014consistent}. According to this rule, combining the results and probabilities of multiple incompatible (or mutually inconsistent) frameworks leads to nonsensical conclusions.

\subsection{The Consistency of Histories in CQM}\label{secconsCQM}

Recall Def. \ref{quantumtheorydef}: quantum theory is a process theory of causal classical-quantum (cq) maps. We focus our attention on the subset of this theory comprising causal quantum maps (\emph{i.e.}, quantum processes according to Def. \ref{quantumtheorydef}), since it suffices to describe consistent histories. More explicitly, a quantum process $\{\Phi^i\}_i$ satisfies the causality postulate:  
\begin{equation}\label{causalpost1}
	\sum_i \  \tikzfig{interpretations/causal2}\ \ = \ \, \tikzfig{interpretations/discard}
\end{equation}
where the individual maps $\Phi^i$ are called \textit{branches} of the process. The quantum process $\{\Phi^i\}_i$ can be an ONB or a more general von Neumann measurement, where the maps $\Phi^i$ are its projectors. One can already notice that the branches of a process correspond to \textit{histories}.

\begin{remark}\label{singeventbranch}
The causality postulate (Eq. (\ref{causalpost1})) guarantees that for a quantum process $\{\Phi^i\}_i$ (such as a von Neumann measurement) and any state $\boldsymbol \rho$, we have 
\[
\sum_i p(i) \ = \ \sum_i \  \tikzfig{interpretations/consistentb2b} \ = \ %\tikzfig{interpretations/consistentb2b2} \ = \ 
\tikzfig{interpretations/discard3} \ = \ \emptydiag
\]
showing that the probabilities add up to one. Therefore, the causality of a quantum process ensures that probabilities can be \textit{consistently} assigned to its branches or histories. 

Adding two or more of the branches of a quantum process yields a \textit{coarse-grained branch}. However, combining branches of different quantum processes does not necessarily result in a legitimate branch of any quantum process. Probabilities of such illegitimate `branches' are undefined. In this way, the causality postulate rules out such `branches' from quantum theory.
\end{remark}

\begin{remark}
	The foregoing discussion has focused on single-event histories, but the same argument can be generalised to multiple-event histories. Consider a \textit{maximally fine-grained branch} the probability of which is calculated in Eq. (\ref{bornconsistency2}). This is a branch of the quantum process $\{\tilde{P}_n^{o_n}\}_{o_n} \cdots \{\tilde{P}_1^{o_1}\}_{o_1}$, which is composed of causal processes $\{\tilde{P}_1^{o_1}\}_{o_1}$, ..., $\{\tilde{P}_n^{o_n}\}_{o_n}$ and is therefore causal as well. Hence, we have
	\[
	\sum_{o_1, \cdots, o_n} p(o_1, \cdots, o_n) \ = \ \sum_{o_1, \cdots, o_n} \tikzfig{interpretations/consistentc11} \ = \ %\tikzfig{interpretations/consistentb2b2} \ = \ 
	\tikzfig{interpretations/discard3} \ = \ \emptydiag
	\]
	meaning the probabilities add up to one, \emph{i.e.}, they can be assigned in a consistent manner. 
	
	Just as discussed in Remark \ref{singeventbranch}, one can combine two or more branches of the process $\{\tilde{P}_n^{o_n}\}_{o_n} \cdots \{\tilde{P}_1^{o_1}\}_{o_1}$ to obtain a coarse-grained branch, the probability of which can be calculated using a formula similar to Eq. (\ref{bornconsistency2}). However, coarse-graining over two or more branches of different quantum processes does not generally result in a well-defined branch. The only legitimate coarse-grained branches are those that are part of quantum processes. Consistency of branches is guaranteed by the causality of quantum processes.
	%process $\{\tilde{P}_n^{o_n}\}_{o_n} \cdots \{\tilde{P}_1^{o_1}\}_{o_1}$
	%Coarse-grain over the branches $\tilde{P}_n^{o_n} \cdots \tilde{P}_1^{o_1}$
	% If the resultant is a branch of a causal process	
	%The composition of causal processes results in a causal process.
\end{remark}
%There is a difference in terminology between the consistent histories framework and CQM. In CQM, consistent histories are called \textit{branches}.
%In the last chapter, we discussed indeterministic processes. A non-demolition von Neumann measurement is an important example of a causal indeterministic process. An indeterministic process has multiple branches. The branches of a von Neumann measurement are projectors; therefore von Neumann measurements are also called \textit{projective measurements}.
%\begin{proposition}\cite{CKbook}
%	The branches of a non-demolition von Neumann measurement are projectors.
%\end{proposition}
%\begin{proposition}\cite{CKbook}\label{causalcomp}
%	The composition of causal processes results in a causal process.
%\end{proposition}
%\begin{proposition}\label{causalcomp2}
%	For a non-demolition von Neumann measurement $\left\{\ \dmap{\widehat P^o}\right\}_o$, the maps $\left\{\ \map{P^o}\right\}_o$ form a resolution of the identity.
%\end{proposition}
%\begin{proof}
%	Using the causality postulate (Eq. (\ref{gencausal})) for the causal process comprising projectors $\left\{\ \dmap{\widehat P^o}\right\}_o$, we have
	%\[
	%\sum_o \  \tikzfig{interpretations/causal3} = \  %\tikzfig{interpretations/discard}
	%\]
	%Unfolding the diagrams, we obtain $\ \sum_o  %\tikzfig{interpretations/consistente1} \ = \ %\tikzfig{interpretations/consistente2}\ $ from which we get $\ \sum_o  %\tikzfig{interpretations/consistente3} \ = \ %\tikzfig{interpretations/singlewire}\ $. Since $P^o$ are projectors, we %have $\ \sum_o  \map{P^o} \ = \ \tikzfig{interpretations/singlewire}\ $.
%\end{proof}
%In CQM, the causality postulate ensures that probabilities are consistently assigned to histories. 
%For a single event (\emph{i.e.}, unitary evolution followed by a projective measurement), the probability is given by 
%\[
%p(o)   \ = \  \tikzfig{interpretations/consistentb2b} \ %= \ \tikzfig{interpretations/consistentb2c} 
%\]
%Now, the causality postulate (Eq. (\ref{gencausal})) ensures that for an indeterministic quantum process (such as the family of projectors $\left\{\ \dmap{\widehat P^o}\right\}_o$), we have 
%\[
 %\sum_o p(o) \ = \ \sum_o \  \tikzfig{interpretations/consistentb2b} \ = \ \tikzfig{interpretations/consistentb2b2} \ = \ \tikzfig{interpretations/discard2} \ = \ \emptydiag
%\]
%which means that the probabilities add up to one. 
%Now consider a history with multiple events: 
%\[
%\tikzfig{interpretations/consistentc10}
%\]
%Its probability can be calculated by taking the trace of the diagram: 
%\[
%\tikzfig{interpretations/consistentc15}
%\]
%The causality postulate (Eq. (\ref{gencausal})) and Proposition \ref{causalcomp} dictate that 
%\[
%\sum \ \tikzfig{interpretations/consistentc15} \ = \ \tikzfig{interpretations/discard2} \ = \ \emptydiag
%\]
%This means that the probabilities are consistently assigned (\emph{i.e.,} they add up to one) if the whole history is a branch of a causal process. We know that the unitaries on the left hand side are causal. 
%Therefore, causality of the overall process requires that
%\[
%\sum_{o_k} \  \tikzfig{interpretations/causal4} = \  \tikzfig{interpretations/discard} \  \ \   \  \ \  \  \ \forall \ k
%\]
%which, using Proposition \ref{causalcomp2}, implies
%\[
%\sum_{o_k}  \map{P_k^{o_k}} \ = \ \tikzfig{interpretations/singlewire}  \  \ \  \  \ \  \  \ \forall \ k
%\]	
Therefore, from the perspective of CQM, a quantum process is a \textit{consistent set of histories}, while its branches are the \textit{consistent histories}. The causality postulate, obeyed by quantum processes, ensures that probabilities can always be assigned to branches, and that any coarse-graining that does not yield a branch of a quantum process is invalid.

%if coarse-graining does not yield a
%if coarse-graining of histories, only those projectors that are part of the same resolution of the identity can be combined. A resolution of the identity in terms of projectors forms a single framework in the sense of consistent histories.
%\textcolor{red}{use Halpha and Hbeta below!!!}
%\textcolor{red}{REVISE BELOW}

\subsection{The Stern-Gerlach Experiment}\label{secconsSG}

\begin{example}%[Stern-Gerlach Experiment]
Suppose we are interested in calculating the probabilities of measurement outcomes in a Stern-Gerlach setting.\footnote{The Stern-Gerlach experiment was one of the first examples of quantum measurement. Historically a demonstration of the quantisation of spin~\cite{castelvecchi2022stern}, it is now employed as a prototypical two-level system to discuss quantum measurement and its interpretations.} A quantum state $\widehat{\psi}$ is subjected to two projective measurements, $\widehat{P}_1$ and $\widehat{P}_2$. The probability of the history comprising projections $\widehat{P}_1^{o1}$ and $\widehat{P}_2^{o2}$ is to be calculated.
\begin{equation}\label{sternborn}
\tikzfig{interpretations/sterngerlach1}
\end{equation}
Suppose the first projective measurement is made in the Z basis, $\left\{\dpointmap{0}, \dpointmap{1}\right\}$, and the second in the X basis, $\left\{\dpointmap{+}, \dpointmap{-}\right\}$. Then a set of maximally fine-grained histories would be:
\begin{equation}\label{gerlachhist1}
\left \{ \scalebox{0.8}{\tikzfig{interpretations/sterngerlach2}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach3}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach5}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach4}} \right \}
\end{equation}
As these are maximally fine-grained histories, the problem of consistency does not arise. In other words, these histories are consistent in a trivial manner, and one can use Eq. (\ref{sternborn}) to calculate the probabilities of these histories. %One can also verify that the bases of the two measurements form resolutions of the identity. 
%\[
%\begin{array}{c}
%	\pointmap{0} \vspace{1mm} \\
%	\copointmap{0}
%\end{array}  + \begin{array}{c}
%	\pointmap{1} \vspace{1mm} \\
%	\copointmap{1}
%\end{array} = \ \tikzfig{interpretations/singlewire} \quad \quad \begin{array}{c}
%\pointmap{+}\vspace{1mm}\\
%\copointmap{+}
%\end{array}  + \begin{array}{c}
%\pointmap{-}\vspace{1mm}\\
%\copointmap{-}
%\end{array} = \ \tikzfig{interpretations/singlewire} 
 %\]
%Since we are dealing with a \textit{consistent} set of maximally fine-grained histories, 
%$\begin{array}{c}
%	\pointmap{0} \vspace{1mm} \\
%	\copointmap{0}
%\end{array}$  and $\begin{array}{c}
%	\pointmap{1} \vspace{1mm} \\
%	\copointmap{1}
%\end{array}$ are part of the same resolution of identity, 
Moreover, we can readily coarse-grain over them. For instance, coarse-graining over the two projectors of the first measurement results in an identity map, and the set of histories becomes
\[
\left \{ \scalebox{0.8}{\tikzfig{interpretations/sterngerlach7}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach6}} \right \}
\]
which is still consistent. 

%As the first measurement comprises only two projectors, coarse-graining results in the identity map. This implies replacing the first projective measurement with no measurement.
% by defining a map $ \map{f_1^{o1}} \ := \ \begin{array}{c}
%\pointmap{0} \vspace{1mm} \\
%\copointmap{0}
%\end{array}  + \begin{array}{c}
%\pointmap{1} \vspace{1mm} \\
%\copointmap{1}
%\end{array} \ = \ \tikzfig{interpretations/singlewire}\ $. As the system has only two elements in the basis, coarse-graining results in the identity map. This implies replacing the first projective measurement with no measurement. After coarse-graining, the set of histories becomes
%\[
%\left \{ \scalebox{0.8}{\tikzfig{interpretations/sterngerlach7}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach6}} \right \}
%\]
%which is still consistent. 

From the CQM perspective, the set (\ref{gerlachhist1}) corresponds to a quantum process the branches of which are given by the elements of the set. One can verify that the probabilities of these branches add up to one. 

Now consider setting up the Stern-Gerlach apparatus such that both the projective measurements are in the X basis, $\left\{\dpointmap{+}, \dpointmap{-}\right\}$. Now the consistent set of maximally fine-grained histories is 
\[
\left \{ \scalebox{0.8}{\tikzfig{interpretations/sterngerlach8}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach9}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach10}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/sterngerlach11}} \right \}
\]
This set also corresponds to a quantum process, and the probabilities of its branches add up to one. Combining any branch of this process with that of the process corresponding to the set (\ref{gerlachhist1}) does not give any branch of a legitimate process. Therefore, the histories in this set are inconsistent with those in the set (\ref{gerlachhist1}).
%because the maps $\begin{array}{c}
%	\pointmap{0} \vspace{1mm} \\
%	\copointmap{0}
%\end{array}$  and $\begin{array}{c}
%	\pointmap{1} \vspace{1mm} \\
%	\copointmap{1}
%\end{array}$ together with $\begin{array}{c}
%\pointmap{+} \vspace{1mm} \\
%\copointmap{+}
%\end{array}$  and $\begin{array}{c}
%\pointmap{-} \vspace{1mm} \\
%\copointmap{-}
%\end{array}$, corresponding to the first projector, do not form a resolution of the identity. 
\end{example}

\subsection{The EPR-Bell Scenario}\label{secconsEPR}

\begin{example}%[EPR Scenario]
In the consistent histories approach, a possible history of the Bell state in an EPR scenario is given by 
\[
\tikzfig{interpretations/decoherenced2}
\]
where $\dmap{\widehat P_{\alpha}^{o_\alpha}}$ and $\dmap{\widehat P_{\beta}^{o_\beta}}$ are projections arising from measurements performed by Alice and Bob respectively. Suppose Alice measures in the Z basis and Bob in the X basis. Then the maximally fine-grained histories are given by 
\begin{equation}\label{eprhistory}
	\left \{ \scalebox{0.8}{\tikzfig{interpretations/decoherenced3}} , \quad \scalebox{0.8}{\tikzfig{interpretations/decoherenced4}} , \quad \scalebox{0.8}{\tikzfig{interpretations/decoherenced6}} , \quad \scalebox{0.8}{\tikzfig{interpretations/decoherenced5}} \right \}
\end{equation}
They form a consistent set and therefore one can coarse-grain over these histories. Their probabilities can be calculated using
\[
\tikzfig{interpretations/decoherenced}
\]
%Moreover, one can coarse grain over these histories.

Suppose Alice and Bob both measure in the Z basis; then a consistent set of maximally fine-grained histories would be
\begin{equation}\label{eprhistory2}
	\left \{ \scalebox{0.8}{\tikzfig{interpretations/decoherence7}} , \quad \scalebox{0.8}{\tikzfig{interpretations/decoherence8}} , \quad \scalebox{0.8}{\tikzfig{interpretations/decoherence10}} , \quad \scalebox{0.8}{\tikzfig{interpretations/decoherence9}} \right \}
\end{equation}
According to CQM, sets (\ref{eprhistory}) and (\ref{eprhistory2}) correspond to quantum processes. Combining any branches of these two processes does not yield any branch of a valid process. Hence, the histories in the two sets are inconsistent with one another. % (\ref{eprhistory2}) are not consistent with histories in set (\ref{eprhistory}) because %the maps $\begin{array}{c}
%	\pointmap{0} \vspace{1mm} \\
%	\copointmap{0}
%\end{array}$  and $\begin{array}{c}
%	\pointmap{1} \vspace{1mm} \\
%	\copointmap{1}
%\end{array}$ together with $\begin{array}{c}
%	\pointmap{+} \vspace{1mm} \\
%	\copointmap{+}
%\end{array}$  and $\begin{array}{c}
%	\pointmap{-} \vspace{1mm} \\
%	\copointmap{-}
%\end{array}$, corresponding to Bob's projector, do not form a resolution of the identity. 
Therefore, one is not allowed to combine histories from sets (\ref{eprhistory} and \ref{eprhistory2}) to form a single coarse-grained history.
\end{example}

In a sense, the consistent histories approach responds to the EPR `paradox’~\cite{einstein1935can} and Einstein's concerns about quantum theory and elements of reality~\cite{einstein1936physics} by imposing the single framework (\emph{i.e.}, single set of consistent histories) rule. There are multiple consistent sets of histories that may be \textit{complementary}, but equally real. The set of histories that makes sense for describing a physical system is dictated by the experimental setup, including the measurements that are actually performed. This aligns closely with Bohr's response~\cite{bohr1935can} to the EPR paper.

\begin{remark}
The EPR paper centred on the eponymous question: `Can quantum-mechanical description of physical reality be considered complete?'~\cite{einstein1935can}. We briefly revisit the argument here, adapting it to an example suited to our purposes. 

We borrow the definition of \textit{(elements of) physical reality} from the EPR paper: ``If, without in any way disturbing a system, we can predict with certainty (i.e., with probability equal to unity) the value of a physical quantity, then there exists an element of physical reality corresponding to this physical quantity"~\cite{einstein1935can}. Moreover, the paper gives the following criterion for a \textit{complete theory}: ``every element of the physical reality must have a counterpart in the physical theory"~\cite{einstein1935can}.

Having defined (elements of) reality and completeness, consider two non-commuting operators, each describing a physical quantity of a quantum system. According to standard quantum theory, the knowledge of one physical quantity precludes the knowledge of the other. This means that either: (a) the quantum mechanical description of physical reality is incomplete, or (b) the two physical quantities cannot be simultaneously real. 

Suppose (a) is false. That is, quantum mechanics provides a complete description of reality. Now consider a bipartite entangled system: a Bell state shared between Alice and Bob.
\[
\tikzfig{interpretations/bellb0}
\]
Suppose Alice performs a measurement in the Z basis, with the outcome $ \dpointmap{i} \in \left\{\dpointmap{0}, \dpointmap{1}\right\}$,
\begin{equation}\label{eprcons1}
\tikzfig{interpretations/bell0f}  \ \ = \ \ \tikzfig{interpretations/bell0f2}
\end{equation}
Then, without disturbing Bob's part of the bipartite state, we can predict with certainty that it is a definite Z-basis state $ \dpointmap{i} $. Therefore, it is an element of physical reality according to the EPR definition.  

Conversely, if Alice had measured in the X basis, with the outcome $ \dpointmap{j} \in \left\{\dpointmap{+}, \dpointmap{-}\right\}$,
\begin{equation}\label{eprcons2}
\tikzfig{interpretations/bell0g}  \ \ = \ \ \tikzfig{interpretations/bell0g2}
\end{equation}
then, without disturbing Bob's part of the bipartite state, we would have predicted with certainty that it is a definite X-basis state $ \dpointmap{j} $. Hence, it is also an element of physical reality according to the EPR definition.  

This analysis shows that considering Bob's part of the Bell state, there exist two physical quantities -- described by non-commuting operators -- that are simultaneously real. This implies that (b) is false. 

We showed that assuming (a) to be false implies that the only other alternative, (b), is also false. Therefore, we conclude that (a) is true, \emph{i.e.,} the quantum mechanical description of physical reality is incomplete.\footnote{The EPR argument assumes locality. As stated in the paper, ``... since at the time of measurement the two systems no longer interact, no real change can take place in the second system in consequence of anything that may be done to the first system."~\cite{einstein1935can} Einstein, in particular, desired a \textit{local} additional variable theory of quantum physics~\cite{einstein1949albert}. However, this possibility was ruled out by John Bell's celebrated theorem~\cite{bell1964einstein} and the experimental violations of the Bell inequalities~\cite{scarani2019bell}.}

In response to the EPR argument, a consistent historian would say that Eqs. (\ref{eprcons1}) and (\ref{eprcons2}) correspond to two incompatible frameworks (\emph{i.e.}  consistent sets of histories), given respectively by:
\begin{equation}
\left \{ \scalebox{0.8}{\tikzfig{interpretations/eprcons1}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/eprcons2}} \right \} \quad, \quad \left \{ \scalebox{0.8}{\tikzfig{interpretations/eprcons3}} \quad , \quad \scalebox{0.8}{\tikzfig{interpretations/eprcons4}} \right \} 
\end{equation}
The single framework rule dictates that combining the results of these frameworks is illegitimate. In each experimental run, one must choose a framework based on the measurement \textit{actually} performed by Alice and adhere to it. Essentially, the consistent historian would reject the EPR argument as it combines results from incompatible frameworks, leading to invalid inferences. 
%According to the consistent histories approach, the evolution of quantum systems is described by multiple frameworks that are \textit{complementary} but equally \textit{real}. 
%The choice of a framework is determined by the experimental setup, while combining incompatible frameworks results in erroneous conclusions.
\end{remark}

\subsection{Interpretation or Framework?} 

Consistent histories is considered an interpretation by several of its proponents~\cite{bacciagaluppi2003role}. What is its relation to other interpretations of quantum theory? It has been dubbed a neo-Copenhagen~\cite{omnes2018interpretation} or neo-Everettian~\cite{gell1996quantum} approach by Omnes, and Gellman and Hartle respectively. It is considered similar to the Everettian interpretation because of its emphasis on the reality of different branches. It is deemed a refinement of the Copenhagen interpretation because it takes seriously the idea of complementarity. %\emph{i.e,} one is allowed to stay within a single framework (of consistent histories) while describing quantum phenomena.

The consistent histories interpretation makes precise the idea of complementarity. According to consistent histories, there are complementary but equally real histories that correspond to trajectories of quantum systems. While describing the histories of quantum systems, one needs to stay within a single framework, which is dictated by the experimental setup. For instance, in the Stern-Gerlach setting, one can calculate the probabilities of measurement outcomes in the Z basis or the X basis, depending on how the apparatus is set up. But one cannot meaningfully add up probabilities for measurement outcomes obtained in different bases. 

In the prevalent textbook version of quantum theory---the Copenhagen interpretation---probabilities are invoked when a measurement takes place and they relate to only the measurement outcomes, given by states (such as `pointer' states) of macroscopic devices. The relation of these probabilities with the quantum states that are the subject of measurement is not clear; this is because of the measurement problem~\cite{griffiths2009consistent}. In the many worlds or Everettian interpretation, the wavefunction of a closed system is regarded as real whereas in the consistent histories approach, it is considered merely a calculating device for determining the probabilities of histories that are real~\cite{griffiths2009consistent}. 

%Griffiths reference and how it responds to criticisms by Dowker and Kent. neo-Copenhagen and causality... Grete Hermann a la Bacciagaluppi... Nick...
However, considered as a formalism, the consistent histories approach is interpretation-neutral. It is particularly useful in situations when interference gets suppressed; the time-evolution of the different non-interfering components can be tracked~\cite{bacciagaluppi2003role}.

In the consistent histories interpretation, the consistency condition is imposed by hand in an ad hoc manner (Eq. (\ref{decfunct})); whereas in CQM, consistency is a consequence of the causality of quantum processes -- a more reasonable postulate from a physics perspective. This suggests that using CQM as the standard formalism provides a refinement of the consistent histories interpretation.

%\textcolor{blue}{consistent histories and Bohmian.... see Guido article... and scholssauer 2005? and Zurek 2003} 

%causality and consistent histories a la dodo book \textcolor{red}{IMPORTANT STUFF THERE!!! and a nice slogan too: Causality and consistent histories!!!}

%Nick interpretation


\section{Relational Quantum Mechanics}\label{secRQM}

Inspired by Everett's original relative-state formulation of quantum theory in the eponymous article~\cite{everett1957relative}, relational quantum mechanics (RQM) was proposed in 1996~\cite{rovelli1996relational}. Over the years, the description of the interpretation and its axioms have evolved and been subject to multiple revisions. In this chapter, we follow the version presented in Ref.~\cite{adlam2022information}.

According to RQM~\cite{rovelli1996relational, rovelli2021relational}, ``A quantum event arises in an interaction between two systems such that the values of some physical variables of one system become definite relative to another system''~\cite{adlam2022information}. Not everything is relational in RQM. Even though events are relative in the sense that they happen with respect to another system, they are absolute in the sense of being observer-independent. Any other observer can, in principle, obtain the same information about a relevant variable of the event by interacting with either of the systems involved in the interaction. On the other hand, all quantum states are relative to some observer. In other words, quantum states encode relationships between the aforementioned events and are dependent on the history of the interactions between the observer and the observed system. 

RQM has received a lot of attention. A charge that is levelled against it is that it is merely a vague interpretational layer on top of the usual textbook formulation of quantum theory. Or that it seems to be a philosophical perspective without a concrete mathematical formulation of its own~\cite{martin2021relational, ormrod2024quantum}. In that regard, there have been efforts to devise a mathematical framework for relational quantum mechanics ~\cite{martin2021relational}, as well as a new interpretation~\cite{ormrod2024quantum} that takes inspiration from RQM regarding the relativity of events.

There have been other objections~\cite{laudisa2019open, pienaar2021quintet, brukner2021qubits, stacey2021relational, lawrence2023relative}, some of which have been satisfactorily answered~\cite{adlam2022information, cavalcanti2023consistency}. While criticism of RQM has helped improve and crystallize its ideas, some of the debate around it may stem from the interplay between the standard formalism of quantum theory and the relational statements arising from the interpretation. RQM would benefit from presentation in a formalism that is better suited to relationalism. In other words, there are reasons to think that CQM is an excellent candidate since it was motivated precisely by the key ideas of compositionality and relationalism. 

%The six postulates of RQM, as explained in [], are that (i) events are relative. they can happen with respect to any system; (ii) no hidden variables are involved OR the completeness of unitary quantum physics; (iii) whenever two systems interact, with respect to a third system a correlations is created. this is modelled by a unitary evolution which entangles the two systems with relative to the third system; (iv) the relation between two systems are intrinsic, meaning they do not depend on anything outside the perspectives of the two systems; (v) one can compare accounts of two perspectives only relative to a third system or perspective \textcolor{red}{problematic}; (vi) if a system A measures S followed by B measuring S in the same basis, then if B interacts with A to get information of A's reading, it is found consistent with B's reading.
%briefly discuss the problematic postulate from above with an example similar to one in Rovelli and Adlam paper
%New 6 postulates:

The postulates of RQM are as follows~\cite{adlam2022information}. 

\textbf{RQM1.} \textit{Events (also called facts) are relative. They can happen with respect to any system.}

%\noindent Events are also called facts. 

\textbf{RQM2.} \textit{No hidden or additional variables are needed to complete quantum theory. In other words, unitary quantum physics is complete.}

\textbf{RQM3.} \textit{The relation between two systems is intrinsic, meaning it is not dependent on anything outside the perspectives of the two systems involved.} 

\textbf{RQM4.} \textit{``In a scenario where some observer Alice measures a variable $V$ of a system $S$, then provided that Alice does not undergo any interactions which destroy the information about $V$ stored in Alice’s physical variables, if Bob subsequently measures the physical variable representing Alice’s information about the variable $V$, then Bob’s measurement result will match Alice’s measurement result."}~\cite{adlam2022information} This is called the \textit{cross-perspective links} postulate. 

\textbf{RQM5.} \textit{Whenever two systems interact, they get correlated with respect to a third system. This is modelled by a unitary evolution that potentially entangles the two systems relative to that third system.}

\textbf{RQM6.} \textit{If a system $A$ measures $S$, then a system $B$ measures $S$ in the same basis, then if $B$ interacts with $A$ to get information about $A$'s reading, this information is found to be consistent with $B$'s.}

\begin{remark}
	It has recently been suggested that this postulate is formally supported by Ozawa's intersubjectivity theorem~\cite{ozawa2019intersubjectivity} and may turn out to be redundant~\cite{khrennikov2024ozawa}.
\end{remark}

\begin{remark}\label{eprremark2}
	In RQM, the quantum state of a physical system depends on the reference system or perspective. The state may be different with respect to different systems, especially after measurement or some interaction has taken place. Fortunately, it is possible to reconcile the measurement outcomes and statistics from the different perspectives within this theory. %Otherwise, if two or more observers could not agree on measurement outcomes, it would pose a serious problem for an empirical theory. 
	%Otherwise, if there were no way for two or more observers to agree on measurement outcomes, it would have been a serious problem for an empirical theory. 
	The different systems can interact with one another to get information about measurement outcomes; if they do, the outcomes they find are consistent across perspectives.% if these interactions take place.
\end{remark}

While ideas from RQM have yet to be concretely cast in the language of CQM, some of the related circuit notation is used in Ref.~\cite{cavalcanti2023consistency}. We take guidance from this article and provide elaborate examples of the application of CQM to RQM below, starting with the Wigner's friend thought experiment~\cite{wigner1995remarks}. 
%REFER TO GHZ PAPER AND GIVE A BRIEFEST SUMMARY
%SINGLE SYSTEM MEASUREMENT (friend and Wigner)

\subsection{Wigner's Friend}\label{secRQMWigner}

\begin{example}[]\label{wignerex1}
	In a typical Wigner's friend scenario, there are two people and a quantum system, the state of which is to be measured. One person, Wigner's friend, is inside a lab with the quantum state. The other person, Wigner, is outside the lab. The lab is completely isolated from the outside world. When Wigner's friend measures the quantum state, assuming the universality of quantum mechanics (in the sense that it applies at all scales, particularly to Wigner's friend), two conflicting descriptions of the quantum system arise depending on the two perspectives of Wigner and his friend. 
	
	Let's pick the name Alice for Wigner's friend. Suppose Alice has measured the state of a quantum system given by $\widehat{\psi}$ in the Z basis, and that the state $\widehat{\psi}$ is not a pointer state in the Z basis, \emph{i.e.}, $0$ or $1$. From Alice's perspective, the measurement gives a definite outcome: either $0$ or $1$, for which the probabilities are respectively given by 
	\[
	\tikzfig{interpretations/RQMb1b}	\quad \quad \quad \quad 	\tikzfig{interpretations/RQMb1c}
	\]
	Diagrammatically, the measurement of the state can be represented as 
	\begin{equation}\label{wignerstat}
	\tikzfig{interpretations/RQMb1}
	\end{equation}
where the classical, thin wire represents the probability distribution of the definite measurement outcomes.

	From Wigner's perspective, as a result of the measurement interaction, Alice's state gets entangled with the state of the quantum system. This is modelled by an entangling unitary interaction $\widehat U$ between the state that is measured and Alice's state $R$ (R standing for the `ready' state).
	\[
\tikzfig{interpretations/decoherenceb}
	\]
This is direct application of postulate (\textbf{RQM5}). One can see that after Alice has performed the measurement, the state of the quantum system with respect to Alice is different from that with respect to Wigner. For Alice, the state of the quantum system is collapsed to a definite state whereas for Wigner, the state of the quantum system is entangled with Alice's state.
	
If Wigner measures Alice's state in the Z basis, \emph{i.e.} the same basis Alice measured the state of the quantum system in, he gets a definite outcome, $0$ or $1$, for which the probabilities can be calculated as 
\[
\tikzfig{interpretations/RQMb2b2}	\quad \quad \quad \quad 	\tikzfig{interpretations/RQMb2b3}
\]
Wigner's measurement of Alice's state is represented by the diagram
\begin{equation}\label{wigner1eq}
\tikzfig{interpretations/RQMb2}
\end{equation}
Postulate (\textbf{RQM4}) ensures that the measurement outcome matches that of Alice's measurement of the quantum system.

Instead of measuring Alice's state, Wigner could have measured the state of the quantum system in the Z basis.
\begin{equation}\label{wigner2eq}
\tikzfig{interpretations/RQMb3}
\end{equation}
Thanks to postulate (\textbf{RQM6}), this measurement outcome matches Alice's measurement result of the same quantum system.
\end{example}

\begin{convention}
	In the above example, for the sake of simplicity, we ascribed pointer states to macroscopic observers/agents. One can replace human observers with individual qubits without changing the conceptual content of the example. This is because RQM considers quantum theory to be universally applicable, and defines measurement in a non-anthropic manner. The same argument applies to Everettian quantum theory. We shall use this convention throughout the chapter. 
\end{convention}

\begin{remark}\label{wignercorrel}
As an illustration, one can provide a more granular analysis of the above example by defining the unitary process $\widehat U$ and the ready state $R$% as in Eq. (\ref{dectake2b}):
\begin{equation}\label{wignerdef}
	\tikzfig{interpretations/decoherenceb2b} \quad \quad \quad \quad \tikzfig{interpretations/decoherenceb2c} 
\end{equation}
\emph{i.e.}, the ready state is $0$ and the unitary is a CNOT gate where the left qubit is the target controlled by the right one. Substituting Eq. (\ref{wignerdef}) in Eq. (\ref{wigner1eq}), we get
\[
\scalebox{0.8}{\tikzfig{interpretations/RQMb2b}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb2c}} \ \ \overset{(f)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb2d}} \ \ \overset{(id)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb2e}} 
\]
\[
\ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb2f}} \ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb2g}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb1}}
\]
which is the same probability distribution as the one in diagram (\ref{wignerstat}). This means that after Alice has performed the measurement of the quantum system, if Wigner measures Alice's state in the same basis, the measurement statistics are the same as those of Alice's measurement of the quantum system. Postulate (\textbf{RQM4}) ensures that the individual measurement outcomes agree as well. Likewise, substituting Eq. (\ref{wignerdef}) in Eq. (\ref{wigner2eq}), we have
\[
\scalebox{0.8}{\tikzfig{interpretations/RQMb3b}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb3c}} \ \ \overset{(f)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb3d}} \ \ \overset{(id)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb3e}} 
\]
\[
\ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb3f}} \ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb3g}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/RQMb1}}
\]
which is again the same probability distribution as the one in diagram (\ref{wignerstat}). This implies that, even though the state of the quantum system differs for Alice and Wigner after Alice performs the measurement, the statistics of Alice's measurement and Wigner's subsequent measurement will be the same, provided the measurements are performed in the same basis. 
%This implies that even though the state of the quantum system is different with respect to Alice and Wigner after Alice has performed the measurement, the statistics of Alice's measurement and Wigner's subsequent measurement of the quantum system is the same provided the measurements are performed in the same basis. 
Postulate (\textbf{RQM6}) makes sure that the individual measurement outcomes of Alice and Wigner agree as well. 

To sum up, CQM analysis shows that the statistics of Alice's measurement (from her perspective) agree with those of Wigner's subsequent measurement of Alice's state in the same basis (from his perspective). 
%To sum it up, CQM analysis shows that the statistics of Alice's measurement (from Alice's perspective) agrees with the statistics of Wigner's subsequent measurement of Alice's state in the same basis (from Wigner's perspective). 
Moreover, Alice's measurement statistics (from her perspective) are consistent with Wigner's subsequent measurement of the quantum state in the same basis (from his perspective). 
%Moreover, Alice's measurement statistics (from Alice's perspective) agrees with the statistics of Wigner's subsequent measurement of the quantum state in the same basis (from Wigner's perspective). 
Postulates (\textbf{RQM4}) and (\textbf{RQM6}) dictate that the individual measurement outcomes agree as well. After Alice's measurement and before Wigner's interaction with either Alice or the quantum system, the state of the quantum system differs from the perspectives of Alice and Wigner.
%After Alice's measurement and before Wigner's interaction with Alice or the quantum system, the state of the quantum system is different relative to Alice and Wigner.
\end{remark}

\begin{remark}[Decoherence in RQM]
	In RQM, decoherence arises as a result of interactions with environmental states but an observer has to be specified relative to whom decoherence takes place. With respect to any observer, if an environmental variable, say the state $R$, interacts with a quantum state $\widehat{\psi}$, the state $R$ gets entangled with $\widehat{\psi}$ via a unitary interaction:
	\[
	\tikzfig{interpretations/decoherenceb}
	\]
	Since the observer has no access to the environmental variable, we have
	\[
	\tikzfig{interpretations/decoherenceb2} 
	\]
	Substituting definitions from Eq. (\ref{wignerdef}) into this diagram gives
	\[
	\scalebox{0.8}{\tikzfig{interpretations/decoherenceb2e}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f}} \ \ \overset{(f)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f2}} 
	\]
	\[
	\ \ \overset{(id)}{=} \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f3}} \ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f4}} \ \ \overset{(f)}{=}  \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherenceb2f5}} \ \ = \ \ \scalebox{0.8}{\tikzfig{interpretations/decoherencee2}}
	\]
\end{remark}

\begin{remark}
The Wigner's friend experiment as described in Example \ref{wignerex1} may seem idealistic to us because there is no mention of decoherence in the experiment. This is an important criticism, particularly on two counts: first, if Alice is a person (and not a photon as in Ref.~\cite{bong2020strong}), there are multiple interactions between Alice and the environmental variables to which Wigner has no access. Secondly, one cannot completely isolate a lab from the rest of the physical universe. In other words, there will always be some interactions between environmental variables inside the lab and those outside the lab. 
\end{remark}

In the example below, we provide a more realistic account of the Wigner's friend experiment by introducing decoherence. 

\begin{example}[Wigner's friend and decoherence]
	Nothing changes from Alice's perspective. She measures the quantum system and sees a definite outcome. The measurement statistics are given by 
	\[
		\tikzfig{interpretations/RQMb1}
	\]
	However, with respect to Wigner, Alice's state gets entangled with the quantum state. Moreover, since Alice is a macroscopic system\footnote{For simplicity, we use a pointer state for Alice, whose macroscopicity is accounted for by environmental decoherence.}, her interactions with the environment lead to decoherence.
	\begin{equation}\label{RQMwigdec1}
	\tikzfig{interpretations/RQMc1}
	\end{equation}
	where $\widehat{U}_{A\widehat{\psi}}$ is a unitary entangling Alice's state $R_A$ with the state $\widehat{\psi}$, and $\widehat{U}_{EA}$ entangles Alice's state (after it is entangled with $\widehat{\psi}$) with the environment state $R_E$. Plugging the following definitions in diagram (\ref{RQMwigdec1})
	\[
		\tikzfig{interpretations/RQMc2}  \quad 	\tikzfig{interpretations/RQMc3}
	\]	
	\[		\tikzfig{interpretations/RQMc4} \quad 	\tikzfig{interpretations/RQMc5}
	\]
	we have\footnote{The environment, Alice and the quantum system undergoing measurement are denoted respectively by E, A and Q in grey.} 
	\[
	\scalebox{0.8}{\tikzfig{interpretations/RQMc6}} \ = \ 	\scalebox{0.8}{\tikzfig{interpretations/RQMc7}}  \ \overset{(f)}{=}  \ \scalebox{0.8}{\tikzfig{interpretations/RQMc8}} \
 \overset{(id)}{=}  \ \scalebox{0.8}{\tikzfig{interpretations/RQMc9}}
 \]
 \[
   \overset{(f)}{=}  \ \scalebox{0.8}{\tikzfig{interpretations/RQMc10}}  \ \overset{(f)}{=}  \  \scalebox{0.8}{\tikzfig{interpretations/RQMc10b}} 
	\overset{(f)}{=}  \  \scalebox{0.8}{\tikzfig{interpretations/RQMc11}} \ 	= \ \scalebox{0.8}{\tikzfig{interpretations/RQMc12}} 
	\]
The last diagram shows that a non-demolition measurement of the quantum state has been performed. The classical outcome goes to Alice and is encoded as a quantum state. %This means that with respect to Wigner, Alice's state is a mixture, corresponding to Wigner's ignorance of the outcome of Alice's measurement.
This means that, from Wigner's perspective, Alice's state is a mixture, reflecting Wigner's ignorance of the outcome of Alice's measurement.

\[
\tikzfig{interpretations/RQMc13} \ 	\overset{(f)}{=}  \  \tikzfig{interpretations/RQMc14} \ = \ \tikzfig{interpretations/RQMc15}
\]
By a similar argument, the state of the quantum system is also a mixed state. 
\[
\tikzfig{interpretations/RQMc16} \ 	\overset{(f)}{=}  \  \tikzfig{interpretations/RQMc17} \ 	\overset{(f)}{=} \ \tikzfig{interpretations/RQMc18} \ 	\overset{(f)}{=}  \ \tikzfig{interpretations/RQMc19}
\]
However, the two mixtures are classically correlated:
\[
\tikzfig{interpretations/RQMc12} \ 	\overset{(f)}{=}  \  \tikzfig{interpretations/RQMc20}  \ 	\overset{(f)}{=}  \  \tikzfig{interpretations/RQMc21} 
\]
Above, in the rightmost diagram, after the quantum state is measured, the measurement outcome is copied and then the two copies are encoded as quantum states; the left one corresponds to Alice's state and the right one to that of the quantum system. It is straightforward to verify that the measurement statistics are the same as those calculated in Remark \ref{wignercorrel}.
\end{example}

\subsection{The EPR-Bell Scenario}\label{secRQMEPR}

\begin{example}\label{RQMeprex}
	
To give a relational account of the EPR-Bell scenario, in addition to Alice and Bob between whom a Bell state is shared, we consider an additional observer, Charlie. Before any measurement is performed, the bipartite state is given by
\begin{equation}\label{epreq1}
	\tikzfig{interpretations/bell0}
\end{equation}
with respect to every observer.	When both Alice and Bob perform measurements, they each see a different bipartite state. With respect to Alice, the state is given by
\begin{equation}\label{epreq2}
\tikzfig{interpretations/bell4a}
\end{equation}
where the unitary $\widehat{U}_{\Phi}$ represents Alice's setting of the measurement basis and $\widehat{U}_{B_{\Psi} R}$ represents an entangling unitary interaction between Bob's part of the Bell state and Bob's pointer state $R$.   

Here, Alice obtains a unique outcome from her measurement and there is no entangling interaction between Alice and the state. The statistics of the unique measurement outcome are available as classical information denoted by the thin wire. On the other hand, 
Bob's pointer state $R$ gets entangled with his part of the Bell state. Now, Alice can interact with Bob to obtain information of his measurement, resulting in a `collapse' and hence a single outcome. The wire corresponding to the original state is discarded in the process and a measure operation results in a thin wire on Bob's side.
\begin{equation}\label{relepr1}
\tikzfig{interpretations/bell4a2}
\end{equation}
As an illustration, the diagram can be further characterised by plugging in the following sub-diagrams: 
\begin{equation}\label{releprb2}
\tikzfig{interpretations/decoherenceb2b} \quad \quad \tikzfig{interpretations/bell4a3}
\end{equation}
where the entangling unitary includes a CNOT gate in which the first wire is the control and the second wire the target. The unitary $\widehat{U}_{\Psi}$ corresponds to the setting of Bob's measurement basis. %\textcolor{red}{make the symbols of basis unitaries consistent. Compare with the previous ones in this chapter.} 
%\textcolor{red}{reconsider entangling unitary: should there be another basis unitary (adjoint of the current one above the CNOT gate?)}
%where the entangling unitary operation is defined as application of Bob's measurement basis $\Phi$ followed  
Diagram (\ref{relepr1}) becomes
\[
\scalebox{0.8}{\tikzfig{interpretations/bell4a4}} \ = \ \scalebox{0.8}{\tikzfig{interpretations/bell4a4b}} \ \overset{(f)}{=}  \  \scalebox{0.8}{\tikzfig{interpretations/bell4a5}}  
\]
\[
 \overset{(id)}{=}  \ \scalebox{0.8}{\tikzfig{interpretations/bell4a6}}  
\overset{(f)}{=}  \ \scalebox{0.8}{\tikzfig{interpretations/bell4a7}}  \ \overset{(f)}{=}  \ \scalebox{0.8}{\tikzfig{interpretations/bell4a8}} 
\]
The diagram on the right-hand side above represents the measurement statistics from Alice's perspective after Alice and Bob have performed their respective measurements, setting measurement bases using unitaries $\widehat U_{\Phi}$ and $\widehat U_{\Psi}$, and Alice's subsequent interaction with Bob to measure his state. 

We can give a similar analysis of Bob's perspective. With respect to Bob, the bipartite state after Alice's and Bob's measurement of their respective systems is
\begin{equation}\label{epreq3}
\tikzfig{interpretations/bell4b}
\end{equation}
It can be shown that after Bob measures Alice's state, 
\begin{equation}\label{epreq3b}
	\tikzfig{interpretations/bell4b2}
\end{equation}
using definitions similar to those in Eq. (\ref{releprb2}), the measurement statistics of the bipartite system from his perspective can be simplified to the diagram
\begin{equation}\label{epreq4}
\tikzfig{interpretations/bell4a8} 
\end{equation}
which is the same as that from Alice's perspective.
	
From Charlie's perspective, both Alice's and Bob's states get entangled with their respective parts of the bipartite system as they perform measurements. 	
%Consider the EPR-Bell scenario with respect to Wigner, when Alice (A) and Bob (B) make measurements in the $\Phi$ and $\Psi$ bases, respectively. With respect to Wigner, each party's measurement results in entanglement of their pointer R with their part of the Bell state. This entanglement is via a unitary process $U...$.
\begin{equation}\label{epreq5}
\tikzfig{interpretations/bell4}
\end{equation}
%\textcolor{red}{MAYBE REVISE LABELS OF ALL BOXES IN THIS SECTION}
Once Charlie has measured both Alice's and Bob's states, resulting in the diagram
\begin{equation}\label{epreq6}
\tikzfig{interpretations/bell4c} 
\end{equation}
it can be shown that he gets the same measurement statistics as those from Alice's and Bob's perspectives.
\end{example}

\begin{remark}\label{eprremark1}
	In the above example, the initial state was given by diagram (\ref{epreq1}) with respect to every observer. When Alice and Bob performed measurements, the state became diagrams (\ref{epreq2}), (\ref{epreq3}), and (\ref{epreq5}) with respect to Alice, Bob and Charlie respectively. After interactions between the observers, the measurement statistics were represented by diagrams (\ref{relepr1}), (\ref{epreq3b}), and (\ref{epreq6}) with respect to Alice, Bob, and Charlie respectively. It was then shown that these diagrams are reducible to diagram (\ref{epreq4}).
		\[
	\tikzfig{interpretations/bell4a8}
	\]
	 This diagram gives the perspective-independent information flow structure of the EPR-Bell scenario. This diagram corresponds to the standard textbook version of quantum theory, which is non-relational in the sense of RQM. The Bell state is measured by Alice and Bob after setting the measurement bases using unitaries $\widehat U_{\Phi}$ and $\widehat U_{\Psi}$ respectively, and there are definite measurement outcomes. In RQM, this diagram is not part of anyone's perspective immediately after Alice's and Bob's measurements of their respective systems.
\end{remark}
%\textit{"In a scenario where some observer Alice measures a variable V of a system S, then provided that Alice does not undergo any interactions which destroy the information about V stored in Alice’s physical variables, if Bob subsequently measures the physical variable representing Alice’s information about the variable V, then Bob’s measurement result will match Alice’s measurement result."}
%According to this postulate, the measurement outcomes in diagrams W, A and B are consistent....
%In the above examples we have performed calculations using the ZX-calculus to show 

Through the preceding examples, we have shown that within RQM, in situations in which interactions involving cross-perspective links take place, the measurement statistics are found to be consistent across perspectives.

%Next, we look at the quantum teleportation protocol from a relational perspective.

\subsection{Quantum Teleportation}\label{secRQMteleport}

\begin{example}\label{telex}

First, we briefly give an account of quantum teleportation without resorting to relational descriptions. The teleportation of a quantum state $\widehat{\psi}$ from one party, called Alice, to another, called Bob, requires a Bell state shared between the two parties. The party that has the state $\widehat{\psi}$ measures this state and their part of the Bell state in the Bell basis. This measurement results in one of four possible outcomes, which is transmitted via a classical channel to the other party. The other party then applies one of four possible unitary maps (depending on the classical information received from the other party) to their part of the Bell state. This results in the teleportation of $\widehat{\psi}$  from the first party to the second party. In standard CQM~\cite{CKbook}, this can be represented by the equation:
	\[
	\tikzfig{interpretations/RQMtele3} 	\ = \ 	\tikzfig{interpretations/RQMtele3f} 	
	\]
where the thin wires represent the classical channel through which two bits of information are transmitted; the Bell-basis measurement and the controlled unitary map are given by 	
	\[
	 \tikzfig{interpretations/RQMtele4} \ := \  	\ \tikzfig{interpretations/RQMtele5} \quad , \quad \quad  \tikzfig{interpretations/RQMtele6} \ := \  	\ \tikzfig{interpretations/RQMtele7}
\]
Therefore, we have %the left-hand side of the teleportation equation is simplified as follows:
	\[
\scalebox{0.8}{\tikzfig{interpretations/RQMtele8}} %\tikzfig{interpretations/RQMtele9} \
 \overset{(f)}{=} \ 
\scalebox{0.8}{\tikzfig{interpretations/RQM11}}
\overset{(f)}{=} \  \scalebox{0.8}{\tikzfig{interpretations/RQM12}}
\]

\[  \overset{(\ref{spchop})}{=} \ 
\scalebox{0.8}{\tikzfig{interpretations/RQMtele13}}
%show intermediate (sub)calculation 
\overset{(id)}{=} \  \scalebox{0.8}{\tikzfig{interpretations/RQMtele14}}
\ \overset{(f)}{=}  \ \quad \quad \quad \quad 
\scalebox{0.8}{\tikzfig{interpretations/RQMtele15}}
\]

\begin{equation}\label{eqtele1}
 \overset{(\ref{spchop})}{=} \ \quad \quad \quad \quad \quad \quad  \scalebox{0.8}{\tikzfig{interpretations/RQMtele16}} \  \overset{(id)}{=}   \ 
\scalebox{0.8}{\tikzfig{interpretations/RQMtele18}}
\end{equation}
%Hence, we have verified, and can also represent, the teleportation protocol as the following identity
%\begin{equation}\label{eqtele1}
%\tikzfig{interpretations/RQMtele8} \ = \ 
%\tikzfig{interpretations/RQMtele18}
%\end{equation}
\noindent In RQM, the above diagrams correspond exactly to Alice's perspective of teleportation. With respect to Alice, the protocol starts with Alice's joint measurement of the state $\widehat{\psi}$ and her part of the Bell state in the Bell basis. As a result of this measurement, Alice sees a definite outcome, which is one of the four possible outcomes. 
\[
 \tikzfig{interpretations/RQMtele5}	
\]	
She then transmits this information to Bob who applies the corresponding unitary transformation on his subsystem of the Bell state. 
\[
\tikzfig{interpretations/RQMtele7}
\]	
Apart from adding a phrase like `with respect to Alice', the description is exactly the same as that in the usual textbook description. This is because the description of this protocol is in terms of definite measurement outcomes. In the teleportation protocol, only Alice performs a measurement. When we discuss Alice's perspective in RQM, Alice sees a definite measurement outcome. Bob's perspective, on the other hand, is more involved.

With respect to Bob, when Alice performs the joint measurement, there is an entangling interaction between two of her ready states $R_1$ and $R_2$, the target state $\widehat{\psi}$ and her part of the Bell state via a unitary interaction.  	
%\[
%\tikzfig{interpretations/RQM39b}
%\]	
\[
\tikzfig{interpretations/RQM39c}
\]	
This entangling unitary involves three CNOT gates. The first CNOT gate from the bottom sets the Bell basis as Alice's measurement basis. The next two CNOT gates entangle  $R_1$ with $\widehat{\psi}$, and $R_2$ with Alice's part of the Bell state. 
%\textcolor{red}{ready states as $\ket{R_1}$  or $\ket{R_1}\bra{R_1}$. Check that these notations are consistent for other states too.}
Teleportation requires definite outcomes of Alice's measurement and Bob needs to know these outcomes to be able to apply the relevant unitary transformation at this side. Bob can find out Alice's outcome by interacting with Alice.
%\[
%\tikzfig{interpretations/RQM39}
%\]	
\[
\tikzfig{interpretations/RQM39d}
\]	
%	\[
%	\tikzfig{interpretations/RQMtele19}
%	\]
%	\[
%	\tikzfig{interpretations/RQM38}
%	\]
The rest of the explanation is the same as that from Alice's perspective.	So the complete diagram of the protocol is 
	%\[
	%\tikzfig{interpretations/RQMtele20}
	%\]
		\[
	\tikzfig{interpretations/RQMtele20c}
	\]
Defining the ready states as $\  \tikzfig{interpretations/RQMc2b}  \quad 	\tikzfig{interpretations/RQMc3b}\ $, we can simplify the diagram as follows:	
	\[
		\scalebox{0.75}{\tikzfig{interpretations/RQMtele20d}}
%\tikzfig{interpretations/RQMtele21b}
\ \ \ \overset{(f)}{=} \ \ \ 
\scalebox{0.75}{\tikzfig{interpretations/RQMtele23b}} 
\overset{(id)}{=} \ \ \ 
\scalebox{0.75}{\tikzfig{interpretations/RQMtele24b}}
\]
\[
= \ \ \ 
\scalebox{0.75}{\tikzfig{interpretations/RQMtele25b}}
\overset{(f)}{=} \ \ \ 
\scalebox{0.75}{\tikzfig{interpretations/RQMtele26b}}
\ \ \ \overset{(f)}{=}  \ \ \ 
\scalebox{0.75}{\tikzfig{interpretations/RQMtele27b}} 
\]
\[
 \overset{(\ref{eqtele1})}{=}  \ \ \  %\tikzfig{interpretations/RQMtele17} 
	\scalebox{0.75}{\tikzfig{interpretations/RQM37}}
\]

\begin{comment}
	\[
	\tikzfig{interpretations/RQMtele21}
	\ \ \ \overset{(f)}{=} \ \ \ 
	\tikzfig{interpretations/RQMtele23} 
	\]
	\[
	\overset{(id)}{=} \ \ \ 
	\tikzfig{interpretations/RQMtele24}
	\ \ \ = \ \ \ 
	\tikzfig{interpretations/RQMtele25}
	\]
	\[
	 \overset{(f)}{=}  \ \ \ 
	\tikzfig{interpretations/RQMtele26}
	\ \ \ \overset{(f)}{=}  \ \ \ 
	\tikzfig{interpretations/RQMtele27}
	\] 
	
	\[
	\overset{(\ref{spchop})}{=}  \ \ \ 
	\tikzfig{interpretations/RQMtele28} \ \	\ 	 \overset{(f)}{=} \ \ \ 
	\tikzfig{interpretations/RQM29}
	\]
	
	\[
		 \overset{(f)}{=} \ \ \ 
	\tikzfig{interpretations/RQM30}
	 \ \ \  \overset{(\ref{spchop})}{=} \ \ \ 
	\tikzfig{interpretations/RQM31}
	\ \ \ \overset{(c)}{=} \ \ \ 
	\tikzfig{interpretations/RQM32}
	\]
	
	\[
	 \overset{(f)}{=}  \ \ \ 
	\tikzfig{interpretations/RQM33}
	 \ \ \  \overset{(id)}{=}  \ \ \ 
	\tikzfig{interpretations/RQM34}
	\]
\end{comment}	
	\noindent which shows that the state $\widehat{\psi}$ has been teleported to Bob. Therefore, the above calculation represents teleportation from Bob's perspective.
	%\[
	%\tikzfig{interpretations/RQMtele20b}
	%\ \ = \ \ 
	%\tikzfig{interpretations/RQM37}
	%\]
\end{example}
%where
%	\[
%\tikzfig{interpretations/RQMc2b}  \quad 	\tikzfig{interpretations/RQMc3b}
%\]		

The above example shows that, in RQM, the differences in wavefunctions from different perspectives arise when measurements take place. 

\begin{remark}
From an RQM perspective, the teleportation protocol (Example \ref{telex}) differs from the EPR-Bell scenario (Example \ref{RQMeprex}) in that the former involves Alice making a measurement and Bob applying a controlled unitary map. The measurement outcome and the control of the unitary map are connected. As Bob is not making a measurement, the part of the diagram corresponding to Bob's side looks the same from both Alice's and Bob's perspectives. 

On the other hand, both Alice and Bob make measurements in the EPR-Bell scenario (Example \ref{RQMeprex}). That is why there is a reciprocity in the wavefunctions from Alice's and Bob's perspectives. From Alice's perspective, Alice sees a single outcome of her measurement and Bob's state gets entangled with the state he measures. Bob's perspective is reciprocal with this.
\end{remark}

\begin{remark}
From a relational perspective, the teleportation example is interesting in another way too. In the EPR-Bell scenario (Example \ref{RQMeprex}), as discussed in Remarks (\ref{eprremark1}) and (\ref{eprremark2}), we saw that the state does not remain the same from different perspectives when measurement is involved. The measurement statistics are the same when there is interaction between the different observers. In the teleportation protocol (Example \ref{telex}), the overall diagram is that of a state and it was shown that the state is the same (\emph{i.e.,} the teleported state) with respect to both Alice and Bob. Why is it the case, especially given that Alice performs a measurement in this protocol? The explanation is as follows: teleportation requires that there is interaction between Alice and Bob after Alice's measurement. This implies that the measurement statistics of Alice's measurement are the same from both Alice's and Bob's perspectives. These statistics are then used to control a unitary map at Bob's system. Alice's measurement, her interaction with Bob, and Bob's controlled unitary operation ensure that the state $\widehat{\psi}$ is teleported. In other words, Alice's interaction with Bob and Bob's unitary map, which is dependent on Alice's measurement outcome, counteract the effect of measurement on the overall quantum state. Therefore, the state is the same from both Alice's and Bob's perspective.
\end{remark}

\subsection{Measuring the GHZ State}\label{secRQMGHZ}

An analysis of measurements of the GHZ state within RQM was presented in Ref.~\cite{cavalcanti2023consistency}. In the example below, we show diagrammatically how measurement appears from different perspectives within RQM. 

\begin{example}%[Measurements of the GHZ state]
The GHZ state comprises three states that are entangled. As three states are to be measured, we need at least three observers or three perspectives. Let's call them Alice (A), Bob (B) and Charlie (C). Before measurements take place, the state is
%\[
%\tikzfig{interpretations/GHZ0}
%\]
\[
\tikzfig{interpretations/GHZ0b}
\]
with respect to all observers. When the three observers perform measurements, the joint state with respect to Alice is as follows.
\[
\tikzfig{interpretations/GHZ14b}
\]
where the unitary $\widehat{U}_{\alpha}$ sets Alice's measurement basis. Alice sees a definite outcome but Bob's and Charlie's states ($R_B$ and $R_C$) get entangled via unitary interactions $\widehat{U}_{R_B B_{\beta}}$ and $\widehat{U}_{R_C C_{\gamma}}$ with their respective parts of the GHZ state.
%$\alpha$, $\beta$ and $\gamma$ respectively
Alice can then interact with Bob and Charlie to find out their measurement outcomes. %This results in the diagram:
\[
\tikzfig{interpretations/GHZ14}
\]
We can give similar diagrams for Bob's and Charlie's perspectives. Using analysis similar to that in Example \ref{RQMeprex}, it can be shown that after Alice, Bob and Charlie perform measurements and there have been interactions between the different observers (such as, from Alice's perspective, between Alice and Bob, and Alice and Charlie), the following joint measurement statistics are obtained for each perspective.
\begin{equation}\label{ghzflow}
\tikzfig{interpretations/GHZ3}
\end{equation}
This diagram depicts the structure of information flow of the joint measurement of a GHZ state after setting measurement bases using the unitary processes $\widehat U_{\alpha}$, $\widehat U_{\beta}$, and $\widehat U_{\gamma}$. Note that in RQM, there is no perspective in which this diagram is obtained as a result of measurements by Alice, Bob, and Charlie of their respective parts of the GHZ state only; there has to be interactions between the three observers as well.

In addition to Alice, Bob, and Charlie, there could be a fourth observer, say Wigner, who does not perform any measurement. With respect to Wigner, when Alice, Bob and Charlie perform measurements, the state of the joint system is given by 
\[
\tikzfig{interpretations/GHZ5b}
\]
Now Wigner interacts with each of the three other observers to find out their measurement outcomes. The joint state then becomes
\[
\tikzfig{interpretations/GHZ5}
\]
which can again be simplified to diagram (\ref{ghzflow}) using definitions like those in Example \ref{RQMeprex}.% and (\ref{telex}).
\end{example}

\begin{remark}
	The above example shows that in a scenario involving measurements of a GHZ state, different observers see different states of the joint system right after measurement; but once there are interactions between the different observers, the measurement statistics agree across the different perspectives. This means that one can do a proof of the GHZ nonlocality theorem~\cite{CKbook} within RQM. One needs to pick an observer's perspective and then ensure that this observer interacts with all the observers after they have made their respective measurements. The rest of the proof is the same as that in the textbook~\cite{CKbook}. In fact, the textbook proof uses a non-relational approach that works directly with the information-flow structure of the GHZ state and its measurements. In RQM, this information flow structure is not a primitive and has to be derived after interactions between the different observers are introduced.
\end{remark}

\section{Everettian Quantum Mechanics}\label{secEverett}

In this section, by Everettian quantum mechanics, we mean the original `relative-state' interpretation of quantum mechanics as proposed by Hugh Everett III in the paper~\cite{everett1957relative} based on his doctoral dissertation~\cite{dewitt1973many}. One of the main motivations of this interpretation was the question: how do we apply \textbf{MP2} and \textbf{MP3} to an isolated system comprising a measuring system and a quantum system whose state is to be measured. According to standard quantum theory, measurement results in collapse of the measured state and hence yields definite outcomes, whereas the state of a system evolves unitarily in the absence of measurement. When the measuring system interacts with the quantum system to perform a measurement, it should obtain a definite outcome of the measurement. In other words, there is a definite state of the measured system. However, the joint state of the two systems should evolve unitarily according to quantum theory; and, in such a case, we cannot say that the measurement yields a definite state of the measuring system or the measured system. Therefore, there is a conflict between the two descriptions of the composite system provided by standard quantum theory.

Another motivating question for this interpretation is how to apply quantum theory to the whole universe. The mainstream (Copenhagen) version of quantum theory requires an `observer' for a measurement to take place so that there is a definite state of the observed system. Assuming that the universe is a closed system and there is no observer outside it, it is unclear how a measurement or measurement-like interaction could be applied to it. 

Everettian quantum mechanics discards the collapse postulate of standard quantum theory and interprets unitary evolution in terms of \textit{absolute} and \textit{relative} states. As Everett remarks, ``There does not in general exist anything like a single state for one subsystem of a composite system. Subsystems do not possess states that are independent of the states of the remainder of the system, so that the subsystem states are generally correlated with one another. One can arbitrarily choose a state for one subsystem, and be led to the relative state for the remainder. Thus we are faced with a fundamental \textit{relativity of states}, which is implied by the formalism of composite systems. It is meaningless to ask the absolute state of a subsystem one can only ask the state relative to a given state of the remainder of the subsystem.''~\cite{everett1957relative}

%\textcolor{red}{single or double quote? make it consistent throughout the thesis.}

We give a diagrammatic exposition of the ideas of this interpretation through examples.

\begin{example}[A measuring device and a quantum system]\label{eqmex1}
	Consider a composite system comprising a measuring device (with state $R$) and a quantum system (with state $\widehat{\psi}$) that is to be measured.\footnote{In Everettian quantum theory, every system is a quantum system. For the sake of simplicity, we use the term `quantum system/state' to refer to systems/states whose measurement is under discussion.} The composite state is given by\footnote{The measuring device and the quantum system undergoing measurement are denoted respectively by M and Q in grey.}    
\[
\tikzfig{interpretations/everettb}
\]	
A measurement is an interaction between $R$ and $\widehat{\psi}$ that produces correlations between the two systems. This process results in possible entanglement of the two systems via a unitary interaction $\widehat U$. 
	\[
\tikzfig{interpretations/everettbb}
\]	
The diagram above gives the absolute state of the composite system after the measurement. If this is an entangled system, one cannot talk about a definite measurement outcome. According to the Everettian interpretation, it does not make sense to talk about the absolute state of the subsystems after a measurement has taken place. One can however talk about the relative states. For example, one can ask what is the state of one subsystem relative to a particular state of the other subsystem. These relative states correspond to definite measurement outcomes. 

How do we find the state of the measuring system relative to a particular state of the object system? The state of the measuring system relative to the state $i$ of the measured system can be calculated as
\begin{equation}\label{everettb2b}
\tikzfig{interpretations/everettb2b}
\end{equation}
%\textcolor{red}{use a similar argument in RQM???}
\noindent Reciprocally, the state of the quantum system relative to the state $i$ of the measuring system is given by
\begin{equation}\label{everettb3b}
\tikzfig{interpretations/everettb3b}
\end{equation}		
\end{example}

\begin{remark}\label{remarkeverett}
To make the above example more specific, consider for illustration, the following definitions of the ready state, the unitary operation and the quantum-system state:
\[
	\tikzfig{interpretations/decoherenceb2b} \quad \quad \quad \tikzfig{interpretations/decoherenceb2c}  \quad \quad \quad \tikzfig{interpretations/everettb4}
\]
Then the state of the measuring system relative to the state $i$ of the quantum system is given by 
\[
\tikzfig{interpretations/everettb2b} \ = \ \tikzfig{interpretations/everettb5}
 \ \overset{(f)}{=} \   \tikzfig{interpretations/everettb6}  \ \overset{(id)}{=} \  \tikzfig{interpretations/everettb7}  \ = \  \tikzfig{interpretations/everettb8} 
\]
\noindent One can also calculate the state of the quantum system relative to a particular state of the measuring system. The composite system however has an absolute state given by 
\[
\tikzfig{interpretations/everettb2b2} \ = \ \tikzfig{interpretations/everettb5b}
\ \overset{(f)}{=} \   \tikzfig{interpretations/everettb6b}  \ \overset{(id)}{=} \  \tikzfig{interpretations/doubled_cupb} 
\]
\noindent We picked the object state to be $+$, the superposition of states $0$ and $1$. The initial state of the measuring system was $0$. During the measurement, the state of the measuring system became entangled with the object state via a CNOT gate. After the measurement, there is no absolute state of the measuring system or the measured system; they have multiple relative states. On the other hand, the composite system has a single absolute state.  
\end{remark}

\begin{remark}
	The above example shows that, after a measurement, there is a single absolute state of the composite system, whereas there may be multiple relative states of its subsystems. These relative states are indexed by the outcomes of measurements. Therefore, measurements give rise to \textit{branching} of the state of the measuring system. This leads to the idea of many worlds~\cite{vaidman2002many, dewitt1973many}, a popular way to think of Everettian quantum mechanics.  
\end{remark}

\begin{remark}
	%In Everettian quantum theory, the overall state evolves unitarily and every possible outcome takes place on each measurement. 
	In Everettian quantum theory, the overall state evolves unitarily, and every possible outcome occurs with each measurement. 
	However, for subsystems or observers that are part of the total system, during a measurement there is an `effective collapse' of the state of the system that is measured~\cite{vaidman2002many, vaidman2024conservation}. This effective collapse is because each of these observers lives in a single world, and lacks access to the overall state. The observer in each single world can calculate probabilities as follows.
	
	Consider Example \ref{eqmex1} again, but with an additional observer. The measuring system measures the quantum system, and there is no interaction between the new observer and either the measuring device or the measured quantum system. The state of the new observer does not change while the joint state of the measuring and quantum systems is 
	\begin{equation}\label{everettabs}
	\tikzfig{interpretations/everettbb}
	\end{equation}	
	That is, the measuring device and the quantum system have become entangled. Note that the above diagram does not depict the additional observer. 
	
	 Now the new observer can calculate the relative states of the measuring device and the quantum system, as was done in Example \ref{eqmex1}; see diagrams (\ref{everettb2b}, \ref{everettb3b}). The observer can calculate the probabilities of definite measurement outcomes $i$ of the measuring-device state as
	 \[
	 \tikzfig{interpretations/RQMb2b4}
	 \]	
	 and the probabilities of definite measurement outcomes $i$ of the quantum state as
	 \[
	 \tikzfig{interpretations/RQMb2b5}
	 \]	
	 
	 Before the observer interacts with (\emph{i.e.,} measures) the measuring device or the quantum system, their joint state is given by diagram (\ref{everettabs}) with respect to the observer. After the interaction, the observer becomes entangled with the joint system. Now there are multiple relative states of the observer, each of which is correlated with a relative composite state of the joint system comprising the measuring device and quantum system. For each relative observer, there is an effective collapse and the observer sees a definite state of the measuring device as well as the quantum system. For illustration, suppose the observer interacts with the measuring device. Then, with respect to the observer in state $i$, the relative composite state of the measuring device and quantum system is given by\footnote{The observer, the measuring device and the quantum system undergoing measurement are denoted respectively by O, M and Q in grey.}    
	  \[
	 \tikzfig{interpretations/RQMb2b6}
	 \]	
	 where $R_o$ is the initial state of the observer, and $\widehat{U}_{R_o R}$ is the unitary entangling the observer state with the measuring-device state.
	%We have ignored the state of the additional observer.
	%Diagrammatically, we can obtain the probability distribution of the relative states of the measuring system as follows:
	%\[
	%\tikzfig{interpretations/RQMb2}
	%\]	
	%and the probability distribution of relative states of the object system is given by 
	%\[
	%\tikzfig{interpretations/RQMb3}
	%\]	
\end{remark}

\subsection{Repeated Measurements}\label{secEverettrepeat}

According to Everett~\cite{everett1957relative}, the consistency of repeated measurement outcomes arises due to the fact that, after measurement, the state of the measured system relative to a particular measuring-device state is the corresponding eigenstate. 

%"Consistency of consecutive measurements" ~\cite{deutsch2015constructor}

\begin{example}%[Repeatability of measurements]
	Consider a composite system comprising a measuring system consisting of two pointers (corresponding to initial states $R_1$ and $R_2$) and a quantum system (with state $\widehat{\psi}$) that is to be measured. The composite state is given by\footnote{The first pointer, the second pointer and the quantum system undergoing measurement are denoted respectively by P1, P2 and Q in grey.}       
\[
\tikzfig{interpretations/everettc}
\]	
When the first pointer measures the state $\widehat{\psi}$, the composite state becomes
\[
\tikzfig{interpretations/everettc2}
\]	
Relative to the first pointer registering the measurement outcome $i$, the composite state of the second pointer and the measured quantum system is given by
\[
\tikzfig{interpretations/everettc3}
\]	 
Now, if the second pointer measures the measured state again, the composite state becomes
\[
\tikzfig{interpretations/everettc4}
\]	 
and the (statistics of) relative outcome(s) of the second pointer's measurement is given by 
\[
\tikzfig{interpretations/everettc5}
\]	 
For illustration, we define the measured state as $\tikzfig{interpretations/everettb4}$. Since the pointers are performing the same measurement, we pick both their ready states as $\tikzfig{interpretations/everettb9}$ and both the unitaries as $\tikzfig{interpretations/everettb10}$. Then the above diagram becomes
\[
\scalebox{0.8}{\tikzfig{interpretations/everettc6}}\ \overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/everettc7}} \ \overset{(id)}{=} \  \scalebox{0.8}{\tikzfig{interpretations/everettc8}}
\]	 
\[
\overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/everettc9}} \ = \ \scalebox{0.8}{\tikzfig{interpretations/everettc10}} \ \overset{(f)}{=} \  \scalebox{0.8}{\tikzfig{interpretations/everettc11}}
\]	 
This shows that the outcome of second measurement agrees with the outcome of the first measurement.

%\textcolor{red}{also need to be consistent about what is a measurement outcome. and what is a relative state. single wire or double wire}
\end{example}

\subsection{The EPR-Bell Scenario}\label{secEverettEPR}

\begin{example}%[EPR-Bell scenario]
	In the EPR-Bell scenario, there are two measuring systems corresponding to Alice (A) and Bob (B), initially in the states $\tikzfig{interpretations/everettd1}$ and $\tikzfig{interpretations/everettd2}$ respectively. Before Alice and Bob measure the Bell state, the composite state is given by the diagram
	\[
	\tikzfig{interpretations/everettd3}
	\]
	When Alice and Bob perform measurements (with measurement bases set with unitaries $\widehat U_{\Phi}$ and $\widehat U_{\Psi}$ respectively), their ready states get entangled with the respective subsystems of the Bell state.
	\[
	\tikzfig{interpretations/bell4}
	\]
%	\textcolor{red}{unitaries above? what are they? one line?}
\noindent Now, the composite state of Alice's and Bob's measuring systems relative to the composite measured state $i \otimes j$ is given by
	\[
\tikzfig{interpretations/everettd4}
\]
 and the measurement statistics of the Alice-Bob composite relative states are given by the diagram
\[
\tikzfig{interpretations/bell4c} 
\]
\noindent If only Alice performed a measurement, the state of the overall composite system would be
	\[
\tikzfig{interpretations/everettd5}
\]
The composite state of Bob's pointer and part of the bipartite system relative to Alice's ONB measurement $i$ is
	\[
\tikzfig{interpretations/everettd6}
\]
For the sake of simplicity, let's pick the Z basis for measurement; then we can have $\tikzfig{interpretations/everettb9}$ as Alice's ready state and $\tikzfig{interpretations/everettb10}$ as the unitary. The above diagram of Bob's composite state becomes
	\[
\scalebox{0.8}{\tikzfig{interpretations/everettd7}} \ \overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/everettd8}} 
\ \overset{(id)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/everettd9}} 
\]
\[
\ \overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/everettd10}}
\ \overset{(\ref{picopyrule})  /  (c)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/everettd11}} \ = \ \scalebox{0.8}{\tikzfig{interpretations/everettd12}}
\]
which shows that if Bob performs a measurement in the same basis, he will measure the same state as Alice did.

%\textcolor{red}{should Bob's ready state be removed from all diagrams for this case?}

%\textcolor{red}{is the copy rule for pi state defined in last chapter?}

This confirms that in the EPR-Bell scenario, the two subsystems of the Bell state are entangled.
\end{example}

\begin{remark}[Difference between RQM and Everettian quantum mechanics]
	The main difference between relational quantum mechanics and Everettian quantum mechanics is the status of quantum states. In RQM, there are no absolute states; every state is relative to some system. On the other hand, in Everettian quantum mechanics, there are both absolute and relative states. For instance, as we saw in Example \ref{eqmex1}, after measurement takes place, we cannot meaningfully talk about the absolute state of the subsystem, only the state of a subsystem relative to a given state of the other subsystem. Essentially, the relativity of states in the Everettian interpretation is with respect to \textit{branches}, in contrast to the relativity of states with respect to \textit{systems} in RQM.
\end{remark}

\begin{remark}
One argument against the Everettian interpretation and its derivatives is that if unitary processes are all that there is as far as the evolution of states is concerned, why do we observe collapses? A response to this line of reasoning is that unitarity holds as long as the system is closed. The whole universe, or rather \textit{multiverse}, itself is a unitarily evolving closed system; in other words, there is a universal state that always evolves unitarily. We have access to a small part of it, which is not a closed system and hence does not evolve unitarily. At each measurement, every possible outcome takes place but we see an `effective collapse' because we have access to only one world that is not a closed system~\cite{vaidman2024conservation}.

Essentially this argument uses Stinespring dilation (Eq. (\ref{stinespring2})), to argue that the ontology of quantum theory comprises unitary processes only. We see non-unitary processes because of our limited experience; we cannot access the complete process. This commitment to unitary processes at the ontological level is sometimes called the `church of the larger Hilbert space'.%\footnote{where they bow before Lord $\Psi$, the universal state!}
\end{remark}

\begin{remark}
	Everettian quantum theory gives a privileged status to unitary evolution and quantum states, and is quiet on other kinds of processes. Unitary processes and quantum states alone do not make a compositional theory without including isometries, which are more general processes than unitaries. See Remark \ref{privilegeunitary} for more detail.
	%For instance, parallel composition of a unitary process and a state
	%\[
	%\dmap{\widehat U} \ \tikzfig{interpretations/copenhagen0}
	%\]
	%yields an isometry; that is, neither a unitary process nor a state.
\end{remark}

\begin{remark}
	Since the Everettian or many worlds interpretation suggests a branching worlds or multiverse ontology, it would make sense to represent this branching process diagrammatically. This could be achieved by including additive structure (direct sums/biproducts) in CQM~\cite{abramsky2004categorical, coecke2007linearizing, selinger2007dagger} to represent superpositions and branches. This would lead to a sheet diagrammatic representation like those in Refs.~\cite{staton2015algebraic, comfort2020sheet} or a `many-worlds' calculus~\cite{chardonnet2022many}. The former representation is likely too complex to be useful in practice. 
	%We leave such investigations to future work.
\end{remark}


\section{Hidden Variable Models}\label{sechidden}

Another class of `interpretations' of quantum theory essentially aim at providing a completion of the theory, usually by rejecting the claim that a quantum state provides a complete description of a physical system. These theories or models supplement the quantum state with additional variable(s). Alternatively, these models add additional variable(s) to the measurement process. Therefore, these are called additional variable or hidden variable theories.\footnote{The term `hidden variable' is not really accurate to describe all of these models. These variables are not derivable from the quantum state, but need not actually be `hidden'~\cite{bricmont2023broglie}.} There are two main motivations to consider a hidden or additional variable theory -- either to make quantum theory deterministic, or to remove nonlocality from it. In this section, we shall explore these two possibilities within CQM.

\subsection{Hidden variables -- Take I}

Here we start by adding hidden variables to the `measurements' rather than the states. In standard quantum theory, the measurement process is indeterministic. In Section \ref{secTQM}, we saw that an ONB measurement is represented by the family of processes
\[
\left(\dmap{\widehat P^i}\right)^i \ = \  \left(\tikzfig{interpretations/copenhagen2b}\right)^i
\]
When such a measurement happens, one of the process from the above list or collection takes place, but \textit{which} one takes place cannot be predicted using standard quantum theory. One can give a \textit{deterministic} model of the process by defining the projectors as cq-maps with classical controls given by ONB states $\{i\}_i$.
\begin{equation}\label{eqbenakb}
\left(\dmap{\widehat P^i}\right)^i \ := \  \left(\tikzfig{interpretations/bekanb}\right)^i 
\end{equation}
The classical variables $\{i\}_i$ form the set of hidden variables of the measurement process. Each single instance of measurement has an associated variable $i$ from this set. Determinism in this context means that given access to the variables $\{i\}_i$, one can predict which projector from the above list is applied in a particular measurement. In other words, prediction of individual measurement outcomes requires access to $\{i\}_i$. 

%Since during the measurement process, the variable $i$ is not known, we can account for this ignorance by representing measurement as a \textit{convex combination} or \textit{mixture} of quantum processes\cite{CKbook}:
%\[
%\sum_{i} p^i \dmap{\widehat P_i}   \ = \ \tikzfig{interpretations/bekan13b}
%\]
%\textcolor{red}{I dont think convex combination (mixing) is relevant here. MIXING is for mixing quantum processes; not branches of processes.}
%and the components of the mixture can be obtained by plugging ONB states into the classical input as defined in Eq. (\ref{eqbenakb}). 

Alternatively, the hidden variable may be considered part of the state instead of the measurement. To illustrate this aspect, we provide an example of a hidden variable model of a single quantum system below.

\begin{example}[A hidden variable model of a single system]\label{exsingle}
	Consider a single quantum system that is described by the quantum state $\widehat{\psi}$. 
\[
\tikzfig{interpretations/hidden1c}
\]
The state $\widehat{\psi}$ evolves unitarily % in the absence of measurement.
%\[
%\tikzfig{interpretations/hidden1d}
%\]
and is then subjected to an ONB measurement. The overall process is given by%, the outcome of which is given by 
\begin{equation}\label{onticstate}
%\tikzfig{interpretations/hidden1e}
\tikzfig{interpretations/hidden1e2}
\end{equation}
The experimenter makes the choice of a measurement basis, which amounts to choosing the family of projectors
\[
\left(\dmap{\widehat P^i}\right)^i \ = \  \left(\tikzfig{interpretations/copenhagen2b}\right)^i = \left(\tikzfig{interpretations/bekanb}\right)^i 
\]
but for this particular instance of the measurement, the hidden variable $i$ determines the projector that is chosen from the list. In this sense, the hidden variable is part of this measurement. 
\[
\tikzfig{interpretations/hidden1e}
\]
The overall measurement process includes a set of hidden variables $\{i\}_i$ 
\[
%\tikzfig{interpretations/hidden1f}
\tikzfig{interpretations/hidden1f2}
\]
Another way to think of the whole process is as follows; see the diagram below. The measurement basis is in the control of the experimenter. But the complete description of the quantum system is not known to the experimenter. The experimenter can prepare the state $\widehat{\psi}$ up to some hidden variable $i$. The outcome of a particular instance of measurement is dependent not only on $\widehat{\psi}$ but also on the variable $i$. As the experimenter cannot access $i$, indeterminism results.
\begin{equation}\label{statehidden}
\tikzfig{interpretations/hidden1g}
\end{equation}
In this sense, the quantum state supplemented by a set of hidden variables gives a complete description of the physical system.
\end{example}

\begin{remark}
In such a model as described in the above example, determinism is regained; does it mean there is no need for calculating probabilities? Very much like in Everettian quantum theory, determinism regained in the theoretical model does not imply one is not allowed to use the Born rule while making quantum mechanical predictions. Precisely because the experimenter does not have access to the hidden variables, they have to take into account the `effective collapse' of the state and cannot help but calculate probabilities. For the scenario described in Example \ref{exsingle}, the probability of measurement outcome $i$ is given by 
 \[
\tikzfig{interpretations/hidden1eb}
\]
\end{remark}

\begin{comment}
\begin{remark}
 Consider again the scenario described in Example (\ref{exsingle}). For the experimenter who has no access to the hidden variable (and who has not yet seen the measurement outcome), the state of the system after measurement is described by the mixture 
 \[
 \tikzfig{interpretations/hidden1h}
 \]
 \textcolor{red}{revisit this mixture thing}
 
 where $p$ represents a probability distribution. This is an \textit{epistemic} state as it represents what the experimenter knows about the state of the quantum system. The state in diagram (\ref{onticstate}) on the other hand is \textit{ontic} state because it represents the actual state of the system. Once the experimenter sees the measurement outcome, the epistemic state collapses. 
  \[
 \tikzfig{interpretations/hidden1i}
 \]
\end{remark}
\end{comment}

\begin{example} [A hidden variable model of two systems]
Consider two physical systems that are to be described with a hidden variable model. These systems evolve unitarily and then are subjected to ONB measurements. If the two systems are completely independent of each other, the overall process may be described as the parallel composition of diagrams of the kind in diagram (\ref{statehidden}):
\[
\tikzfig{interpretations/hidden2b}
\]
%\textcolor{red}{BIG TODO: superscript outcome? subscript numbering of process? make it consistent.}
\noindent If the two systems are subjected to ONB measurements in the same basis, then it is possible for the two systems to have a common set of hidden variables. This is depicted in the diagram
\begin{equation}\label{eqclasscorr}
	\tikzfig{interpretations/hidden2c}
\end{equation}
where a copy map copies the hidden variables and then supplies them to the classical controls of the two cq-maps. This diagram shows that the two systems are subjected to measurements $\ \left(\tikzfig{interpretations/bekanc}\right)^i \ \  \text{and} \ \ 
\left(\tikzfig{interpretations/bekand}\right)^i \ \  \text{respectively}$. The two measurements are in the same basis while the hidden variable ensures that the measurement outcomes are correlated.
\end{example}

\begin{remark}
There are two ways to think of the set of hidden variables in diagram (\ref{eqclasscorr}). It could be considered part of the state
\[
\tikzfig{interpretations/hidden2d}
\]
or part of the measurement.
\[
\tikzfig{interpretations/hidden2e}
\]
\end{remark}




\begin{remark}
	The two systems in the state (\ref{eqclasscorr}) are classically correlated. The diagram shows that whenever the first system is subjected to the measurement
	\[
	\tikzfig{interpretations/bekanc}
	\]
	the second is subjected to 
	\[
	\tikzfig{interpretations/bekand}
	\]
	If both measurements are in the  Z basis, $\left\{\dpointmap{0}, \dpointmap{1}\right\}$, and we do not have access to the hidden variable $i$, the \textit{epistemic} state is obtained by plugging a uniform distribution of ONB states, which (ignoring the normalisation scalar) is $\ \tikzfig{interpretations/codelete}\ $,  in place of the classical input.
		\[
	\scalebox{0.8}{\tikzfig{interpretations/hidden2c2}} \ \overset{(f)}{=} \ 	\scalebox{0.8}{\tikzfig{interpretations/hidden2c3}} \
\overset{(id)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/hidden2c4}} 
\]
\[
\ = \ 	\scalebox{0.8}{\tikzfig{interpretations/hidden2c5}}
\]	
The classical cup means that even though we do not know the exact state of the first or the second system, if we measure their states the measurement outcomes will be classically correlated. 
\end{remark}

While one can derive satisfaction from having a deterministic hidden variable model of quantum measurement as described above, these models cannot account for entangled states and their violation of Bell's inequality~\cite{bell1964einstein}. For an entangled system, the model must include a quantum cup. We provide an example of such a model below.

\begin{example}[The EPR-Bell scenario]
	
Consider measurements of the Bell state in the EPR setting. If measurements of both the systems are in the same ONB, one can assign classical hidden variables $\{i\}_i$ that determine the outcomes of both measurements. 
	\[
		\tikzfig{interpretations/hidden2f}
	\]
%This model fails to violate the Bell inequalities. 
The presence of the quantum cup means the bipartite state violates the Bell inequalities. Given access to the hidden variables $\{i\}_i$, the individual measurement outcomes can be predicted with certainty. 
\end{example}

\subsection{Hidden variables -- Take II}

So far, we have discussed hidden variables that are introduced to account for the indeterminism in quantum theory. These variables (in addition to the quantum states) determine measurement outcomes, but it was the quantum state that was measured. 

One can have another kind of hidden variable model in which the quantum state influences the additional variables and it is the additional variables that are measured. This is in the spirit of Bohmian mechanics~\cite{bohm1952suggested, bohm1952suggestedii} % in the sense that the quantum state gives a partial description of the physical system. 
%The state evolves unitarily but cannot be directly measured. When measurement is performed, it is the hidden variable that is measured. 
in which the hidden variable is guided by the state. We describe such a toy model of Bohmian mechanics with examples below.

\begin{example}[Single system]
	The complete description of a physical system is given by its quantum state $\widehat{\psi}$ and a classical variable $\lambda$.
\[
\tikzfig{interpretations/bohm0}
\]
As long as there is no measurement, the state evolves unitaraily and the classical variable is not affected. 
\[
\tikzfig{interpretations/bohm0b}
\]
During a measurement, the classical variable and the state interact and afterwards the classical variable is measured as follows. 
\[
\tikzfig{interpretations/bohm0c2}
\]
The complete `measurement' process comprises the following components: the quantum state undergoes a unitary process $\widehat{U}_{\Phi}$ accounting for the setting of the measurement basis. The classical variable is encoded as a quantum state and is then influenced by the state via an entangling unitary interaction $\widehat U_{\lambda \widehat{\psi}}$. Finally, the encoded classical variable is measured and the quantum state is discarded.  
\end{example}

\begin{remark}
	As an illustration, we can provide a more fine-grained description of the above example by defining the interaction unitary and the hidden variable. Consider a slightly simpler version of the overall process.
	\[
	\tikzfig{interpretations/bohm0d}
	\]
	Using definitions $\ 	\tikzfig{interpretations/bohm0f} \ := \  \tikzfig{interpretations/everettb10}\ $ and  $\ 	\tikzfig{interpretations/bohm0e} \ := \  \tikzfig{interpretations/bohm0g}\ $, we have
		\[
	\tikzfig{interpretations/bohm0h}
	\]
In the diagram above, the state $\widehat{\psi}$ undergoes  unitary evolution represented by the process $\widehat{U}_{\Phi}$. The measurement process includes encoding the hidden variable $0$ into a quantum state. This encoded hidden variable then interacts with the original quantum state of the system via a CNOT gate. The original quantum state acts as the control whereas the hidden variable acts as the target of the CNOT gate. Finally, the hidden variable is measured and the original quantum state is discarded. The diagram can be simplified as follows.	
		\[
\scalebox{0.8}{\tikzfig{interpretations/bohm0h}} \ = \ \scalebox{0.8}{\tikzfig{interpretations/bohm4}} \ \overset{(c)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/bohm4b}}
\overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/bohm4c}}
\]
\[
\overset{(id)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/bohm4d}} \ \overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/bohm4e}}
\overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/bohm4f}} \ = \ \scalebox{0.8}{\tikzfig{interpretations/bohm4g}} 
\]	
\noindent The simplified diagram mirrors exactly the textbook quantum theory we would use to describe the measurement.
\end{remark}


\begin{remark}
	What is the role of the hidden variable in the model above?	It can be considered a pointer state that records the quantum state of the physical system under investigation. The hidden variable becomes relevant only during the measurement; that is, it can be considered part of the measurement process.
	\begin{equation}\label{bohm0d2}
	\tikzfig{interpretations/bohm0d3}
	\end{equation}
\end{remark}

\begin{remark}
	One can compare the hidden variable model of measurement with measurement in Everettian quantum theory. The two are similar in the sense that the quantum state gets entangled with another state during the measurement. In the hidden variable model, the classical hidden variable is encoded into a quantum state that gets entangled with the state that is to be measured. In Everettian quantum theory, the quantum state of the measuring device gets entangled with the state to be measured. The difference is that in Everettian quantum theory, every measurement outcome is realised whereas in the hidden variable model, a single outcome is realised. From a diagrammatic perspective, this means that a single diagram (\ref{bohm0d2}) completely characterises measurement in the hidden variable model. On the other hand, there are multiple diagrams (of the relative subsystem states, and the absolute composite state) characterising measurement in the Everettian interpretation; see Example \ref{eqmex1} and Remark \ref{remarkeverett}.
\end{remark}

%\begin{remark}
%	ontology of hidden variable
%\end{remark}

%define what are the hidden vairables and how do they differ from wavefunction

\subsection{The EPR-Bell Scanario}\label{sechiddenEPR}

\begin{example}%[EPR scenario]
In the EPR scenario, we can model the physical system by an entangled state and two hidden variables.
\[
\tikzfig{interpretations/bohm11b}
\]
When Alice and Bob perform measurements in their respective measurement bases, the hidden variables get updated via interaction with the quantum state and become accessible to Alice and Bob.
\[
\tikzfig{interpretations/bohm11}
\]
Inside the unitary boxes, there are unitaries that correspond to the setting of measurement bases by Alice and Bob respectively, followed by unitary maps that entangle Alice's and Bob's part of the bipartite state with their respective hidden variables (encoded as quantum states).
\begin{equation}\label{hiddenepr}
\tikzfig{interpretations/bohm12}
\end{equation}
We can further specify the example by using the following definitions 
\[
\tikzfig{interpretations/bohm12b} \ := \ \tikzfig{interpretations/bohm0g} \ , \ \ \ 
\tikzfig{interpretations/bohm12c} \ :=\ \tikzfig{interpretations/bohm0g} \ , \ \ \ 
  \tikzfig{interpretations/bohm12d} \ := \ \tikzfig{interpretations/everettb10} \ , \ \ \  \tikzfig{interpretations/bohm12e} \ := \ \tikzfig{interpretations/everettb11} 
\]
Diagram (\ref{hiddenepr}) becomes
\[
\tikzfig{interpretations/bohm12f}
\]
In the above diagram, Alice's and Bob's subsystems are subjected to measurements with bases set by unitaries $\widehat U_{\Phi}$ and $\widehat U_{\Psi}$ respectively. The measurement process includes encoding the hidden variables---each of which is $0$---into quantum states. The encoded hidden variables interact with the quantum states of the subsystems via CNOT gates. At the end of the measurement process, the hidden variable states are measured and the original quantum state is discarded. 
%The diagram can be simplified as follows
\noindent After simplification, we get the same diagram as that of the EPR-Bell scenario in textbook quantum theory.
\[
\scalebox{0.8}{\tikzfig{interpretations/bohm12f}} \ \overset{(c)}{=} \  \scalebox{0.8}{\tikzfig{interpretations/bohm12g}} 
\overset{(f)}{=}\ \scalebox{0.8}{\tikzfig{interpretations/bohm12h}}
\]
\[ \overset{(id)}{=} \  \scalebox{0.8}{\tikzfig{interpretations/bohm12i}} 
\overset{(f)}{=} \ \scalebox{0.8}{\tikzfig{interpretations/bohm12j}} \ \overset{(f)}{=} \  \scalebox{0.8}{\tikzfig{interpretations/bohm12k}} 
\]
\end{example}


\begin{remark}
	The above hidden variable model is different from Bohmian mechanics~\cite{bohm1952suggested, bohm1952suggestedii, tumulka2021bohmian} in at least two respects. Bohmian mechanics is explicitly more nonlocal than our model. Apart from the non-locality that arises from the entangled state, the evolution of each hidden variable in Bohmian theory is also dependent on the values of all hidden variables. Moreover, in a Bohmian theory, the hidden variable is continuously guided by the state whether or not there is measurement. In our model, the hidden variable is updated only when a measurement is performed. 
	
	We leave the diagrammatic exploration of Bohmian hidden variable models and theories to future work. A good place to start will be modelling quantum computation within a Bohmian interpretation of quantum theory~\cite{roser2010quantum, roser2012quantum}. 
\end{remark}

\begin{comment}
	content...

\section{Discussion}

CQM and Interpretations of Quantum Theory

CQM and the Measurement Problem

CQM and Quantum Ontology

%\begin{remark}
%	information flow structure like that of textbook quantum theory...
%\end{remark}

%\textcolor{blue}{Also diagrammatic `definitions' of measurement!!!}

%\textcolor{red}{Read Oxford handbook for good intros to all interpretations. use it for providing intros and explanations!!!!!1}

We have looked at quantum measurement, and in particular its interpretations~\cite{everett1957relative, brown2019everettian, schlosshauer2019quantum, bohm1952suggested, bohm1952suggestedii, rovelli1996relational, rovelli2021relational} through a compositional lens.

After looking at these interpretations in the canvas of CQM, one may conclude that quantum theory needs no interpretation. 

%other graphical calculi

The diagrammatic representations clearly reflect the varied levels of complexity of structure involved in these interpretations. 

%The structural relationships between the different interpretations may be of interest to the structural realist.





%Now that we have diagrammatic versions of the different interpretations, let's try to answer the following questions:

%Some questions to think about:


What are the quantum and classical structures involved in the theory?    

What are the structural and conceptual relationships between the different interpretations?    

Which is the most natural interpretation of quantum mechanics from a compositional point of view?   
Can we develop a process ontology for quantum physics?


Maudlin beables etc... object ontology.... vs all interpretations in process relational ontology.

%\textcolor{red}{HEISENBERG VS SCHRODINGER PICTURE}

ONTOLOGY

PROCESS ONTOLOGY

PROCESS PHILOSOPHY

%POTENTIALITY REALISM? flavio del santo reference

IS CQM AN INTERPRETATION? WHY AND HOW? \textcolor{red}{nice discussion in Nick's interpretation paper}

%we have only focused on qubits here \textcolor{red}{clarify in the beginning of the chapter}. potential to expand on this work to general quantum states. 

%limitations and future work

my defence of interpretatiosn in slack worklog

CQM being like ZX but for interpretations (provide generators for interpretations)

%justify starting from CQM aka doubling for all the interpretations

%justify using just qubits and discarding

%probability in RQM... same diagram for others too?... collapse of unitary?

%why not POVM

%probabilities in EQM

%calculating probabilities in RQM

%should not EQM be pure processs only? 

%why CPM for many worlds?

%no probailities in EQM or will they be derived?

%EQM --> stinespring argument

%discussion of measurement problem and interpretations in the dodo book

\textcolor{blue}{comments on RQM as a relational interpretation, which is natural from CQM point of view}

%\printbibliography
\end{comment}

